Globular clusters of NGC 3115 in the near-infrared. Demonstrating the correctness of two opposing scenarios

We combined new near-infrared VLT/HAWK-I data of the globular clusters (GCs) in the isolated edge-on S0 galaxy NGC 3115 with optical and spectroscopic ones taken from the literature, with the aim of analyzing the multiband GC color distributions. A recent study from the SLUGGS survey has shown that the GCs in this galaxy follow a bimodal distribution of Ca II triplet indices. Thus, NGC 3115 presents a critical example of a GC system with multiple, distinct, metallicity subpopulations, and this may argue against the "projection" scenario, which posits that the ubiquitous color bimodality mainly results from nonlinearities in the color-metallicity relations. Using optical, NIR, and spectroscopic data, we found strong and consistent evidence of index bimodality, which independently confirms the metallicity bimodality in NGC 3115 GCs. At the same time, we also found evidence for some color-color nonlinearity. Taken in the broader context of previous studies, the multicolor consistency of the GC bimodality in NGC 3115 suggests that in cases where GC systems exhibit clear differences between their optical and optical-NIR color distributions (as in some giant ellipticals), the apparent inconsistencies most likely result from nonlinearities in the color-metallicity relations.

==> table_jhk_full.tex <==
\begin{table}
\scriptsize
\caption{Matched HAWK--I $JHKs$ photometry for all detected sources}
\label{tab_jhks}
\centering
\begin{tabular}{l c c c c c c}
\hline\hline 
   ID  &   R.A.     &   Dec.     &            $m_J$         &           $m_H$          &            $m_{Ks}$      &$\langle CS\rangle$ \\
       & (J2000)    & (J2000)    &            (mag)         &           (mag)          &           (mag)        &           \\
   (1) &   (2)      &   (3)      &            (4)           &           (5)            &           (6)          &     (7)    \\
\hline
     1 & 151.261846 &  -7.778326 &     14.532 $\pm$   0.001 &    14.560 $\pm$   0.001 &    14.832 $\pm$   0.001 &      0.997 \\ 
     2 & 151.339249 &  -7.779547 &     15.262 $\pm$   0.002 &    15.290 $\pm$   0.001 &    15.713 $\pm$   0.001 &      0.990 \\ 
     3 & 151.328988 &  -7.781540 &     13.407 $\pm$   0.001 &    13.335 $\pm$   0.001 &    13.949 $\pm$   0.001 &      1.000 \\ 
     4 & 151.246152 &  -7.782556 &     20.196 $\pm$   0.013 &    20.526 $\pm$   0.018 &    21.869 $\pm$   0.061 &      0.020 \\ 
     5 & 151.280919 &  -7.782237 &     19.050 $\pm$   0.007 &    19.092 $\pm$   0.006 &    19.317 $\pm$   0.008 &      0.983 \\ 
     6 & 151.282733 &  -7.782252 &     20.158 $\pm$   0.012 &    20.086 $\pm$   0.013 &    20.282 $\pm$   0.017 &      0.983 \\ 
     7 & 151.326993 &  -7.782593 &     21.895 $\pm$   0.047 &    21.797 $\pm$   0.050 &    21.289 $\pm$   0.037 &      0.460 \\ 
     8 & 151.371508 &  -7.782564 &     22.534 $\pm$   0.080 &    22.320 $\pm$   0.077 &    21.803 $\pm$   0.056 &      0.570 \\ 
     9 & 151.279711 &  -7.782779 &     22.404 $\pm$   0.072 &    22.729 $\pm$   0.112 &    22.149 $\pm$   0.083 &      0.593 \\ 
    10 & 151.280276 &  -7.782759 &     23.078 $\pm$   0.130 &    22.863 $\pm$   0.127 &    22.582 $\pm$   0.121 &      0.547 \\ 
    11 & 151.318578 &  -7.782969 &     20.862 $\pm$   0.021 &    20.072 $\pm$   0.013 &    19.673 $\pm$   0.010 &      0.490 \\ 
    12 & 151.276504 &  -7.782910 &     23.067 $\pm$   0.129 &    22.762 $\pm$   0.115 &    22.211 $\pm$   0.087 &      0.500 \\ 
    13 & 151.349516 &  -7.782973 &     21.800 $\pm$   0.042 &    20.288 $\pm$   0.015 &    20.175 $\pm$   0.015 &      0.323 \\ 
    14 & 151.335713 &  -7.782982 &     22.872 $\pm$   0.104 &    21.301 $\pm$   0.032 &    20.842 $\pm$   0.025 &      0.277 \\ 
    15 & 151.333685 &  -7.782999 &     21.788 $\pm$   0.040 &    17.351 $\pm$   0.002 &    17.846 $\pm$   0.003 &      0.907 \\ 
    16 & 151.321701 &  -7.659079 &     22.806 $\pm$   0.105 &    22.827 $\pm$   0.133 &    22.089 $\pm$   0.083 &      0.600 \\ 
    17 & 151.254927 &  -7.659200 &     23.275 $\pm$   0.154 &    22.849 $\pm$   0.123 &    22.350 $\pm$   0.091 &      0.533 \\ 
    18 & 151.283626 &  -7.659647 &     22.516 $\pm$   0.080 &    22.309 $\pm$   0.081 &    21.187 $\pm$   0.036 &      0.280 \\ 
    19 & 151.249497 &  -7.659720 &     23.086 $\pm$   0.130 &    22.891 $\pm$   0.128 &    22.381 $\pm$   0.093 &      0.507 \\ 
    20 & 151.295751 &  -7.659781 &     22.640 $\pm$   0.091 &    22.284 $\pm$   0.081 &    21.667 $\pm$   0.056 &      0.837 \\ 
    21 & 151.363185 &  -7.659687 &     23.220 $\pm$   0.145 &    23.062 $\pm$   0.148 &    22.520 $\pm$   0.106 &      0.467 \\ 
    22 & 151.266671 &  -7.659817 &     22.963 $\pm$   0.116 &    22.820 $\pm$   0.123 &    22.354 $\pm$   0.095 &      0.507 \\ 
    23 & 151.291570 &  -7.659904 &     21.982 $\pm$   0.051 &    22.380 $\pm$   0.088 &    21.513 $\pm$   0.049 &      0.010 \\ 
    24 & 151.325154 &  -7.659852 &     22.367 $\pm$   0.072 &    22.422 $\pm$   0.093 &    22.636 $\pm$   0.137 &      0.503 \\ 
    25 & 151.288847 &  -7.660173 &     22.359 $\pm$   0.071 &    22.523 $\pm$   0.099 &    22.556 $\pm$   0.123 &      0.660 \\ 
    26 & 151.343589 &  -7.660227 &     22.472 $\pm$   0.076 &    22.748 $\pm$   0.118 &    22.104 $\pm$   0.083 &      0.447 \\ 
    27 & 151.359311 &  -7.660344 &     20.936 $\pm$   0.021 &    20.953 $\pm$   0.024 &    20.955 $\pm$   0.028 &      0.967 \\ 
    28 & 151.296608 &  -7.660451 &     19.950 $\pm$   0.011 &    19.810 $\pm$   0.011 &    19.814 $\pm$   0.012 &      0.970 \\ 
    29 & 151.362195 &  -7.660574 &     18.369 $\pm$   0.005 &    18.490 $\pm$   0.004 &    18.748 $\pm$   0.005 &      0.980 \\ 
    30 & 151.254433 &  -7.660686 &     20.761 $\pm$   0.019 &    20.610 $\pm$   0.019 &    20.079 $\pm$   0.014 &      0.570 \\ 
    31 & 151.278946 &  -7.660762 &     20.722 $\pm$   0.018 &    20.625 $\pm$   0.019 &    19.984 $\pm$   0.014 &      0.357 \\ 
    32 & 151.320166 &  -7.660721 &     21.350 $\pm$   0.030 &    21.366 $\pm$   0.037 &    21.385 $\pm$   0.045 &      0.960 \\ 
    33 & 151.337357 &  -7.660828 &     22.260 $\pm$   0.064 &    22.610 $\pm$   0.108 &    21.710 $\pm$   0.060 &      0.107 \\ 
    34 & 151.248288 &  -7.660839 &     21.804 $\pm$   0.043 &    21.741 $\pm$   0.047 &    21.986 $\pm$   0.066 &      0.860 \\ 
    35 & 151.315570 &  -7.660961 &     21.687 $\pm$   0.040 &    21.697 $\pm$   0.049 &    21.105 $\pm$   0.035 &      0.127 \\ 
    36 & 151.259447 &  -7.661394 &     19.547 $\pm$   0.009 &    19.562 $\pm$   0.009 &    18.914 $\pm$   0.006 &      0.043 \\ 
    37 & 151.289066 &  -7.661596 &     20.886 $\pm$   0.021 &    20.983 $\pm$   0.026 &    20.284 $\pm$   0.017 &      0.030 \\ 
    38 & 151.347392 &  -7.661598 &     21.778 $\pm$   0.042 &    21.821 $\pm$   0.052 &    21.116 $\pm$   0.035 &      0.147 \\ 
    39 & 151.254582 &  -7.661662 &     21.528 $\pm$   0.034 &    21.477 $\pm$   0.037 &    21.530 $\pm$   0.044 &      0.863 \\ 
    40 & 151.302251 &  -7.661898 &     20.694 $\pm$   0.019 &    20.620 $\pm$   0.020 &    20.050 $\pm$   0.015 &      0.820 \\ 
    41 & 151.355952 &  -7.661719 &     22.757 $\pm$   0.097 &    21.904 $\pm$   0.054 &    21.427 $\pm$   0.043 &      0.523 \\ 
    42 & 151.308055 &  -7.662184 &     21.052 $\pm$   0.025 &    20.957 $\pm$   0.026 &    19.934 $\pm$   0.014 &      0.023 \\ 
    43 & 151.265820 &  -7.662262 &     21.648 $\pm$   0.037 &    21.773 $\pm$   0.050 &    21.192 $\pm$   0.035 &      0.053 \\ 
    44 & 151.269997 &  -7.662174 &     22.796 $\pm$   0.101 &    22.566 $\pm$   0.100 &    21.771 $\pm$   0.059 &      0.707 \\ 
    45 & 151.253564 &  -7.662504 &     20.242 $\pm$   0.013 &    20.348 $\pm$   0.015 &    19.946 $\pm$   0.013 &      0.043 \\ 
    46 & 151.345945 &  -7.662435 &     22.474 $\pm$   0.076 &    22.275 $\pm$   0.078 &    21.599 $\pm$   0.053 &      0.830 \\ 
    47 & 151.328977 &  -7.662564 &     22.928 $\pm$   0.120 &    22.853 $\pm$   0.139 &    22.334 $\pm$   0.106 &      0.597 \\ 
    48 & 151.274360 &  -7.663059 &     20.676 $\pm$   0.018 &    20.437 $\pm$   0.017 &    19.492 $\pm$   0.009 &      0.030 \\ 
    49 & 151.354556 &  -7.662952 &     22.552 $\pm$   0.081 &    22.634 $\pm$   0.103 &    21.666 $\pm$   0.053 &      0.107 \\ 
    50 & 151.298481 &  -7.662965 &     22.339 $\pm$   0.071 &    22.407 $\pm$   0.091 &    22.275 $\pm$   0.098 &      0.683 \\ 
    51 & 151.248942 &  -7.663516 &     17.999 $\pm$   0.004 &    17.909 $\pm$   0.003 &    17.986 $\pm$   0.003 &      0.980 \\ 
    52 & 151.329109 &  -7.663610 &     19.889 $\pm$   0.011 &    19.795 $\pm$   0.011 &    19.200 $\pm$   0.008 &      0.037 \\ 
    53 & 151.300730 &  -7.663245 &     22.580 $\pm$   0.088 &    22.280 $\pm$   0.082 &    21.419 $\pm$   0.046 &      0.480 \\ 
    54 & 151.357923 &  -7.663648 &     17.867 $\pm$   0.004 &    17.765 $\pm$   0.003 &    17.849 $\pm$   0.003 &      0.980 \\ 
    55 & 151.255034 &  -7.664390 &     17.733 $\pm$   0.004 &    17.777 $\pm$   0.003 &    17.369 $\pm$   0.003 &      0.030 \\ 
    56 & 151.347123 &  -7.663574 &     21.854 $\pm$   0.044 &    21.661 $\pm$   0.045 &    21.009 $\pm$   0.032 &      0.663 \\ 
    57 & 151.289567 &  -7.664043 &     21.377 $\pm$   0.031 &    21.384 $\pm$   0.037 &    21.446 $\pm$   0.046 &      0.753 \\ 
    58 & 151.285741 &  -7.664252 &     22.347 $\pm$   0.071 &    22.284 $\pm$   0.081 &    21.038 $\pm$   0.032 &      0.023 \\ 
    59 & 151.351126 &  -7.664237 &     19.367 $\pm$   0.008 &    19.240 $\pm$   0.007 &    19.377 $\pm$   0.009 &      0.973 \\ 
    60 & 151.336895 &  -7.664337 &     23.092 $\pm$   0.138 &    22.865 $\pm$   0.139 &    22.385 $\pm$   0.112 &      0.537 \\ 
    61 & 151.334567 &  -7.664466 &     22.299 $\pm$   0.069 &    22.234 $\pm$   0.080 &    21.335 $\pm$   0.044 &      0.103 \\ 
    62 & 151.283315 &  -7.665376 &     18.647 $\pm$   0.006 &    18.528 $\pm$   0.005 &    18.463 $\pm$   0.005 &      0.943 \\ 
    63 & 151.338615 &  -7.665349 &     22.640 $\pm$   0.093 &    22.514 $\pm$   0.102 &    21.863 $\pm$   0.070 &      0.733 \\ 
    64 & 151.268612 &  -7.665468 &     22.333 $\pm$   0.068 &    22.009 $\pm$   0.061 &    21.393 $\pm$   0.042 &      0.893 \\ 
    65 & 151.261697 &  -7.665611 &     21.985 $\pm$   0.050 &    21.855 $\pm$   0.053 &    21.066 $\pm$   0.031 &      0.207 \\ 
    66 & 151.248152 &  -7.665756 &     22.118 $\pm$   0.056 &    22.471 $\pm$   0.088 &    21.978 $\pm$   0.066 &      0.053 \\ 
    67 & 151.308068 &  -7.666037 &     17.907 $\pm$   0.004 &    17.694 $\pm$   0.003 &    17.791 $\pm$   0.003 &      0.983 \\ 
    68 & 151.346139 &  -7.666062 &     21.942 $\pm$   0.049 &    21.727 $\pm$   0.049 &    21.165 $\pm$   0.037 &      0.650 \\ 
    69 & 151.324058 &  -7.666312 &     21.540 $\pm$   0.037 &    21.472 $\pm$   0.041 &    20.697 $\pm$   0.026 &      0.183 \\ 
    70 & 151.268406 &  -7.666460 &     19.567 $\pm$   0.009 &    19.419 $\pm$   0.008 &    19.550 $\pm$   0.010 &      0.980 \\ 
    71 & 151.251007 &  -7.666490 &     21.494 $\pm$   0.033 &    21.142 $\pm$   0.028 &    20.377 $\pm$   0.017 &      0.380 \\ 
    72 & 151.320544 &  -7.666447 &     21.536 $\pm$   0.037 &    21.696 $\pm$   0.050 &    21.773 $\pm$   0.065 &      0.653 \\ 
    73 & 151.344944 &  -7.666471 &     22.958 $\pm$   0.119 &    22.454 $\pm$   0.093 &    21.548 $\pm$   0.052 &      0.457 \\ 
    74 & 151.358945 &  -7.666697 &     21.421 $\pm$   0.031 &    21.130 $\pm$   0.028 &    20.637 $\pm$   0.022 &      0.560 \\ 
    75 & 151.313734 &  -7.666831 &     22.586 $\pm$   0.091 &    22.547 $\pm$   0.106 &    22.223 $\pm$   0.097 &      0.717 \\ 
    76 & 151.325383 &  -7.667042 &     21.135 $\pm$   0.027 &    21.184 $\pm$   0.032 &    21.369 $\pm$   0.046 &      0.870 \\ 
    77 & 151.328494 &  -7.667101 &     18.942 $\pm$   0.006 &    18.807 $\pm$   0.005 &    18.992 $\pm$   0.007 &      0.980 \\ 
    78 & 151.284583 &  -7.667060 &     21.906 $\pm$   0.049 &    21.756 $\pm$   0.051 &    21.692 $\pm$   0.057 &      0.863 \\ 
    79 & 151.327894 &  -7.667150 &     22.244 $\pm$   0.069 &    21.744 $\pm$   0.053 &    20.697 $\pm$   0.026 &      0.237 \\ 
    80 & 151.270252 &  -7.667535 &     18.156 $\pm$   0.005 &    18.037 $\pm$   0.003 &    18.090 $\pm$   0.004 &      0.980 \\ 
    81 & 151.366988 &  -7.667467 &     18.450 $\pm$   0.005 &    18.344 $\pm$   0.004 &    18.561 $\pm$   0.005 &      0.980 \\ 
    82 & 151.345691 &  -7.667331 &     21.620 $\pm$   0.038 &    21.665 $\pm$   0.047 &    21.832 $\pm$   0.068 &      0.803 \\ 
    83 & 151.327638 &  -7.667863 &     22.169 $\pm$   0.065 &    22.008 $\pm$   0.067 &    21.290 $\pm$   0.043 &      0.850 \\ 
    84 & 151.310084 &  -7.667937 &     20.989 $\pm$   0.024 &    20.890 $\pm$   0.025 &    20.989 $\pm$   0.033 &      0.970 \\ 
    85 & 151.345660 &  -7.668002 &     21.998 $\pm$   0.052 &    22.031 $\pm$   0.065 &    21.453 $\pm$   0.049 &      0.230 \\ 
    86 & 151.247105 &  -7.668237 &     22.880 $\pm$   0.109 &    23.084 $\pm$   0.151 &    22.579 $\pm$   0.112 &      0.530 \\ 
    87 & 151.250217 &  -7.668313 &     22.753 $\pm$   0.097 &    22.542 $\pm$   0.094 &    21.029 $\pm$   0.030 &      0.183 \\ 
    88 & 151.347180 &  -7.668263 &     22.993 $\pm$   0.124 &    22.436 $\pm$   0.092 &    21.439 $\pm$   0.048 &      0.347 \\ 
    89 & 151.341767 &  -7.668452 &     20.970 $\pm$   0.023 &    20.820 $\pm$   0.024 &    20.241 $\pm$   0.018 &      0.153 \\ 
    90 & 151.356334 &  -7.668560 &     21.643 $\pm$   0.037 &    21.972 $\pm$   0.058 &    21.001 $\pm$   0.030 &      0.003 \\ 
    91 & 151.345008 &  -7.668480 &     22.481 $\pm$   0.080 &    22.737 $\pm$   0.122 &    22.282 $\pm$   0.102 &      0.697 \\ 
    92 & 151.372230 &  -7.668438 &     22.214 $\pm$   0.060 &    22.373 $\pm$   0.080 &    22.450 $\pm$   0.099 &      0.700 \\ 
    93 & 151.313169 &  -7.668517 &     22.722 $\pm$   0.104 &    22.413 $\pm$   0.095 &    21.895 $\pm$   0.073 &      0.513 \\ 
    94 & 151.371054 &  -7.668658 &     21.788 $\pm$   0.042 &    21.777 $\pm$   0.048 &    21.675 $\pm$   0.050 &      0.930 \\ 
    95 & 151.262780 &  -7.669027 &     18.297 $\pm$   0.005 &    18.170 $\pm$   0.004 &    18.231 $\pm$   0.004 &      0.980 \\ 
    96 & 151.331944 &  -7.668898 &     22.642 $\pm$   0.099 &    22.518 $\pm$   0.106 &    21.731 $\pm$   0.065 &      0.067 \\ 
    97 & 151.280153 &  -7.669080 &     19.595 $\pm$   0.009 &    19.639 $\pm$   0.009 &    19.786 $\pm$   0.012 &      0.980 \\ 
    98 & 151.373168 &  -7.669093 &     21.456 $\pm$   0.032 &    21.564 $\pm$   0.040 &    21.478 $\pm$   0.042 &      0.843 \\ 
    99 & 151.334822 &  -7.669288 &     20.195 $\pm$   0.014 &    20.298 $\pm$   0.016 &    20.530 $\pm$   0.023 &      0.973 \\ 
   100 & 151.305807 &  -7.669641 &     20.847 $\pm$   0.022 &    20.920 $\pm$   0.026 &    20.775 $\pm$   0.027 &      0.973 \\ 
   101 & 151.306964 &  -7.670013 &     20.476 $\pm$   0.017 &    20.551 $\pm$   0.019 &    19.705 $\pm$   0.012 &      0.023 \\ 
   102 & 151.369193 &  -7.669764 &     22.040 $\pm$   0.052 &    21.760 $\pm$   0.047 &    21.022 $\pm$   0.029 &      0.153 \\ 
   103 & 151.272370 &  -7.669820 &     22.847 $\pm$   0.109 &    22.901 $\pm$   0.139 &    22.104 $\pm$   0.080 &      0.430 \\ 
   104 & 151.276789 &  -7.669898 &     22.245 $\pm$   0.065 &    22.166 $\pm$   0.072 &    22.326 $\pm$   0.099 &      0.717 \\ 
   105 & 151.350759 &  -7.669973 &     22.497 $\pm$   0.079 &    22.503 $\pm$   0.096 &    21.629 $\pm$   0.055 &      0.457 \\ 
   106 & 151.357574 &  -7.668379 &     22.428 $\pm$   0.073 &    22.170 $\pm$   0.069 &    21.242 $\pm$   0.037 &      0.103 \\ 
   107 & 151.268419 &  -7.671567 &     18.387 $\pm$   0.005 &    18.380 $\pm$   0.004 &    17.665 $\pm$   0.003 &      0.030 \\ 
   108 & 151.353494 &  -7.670336 &     21.924 $\pm$   0.048 &    22.001 $\pm$   0.061 &    21.074 $\pm$   0.034 &      0.003 \\ 
   109 & 151.301771 &  -7.670247 &     22.507 $\pm$   0.086 &    22.591 $\pm$   0.110 &    22.185 $\pm$   0.094 &      0.450 \\ 
   110 & 151.324210 &  -7.670547 &     19.767 $\pm$   0.010 &    19.726 $\pm$   0.010 &    19.795 $\pm$   0.013 &      0.983 \\ 
   111 & 151.260894 &  -7.669701 &     22.691 $\pm$   0.092 &    23.012 $\pm$   0.148 &    22.148 $\pm$   0.079 &      0.603 \\ 
   112 & 151.364062 &  -7.671057 &     18.964 $\pm$   0.006 &    18.963 $\pm$   0.006 &    19.013 $\pm$   0.007 &      0.980 \\ 
   113 & 151.266236 &  -7.671251 &     20.012 $\pm$   0.011 &    20.081 $\pm$   0.013 &    19.373 $\pm$   0.009 &      0.030 \\ 
   114 & 151.332889 &  -7.670024 &     23.059 $\pm$   0.146 &    22.735 $\pm$   0.129 &    22.382 $\pm$   0.117 &      0.503 \\ 
   115 & 151.273659 &  -7.671074 &     22.677 $\pm$   0.094 &    22.375 $\pm$   0.087 &    21.305 $\pm$   0.040 &      0.657 \\ 
   116 & 151.341860 &  -7.671217 &     22.519 $\pm$   0.088 &    22.171 $\pm$   0.077 &    21.551 $\pm$   0.055 &      0.767 \\ 
   117 & 151.285993 &  -7.671925 &     15.773 $\pm$   0.002 &    15.564 $\pm$   0.001 &    15.699 $\pm$   0.001 &      0.990 \\ 
   118 & 151.276270 &  -7.671113 &     20.778 $\pm$   0.020 &    20.882 $\pm$   0.024 &    20.936 $\pm$   0.030 &      0.887 \\ 
   119 & 151.312979 &  -7.671526 &     22.246 $\pm$   0.070 &    21.934 $\pm$   0.063 &    21.278 $\pm$   0.043 &      0.303 \\ 
   120 & 151.297019 &  -7.672233 &     20.974 $\pm$   0.024 &    20.718 $\pm$   0.022 &    20.059 $\pm$   0.015 &      0.290 \\ 
   121 & 151.306704 &  -7.672126 &     20.899 $\pm$   0.023 &    21.011 $\pm$   0.028 &    20.977 $\pm$   0.033 &      0.953 \\ 
   122 & 151.311146 &  -7.672150 &     21.332 $\pm$   0.032 &    20.858 $\pm$   0.025 &    20.139 $\pm$   0.016 &      0.473 \\ 
   123 & 151.351652 &  -7.672186 &     22.932 $\pm$   0.117 &    22.920 $\pm$   0.140 &    22.294 $\pm$   0.100 &      0.617 \\ 
   124 & 151.330299 &  -7.672412 &     21.568 $\pm$   0.041 &    21.746 $\pm$   0.054 &    21.722 $\pm$   0.066 &      0.653 \\ 
   125 & 151.352805 &  -7.672309 &     23.127 $\pm$   0.138 &    23.050 $\pm$   0.156 &    21.878 $\pm$   0.068 &      0.410 \\ 
   126 & 151.277335 &  -7.672465 &     21.299 $\pm$   0.030 &    21.358 $\pm$   0.036 &    21.479 $\pm$   0.047 &      0.913 \\ 
   127 & 151.365416 &  -7.672503 &     22.410 $\pm$   0.071 &    22.873 $\pm$   0.125 &    22.192 $\pm$   0.080 &      0.570 \\ 
   128 & 151.345551 &  -7.672759 &     22.243 $\pm$   0.068 &    21.877 $\pm$   0.059 &    21.115 $\pm$   0.037 &      0.720 \\ 
   129 & 151.256477 &  -7.673024 &     22.772 $\pm$   0.099 &    22.953 $\pm$   0.140 &    22.568 $\pm$   0.113 &      0.330 \\ 
   130 & 151.281169 &  -7.673152 &     21.612 $\pm$   0.039 &    21.763 $\pm$   0.052 &    21.110 $\pm$   0.035 &      0.010 \\ 
   131 & 151.314551 &  -7.673614 &     15.865 $\pm$   0.002 &    15.971 $\pm$   0.001 &    16.239 $\pm$   0.001 &      0.987 \\ 
   132 & 151.274004 &  -7.673278 &     21.511 $\pm$   0.035 &    21.354 $\pm$   0.036 &    20.618 $\pm$   0.023 &      0.487 \\ 
   133 & 151.354664 &  -7.673037 &     23.149 $\pm$   0.140 &    22.974 $\pm$   0.144 &    22.334 $\pm$   0.101 &      0.503 \\ 
   134 & 151.352389 &  -7.673130 &     22.778 $\pm$   0.102 &    22.880 $\pm$   0.134 &    22.502 $\pm$   0.121 &      0.540 \\ 
   135 & 151.326651 &  -7.673300 &     22.317 $\pm$   0.079 &    22.174 $\pm$   0.079 &    21.449 $\pm$   0.052 &      0.247 \\ 
   136 & 151.369480 &  -7.673133 &     21.416 $\pm$   0.031 &    21.364 $\pm$   0.034 &    21.400 $\pm$   0.040 &      0.577 \\ 
   137 & 151.289044 &  -7.673376 &     22.524 $\pm$   0.086 &    22.556 $\pm$   0.106 &    22.470 $\pm$   0.118 &      0.720 \\ 
   138 & 151.266120 &  -7.674065 &     19.026 $\pm$   0.007 &    19.015 $\pm$   0.006 &    18.308 $\pm$   0.004 &      0.030 \\ 
   139 & 151.337056 &  -7.673562 &     21.432 $\pm$   0.037 &    21.176 $\pm$   0.033 &    20.454 $\pm$   0.022 &      0.430 \\ 
   140 & 151.359055 &  -7.673506 &     22.362 $\pm$   0.069 &    22.472 $\pm$   0.090 &    21.794 $\pm$   0.059 &      0.353 \\ 
   141 & 151.367015 &  -7.673690 &     20.597 $\pm$   0.017 &    20.468 $\pm$   0.017 &    19.825 $\pm$   0.011 &      0.110 \\ 
   142 & 151.293549 &  -7.673611 &     22.467 $\pm$   0.083 &    22.101 $\pm$   0.071 &    21.660 $\pm$   0.058 &      0.850 \\ 
   143 & 151.366040 &  -7.673699 &     21.973 $\pm$   0.049 &    22.489 $\pm$   0.089 &    21.523 $\pm$   0.045 &      0.003 \\ 
   144 & 151.249405 &  -7.673968 &     22.672 $\pm$   0.090 &    22.916 $\pm$   0.130 &    22.337 $\pm$   0.091 &      0.633 \\ 
   145 & 151.325633 &  -7.673949 &     22.054 $\pm$   0.063 &    22.027 $\pm$   0.070 &    21.314 $\pm$   0.046 &      0.093 \\ 
   146 & 151.262186 &  -7.674225 &     21.348 $\pm$   0.030 &    21.479 $\pm$   0.039 &    21.538 $\pm$   0.048 &      0.607 \\ 
   147 & 151.302766 &  -7.674438 &     20.861 $\pm$   0.022 &    20.758 $\pm$   0.023 &    20.862 $\pm$   0.030 &      0.920 \\ 
   148 & 151.314844 &  -7.674505 &     22.489 $\pm$   0.090 &    22.463 $\pm$   0.102 &    21.752 $\pm$   0.067 &      0.227 \\ 
   149 & 151.363192 &  -7.674397 &     22.311 $\pm$   0.066 &    22.239 $\pm$   0.073 &    21.886 $\pm$   0.062 &      0.390 \\ 
   150 & 151.317367 &  -7.674541 &     21.026 $\pm$   0.026 &    21.100 $\pm$   0.031 &    21.135 $\pm$   0.039 &      0.970 \\ 
   151 & 151.362766 &  -7.674793 &     21.451 $\pm$   0.032 &    21.525 $\pm$   0.039 &    21.466 $\pm$   0.044 &      0.510 \\ 
   152 & 151.254749 &  -7.674898 &     22.186 $\pm$   0.060 &    22.385 $\pm$   0.084 &    21.624 $\pm$   0.049 &      0.070 \\ 
   153 & 151.327595 &  -7.674989 &     20.371 $\pm$   0.016 &    20.258 $\pm$   0.016 &    20.292 $\pm$   0.019 &      0.980 \\ 
   154 & 151.259677 &  -7.674900 &     22.669 $\pm$   0.091 &    22.870 $\pm$   0.132 &    22.494 $\pm$   0.109 &      0.613 \\ 
   155 & 151.361331 &  -7.675015 &     22.463 $\pm$   0.075 &    22.637 $\pm$   0.104 &    21.912 $\pm$   0.065 &      0.440 \\ 
   156 & 151.349947 &  -7.674967 &     22.432 $\pm$   0.079 &    22.436 $\pm$   0.093 &    22.741 $\pm$   0.155 &      0.657 \\ 
   157 & 151.350153 &  -7.675072 &     22.560 $\pm$   0.088 &    22.485 $\pm$   0.097 &    22.822 $\pm$   0.167 &      0.663 \\ 
   158 & 151.368538 &  -7.675238 &     20.517 $\pm$   0.016 &    20.292 $\pm$   0.015 &    19.592 $\pm$   0.010 &      0.143 \\ 
   159 & 151.367433 &  -7.675079 &     23.098 $\pm$   0.131 &    22.808 $\pm$   0.118 &    22.513 $\pm$   0.105 &      0.573 \\ 
   160 & 151.334001 &  -7.675384 &     22.218 $\pm$   0.075 &    22.678 $\pm$   0.127 &    21.613 $\pm$   0.062 &      0.157 \\ 
   161 & 151.303809 &  -7.675428 &     21.417 $\pm$   0.035 &    21.547 $\pm$   0.045 &    20.853 $\pm$   0.030 &      0.107 \\ 
   162 & 151.314755 &  -7.675607 &     21.643 $\pm$   0.043 &    21.637 $\pm$   0.049 &    21.669 $\pm$   0.062 &      0.720 \\ 
   163 & 151.335800 &  -7.675907 &     22.019 $\pm$   0.063 &    22.109 $\pm$   0.076 &    22.081 $\pm$   0.094 &      0.433 \\ 
   164 & 151.250024 &  -7.676208 &     19.846 $\pm$   0.010 &    19.759 $\pm$   0.010 &    19.875 $\pm$   0.012 &      0.980 \\ 
   165 & 151.360439 &  -7.676271 &     21.357 $\pm$   0.030 &    21.088 $\pm$   0.028 &    20.453 $\pm$   0.019 &      0.383 \\ 
   166 & 151.253566 &  -7.676282 &     22.077 $\pm$   0.054 &    22.363 $\pm$   0.083 &    21.663 $\pm$   0.051 &      0.057 \\ 
   167 & 151.361841 &  -7.676386 &     22.060 $\pm$   0.053 &    22.226 $\pm$   0.073 &    21.514 $\pm$   0.046 &      0.007 \\ 
   168 & 151.304164 &  -7.676519 &     22.499 $\pm$   0.089 &    21.871 $\pm$   0.060 &    20.885 $\pm$   0.031 &      0.603 \\ 
   169 & 151.346978 &  -7.676711 &     21.910 $\pm$   0.054 &    22.140 $\pm$   0.076 &    21.438 $\pm$   0.051 &      0.100 \\ 
   170 & 151.256373 &  -7.676706 &     17.184 $\pm$   0.003 &    17.120 $\pm$   0.002 &    17.273 $\pm$   0.002 &      0.980 \\ 
   171 & 151.250250 &  -7.676891 &     22.539 $\pm$   0.081 &    22.701 $\pm$   0.109 &    22.082 $\pm$   0.072 &      0.653 \\ 
   172 & 151.335786 &  -7.677083 &     22.316 $\pm$   0.084 &    22.476 $\pm$   0.107 &    22.378 $\pm$   0.126 &      0.617 \\ 
   173 & 151.339845 &  -7.677344 &     20.673 $\pm$   0.021 &    20.542 $\pm$   0.020 &    20.502 $\pm$   0.024 &      0.840 \\ 
   174 & 151.356460 &  -7.677496 &     21.246 $\pm$   0.028 &    21.300 $\pm$   0.034 &    20.345 $\pm$   0.018 &      0.013 \\ 
   175 & 151.268845 &  -7.676588 &     21.431 $\pm$   0.033 &    21.584 $\pm$   0.044 &    20.894 $\pm$   0.028 &      0.067 \\ 
   176 & 151.267016 &  -7.677766 &     22.101 $\pm$   0.057 &    21.991 $\pm$   0.062 &    21.390 $\pm$   0.043 &      0.827 \\ 
   177 & 151.296207 &  -7.677901 &     22.365 $\pm$   0.078 &    22.476 $\pm$   0.101 &    22.625 $\pm$   0.142 &      0.583 \\ 
   178 & 151.330970 &  -7.678244 &     19.153 $\pm$   0.008 &    19.081 $\pm$   0.007 &    19.144 $\pm$   0.008 &      0.980 \\ 
   179 & 151.347130 &  -7.677862 &     22.316 $\pm$   0.078 &    22.388 $\pm$   0.095 &    22.277 $\pm$   0.108 &      0.517 \\ 
   180 & 151.263880 &  -7.678347 &     22.301 $\pm$   0.068 &    22.447 $\pm$   0.092 &    22.261 $\pm$   0.091 &      0.387 \\ 
   181 & 151.267484 &  -7.678372 &     21.525 $\pm$   0.035 &    21.309 $\pm$   0.034 &    20.805 $\pm$   0.026 &      0.963 \\ 
   182 & 151.334637 &  -7.678401 &     21.141 $\pm$   0.032 &    21.136 $\pm$   0.033 &    21.211 $\pm$   0.045 &      0.953 \\ 
   183 & 151.245815 &  -7.678473 &     22.366 $\pm$   0.069 &    22.096 $\pm$   0.063 &    22.587 $\pm$   0.103 &      0.810 \\ 
   184 & 151.373858 &  -7.678664 &     21.669 $\pm$   0.038 &    21.940 $\pm$   0.055 &    20.932 $\pm$   0.027 &      0.047 \\ 
   185 & 151.276513 &  -7.678502 &     23.151 $\pm$   0.148 &    22.857 $\pm$   0.137 &    21.924 $\pm$   0.071 &      0.410 \\ 
   186 & 151.371108 &  -7.678718 &     22.193 $\pm$   0.059 &    22.238 $\pm$   0.071 &    22.288 $\pm$   0.085 &      0.660 \\ 
   187 & 151.321800 &  -7.678765 &     22.337 $\pm$   0.085 &    22.053 $\pm$   0.073 &    21.350 $\pm$   0.050 &      0.503 \\ 
   188 & 151.350838 &  -7.678897 &     22.584 $\pm$   0.094 &    22.586 $\pm$   0.108 &    22.727 $\pm$   0.156 &      0.553 \\ 
   189 & 151.261700 &  -7.678937 &     23.014 $\pm$   0.127 &    22.975 $\pm$   0.147 &    22.083 $\pm$   0.078 &      0.443 \\ 
   190 & 151.261325 &  -7.679177 &     22.039 $\pm$   0.054 &    22.233 $\pm$   0.076 &    21.562 $\pm$   0.049 &      0.047 \\ 
   191 & 151.342946 &  -7.679012 &     20.969 $\pm$   0.027 &    20.953 $\pm$   0.028 &    20.898 $\pm$   0.033 &      0.717 \\ 
   192 & 151.280279 &  -7.679090 &     20.879 $\pm$   0.022 &    20.833 $\pm$   0.024 &    20.846 $\pm$   0.028 &      0.970 \\ 
   193 & 151.255299 &  -7.679441 &     20.785 $\pm$   0.019 &    20.829 $\pm$   0.023 &    20.224 $\pm$   0.016 &      0.147 \\ 
   194 & 151.309224 &  -7.679299 &     22.653 $\pm$   0.106 &    22.544 $\pm$   0.111 &    22.534 $\pm$   0.138 &      0.587 \\ 
   195 & 151.295286 &  -7.679550 &     21.835 $\pm$   0.050 &    21.988 $\pm$   0.066 &    21.184 $\pm$   0.040 &      0.100 \\ 
   196 & 151.293039 &  -7.679548 &     21.864 $\pm$   0.051 &    21.811 $\pm$   0.056 &    21.952 $\pm$   0.077 &      0.893 \\ 
   197 & 151.360820 &  -7.679874 &     20.810 $\pm$   0.020 &    20.660 $\pm$   0.020 &    19.932 $\pm$   0.013 &      0.170 \\ 
   198 & 151.259693 &  -7.679923 &     19.386 $\pm$   0.008 &    19.409 $\pm$   0.008 &    19.419 $\pm$   0.009 &      0.980 \\ 
   199 & 151.333157 &  -7.679936 &     21.922 $\pm$   0.063 &    21.763 $\pm$   0.059 &    20.970 $\pm$   0.037 &      0.863 \\ 
   200 & 151.366801 &  -7.680345 &     20.332 $\pm$   0.014 &    20.518 $\pm$   0.017 &    20.729 $\pm$   0.023 &      0.980 \\ 
   201 & 151.286964 &  -7.680326 &     21.438 $\pm$   0.035 &    21.300 $\pm$   0.035 &    21.324 $\pm$   0.044 &      0.910 \\ 
   202 & 151.339480 &  -7.680313 &     21.915 $\pm$   0.062 &    21.844 $\pm$   0.062 &    20.953 $\pm$   0.036 &      0.153 \\ 
   203 & 151.247231 &  -7.680562 &     20.827 $\pm$   0.020 &    20.642 $\pm$   0.019 &    19.963 $\pm$   0.013 &      0.290 \\ 
   204 & 151.260560 &  -7.680565 &     22.866 $\pm$   0.111 &    22.968 $\pm$   0.146 &    22.135 $\pm$   0.081 &      0.613 \\ 
   205 & 151.372131 &  -7.680614 &     21.426 $\pm$   0.031 &    21.337 $\pm$   0.033 &    20.720 $\pm$   0.023 &      0.503 \\ 
   206 & 151.271851 &  -7.680733 &     22.580 $\pm$   0.089 &    22.672 $\pm$   0.115 &    22.140 $\pm$   0.085 &      0.530 \\ 
   207 & 151.347622 &  -7.680841 &     21.443 $\pm$   0.038 &    21.384 $\pm$   0.040 &    21.433 $\pm$   0.051 &      0.713 \\ 
   208 & 151.293887 &  -7.681030 &     20.914 $\pm$   0.023 &    20.834 $\pm$   0.024 &    20.979 $\pm$   0.033 &      0.973 \\ 
   209 & 151.310541 &  -7.681131 &     21.227 $\pm$   0.032 &    21.400 $\pm$   0.041 &    20.809 $\pm$   0.030 &      0.087 \\ 
   210 & 151.312962 &  -7.681066 &     21.232 $\pm$   0.032 &    21.109 $\pm$   0.032 &    20.483 $\pm$   0.023 &      0.567 \\ 
   211 & 151.279985 &  -7.680948 &     23.144 $\pm$   0.150 &    22.605 $\pm$   0.111 &    21.707 $\pm$   0.060 &      0.670 \\ 
   212 & 151.359038 &  -7.681132 &     20.601 $\pm$   0.017 &    20.414 $\pm$   0.016 &    19.873 $\pm$   0.012 &      0.393 \\ 
   213 & 151.359875 &  -7.681091 &     22.441 $\pm$   0.075 &    22.097 $\pm$   0.066 &    20.835 $\pm$   0.026 &      0.033 \\ 
   214 & 151.273051 &  -7.681457 &     20.722 $\pm$   0.019 &    20.632 $\pm$   0.020 &    20.632 $\pm$   0.023 &      0.977 \\ 
   215 & 151.288900 &  -7.681450 &     21.602 $\pm$   0.040 &    21.524 $\pm$   0.044 &    20.629 $\pm$   0.024 &      0.110 \\ 
   216 & 151.266331 &  -7.682090 &     21.004 $\pm$   0.024 &    21.274 $\pm$   0.034 &    20.680 $\pm$   0.024 &      0.020 \\ 
   217 & 151.293697 &  -7.681644 &     21.361 $\pm$   0.034 &    21.200 $\pm$   0.033 &    20.288 $\pm$   0.019 &      0.253 \\ 
   218 & 151.356450 &  -7.682502 &     14.852 $\pm$   0.002 &    14.891 $\pm$   0.001 &    15.100 $\pm$   0.001 &      0.990 \\ 
   219 & 151.340983 &  -7.682546 &     20.632 $\pm$   0.022 &    20.722 $\pm$   0.024 &    19.932 $\pm$   0.015 &      0.023 \\ 
   220 & 151.371644 &  -7.682445 &     22.180 $\pm$   0.058 &    22.312 $\pm$   0.076 &    21.950 $\pm$   0.064 &      0.477 \\ 
   221 & 151.262285 &  -7.682693 &     20.338 $\pm$   0.014 &    20.358 $\pm$   0.016 &    19.762 $\pm$   0.011 &      0.093 \\ 
   222 & 151.367599 &  -7.682990 &     20.434 $\pm$   0.015 &    20.295 $\pm$   0.015 &    20.337 $\pm$   0.017 &      0.980 \\ 
   223 & 151.284816 &  -7.683067 &     21.089 $\pm$   0.026 &    21.167 $\pm$   0.032 &    20.588 $\pm$   0.023 &      0.070 \\ 
   224 & 151.348426 &  -7.683052 &     21.251 $\pm$   0.033 &    21.211 $\pm$   0.034 &    21.261 $\pm$   0.044 &      0.807 \\ 
   225 & 151.303436 &  -7.683188 &     21.945 $\pm$   0.057 &    22.070 $\pm$   0.073 &    22.000 $\pm$   0.086 &      0.880 \\ 
   226 & 151.332937 &  -7.683336 &     21.307 $\pm$   0.040 &    21.122 $\pm$   0.035 &    21.322 $\pm$   0.054 &      0.967 \\ 
   227 & 151.289037 &  -7.683698 &     17.604 $\pm$   0.004 &    17.643 $\pm$   0.003 &    17.867 $\pm$   0.003 &      0.980 \\ 
   228 & 151.300542 &  -7.682072 &     22.254 $\pm$   0.073 &    22.315 $\pm$   0.089 &    22.453 $\pm$   0.126 &      0.740 \\ 
   229 & 151.359839 &  -7.683399 &     22.537 $\pm$   0.082 &    22.785 $\pm$   0.122 &    22.434 $\pm$   0.104 &      0.630 \\ 
   230 & 151.364360 &  -7.683444 &     22.118 $\pm$   0.056 &    22.222 $\pm$   0.072 &    21.552 $\pm$   0.046 &      0.120 \\ 
   231 & 151.326265 &  -7.683882 &     22.525 $\pm$   0.116 &    22.618 $\pm$   0.132 &    22.044 $\pm$   0.104 &      0.637 \\ 
   232 & 151.268430 &  -7.684048 &     22.210 $\pm$   0.064 &    22.638 $\pm$   0.112 &    21.862 $\pm$   0.066 &      0.617 \\ 
   233 & 151.253442 &  -7.684538 &     16.230 $\pm$   0.002 &    16.237 $\pm$   0.002 &    16.437 $\pm$   0.002 &      0.987 \\ 
   234 & 151.280627 &  -7.684297 &     20.937 $\pm$   0.023 &    20.958 $\pm$   0.027 &    20.445 $\pm$   0.020 &      0.643 \\ 
   235 & 151.287287 &  -7.684718 &     22.581 $\pm$   0.095 &    22.811 $\pm$   0.136 &    22.334 $\pm$   0.109 &      0.610 \\ 
   236 & 151.303361 &  -7.684804 &     20.857 $\pm$   0.024 &    20.687 $\pm$   0.022 &    20.208 $\pm$   0.018 &      0.827 \\ 
   237 & 151.340746 &  -7.684838 &     22.763 $\pm$   0.139 &    22.645 $\pm$   0.133 &    22.251 $\pm$   0.122 &      0.517 \\ 
   238 & 151.261114 &  -7.685246 &     20.245 $\pm$   0.014 &    20.215 $\pm$   0.014 &    19.363 $\pm$   0.009 &      0.030 \\ 
   239 & 151.345250 &  -7.685079 &     19.830 $\pm$   0.012 &    19.798 $\pm$   0.011 &    19.919 $\pm$   0.015 &      0.980 \\ 
   240 & 151.314447 &  -7.685027 &     22.212 $\pm$   0.080 &    21.820 $\pm$   0.062 &    21.312 $\pm$   0.051 &      0.877 \\ 
   241 & 151.259087 &  -7.685399 &     19.771 $\pm$   0.010 &    19.621 $\pm$   0.009 &    19.024 $\pm$   0.007 &      0.197 \\ 
   242 & 151.282284 &  -7.685460 &     19.359 $\pm$   0.008 &    19.405 $\pm$   0.008 &    18.679 $\pm$   0.006 &      0.030 \\ 
   243 & 151.288553 &  -7.685268 &     22.002 $\pm$   0.057 &    21.995 $\pm$   0.066 &    21.197 $\pm$   0.040 &      0.150 \\ 
   244 & 151.346650 &  -7.685291 &     20.768 $\pm$   0.023 &    20.700 $\pm$   0.023 &    20.130 $\pm$   0.017 &      0.697 \\ 
   245 & 151.367819 &  -7.685176 &     22.352 $\pm$   0.067 &    22.124 $\pm$   0.065 &    21.304 $\pm$   0.037 &      0.733 \\ 
   246 & 151.359560 &  -7.685711 &     22.365 $\pm$   0.072 &    22.524 $\pm$   0.097 &    22.048 $\pm$   0.074 &      0.153 \\ 
   247 & 151.270662 &  -7.685867 &     21.364 $\pm$   0.032 &    21.436 $\pm$   0.039 &    21.536 $\pm$   0.050 &      0.800 \\ 
   248 & 151.367590 &  -7.686053 &     22.743 $\pm$   0.095 &    22.459 $\pm$   0.088 &    21.831 $\pm$   0.058 &      0.530 \\ 
   249 & 151.327071 &  -7.686142 &     21.635 $\pm$   0.056 &    21.642 $\pm$   0.057 &    21.692 $\pm$   0.079 &      0.887 \\ 
   250 & 151.365414 &  -7.686268 &     21.568 $\pm$   0.035 &    21.571 $\pm$   0.041 &    21.758 $\pm$   0.055 &      0.913 \\ 
   251 & 151.322612 &  -7.686341 &     21.040 $\pm$   0.033 &    20.934 $\pm$   0.030 &    21.012 $\pm$   0.042 &      0.970 \\ 
   252 & 151.357368 &  -7.686295 &     22.530 $\pm$   0.086 &    22.520 $\pm$   0.098 &    21.973 $\pm$   0.072 &      0.323 \\ 
   253 & 151.276538 &  -7.686764 &     19.249 $\pm$   0.008 &    19.195 $\pm$   0.007 &    18.470 $\pm$   0.005 &      0.030 \\ 
   254 & 151.295298 &  -7.686619 &     20.785 $\pm$   0.022 &    20.609 $\pm$   0.021 &    19.913 $\pm$   0.014 &      0.503 \\ 
   255 & 151.340119 &  -7.686496 &     22.837 $\pm$   0.153 &    22.379 $\pm$   0.106 &    21.674 $\pm$   0.074 &      0.443 \\ 
   256 & 151.323344 &  -7.686769 &     21.551 $\pm$   0.052 &    21.374 $\pm$   0.044 &    21.505 $\pm$   0.066 &      0.927 \\ 
   257 & 151.344492 &  -7.686848 &     20.349 $\pm$   0.018 &    20.322 $\pm$   0.017 &    20.380 $\pm$   0.022 &      0.967 \\ 
   258 & 151.366356 &  -7.687021 &     17.956 $\pm$   0.004 &    17.886 $\pm$   0.003 &    17.920 $\pm$   0.003 &      0.983 \\ 
   259 & 151.297283 &  -7.686937 &     22.072 $\pm$   0.064 &    22.304 $\pm$   0.090 &    21.484 $\pm$   0.054 &      0.053 \\ 
   260 & 151.320185 &  -7.687059 &     20.602 $\pm$   0.023 &    20.441 $\pm$   0.020 &    20.465 $\pm$   0.026 &      0.933 \\ 
   261 & 151.319843 &  -7.687081 &     20.933 $\pm$   0.030 &    20.902 $\pm$   0.029 &    20.959 $\pm$   0.040 &      0.970 \\ 
   262 & 151.268154 &  -7.687218 &     18.165 $\pm$   0.005 &    18.077 $\pm$   0.004 &    18.159 $\pm$   0.004 &      0.980 \\ 
   263 & 151.270001 &  -7.687209 &     22.299 $\pm$   0.070 &    22.405 $\pm$   0.091 &    21.724 $\pm$   0.060 &      0.593 \\ 
   264 & 151.258112 &  -7.687394 &     21.369 $\pm$   0.031 &    21.421 $\pm$   0.037 &    21.402 $\pm$   0.043 &      0.960 \\ 
   265 & 151.284305 &  -7.687488 &     21.241 $\pm$   0.030 &    21.329 $\pm$   0.037 &    21.516 $\pm$   0.053 &      0.943 \\ 
   266 & 151.296123 &  -7.688223 &     22.017 $\pm$   0.061 &    22.145 $\pm$   0.078 &    21.443 $\pm$   0.052 &      0.073 \\ 
   267 & 151.343620 &  -7.688169 &     22.169 $\pm$   0.081 &    21.876 $\pm$   0.066 &    21.236 $\pm$   0.048 &      0.877 \\ 
   268 & 151.252911 &  -7.688447 &     19.399 $\pm$   0.008 &    19.461 $\pm$   0.008 &    19.649 $\pm$   0.010 &      0.980 \\ 
   269 & 151.365343 &  -7.688603 &     21.680 $\pm$   0.038 &    21.532 $\pm$   0.040 &    20.985 $\pm$   0.029 &      0.263 \\ 
   270 & 151.368764 &  -7.688626 &     22.354 $\pm$   0.068 &    22.139 $\pm$   0.066 &    21.039 $\pm$   0.030 &      0.053 \\ 
   271 & 151.326020 &  -7.688863 &     22.551 $\pm$   0.133 &    22.172 $\pm$   0.093 &    22.048 $\pm$   0.113 &      0.683 \\ 
   272 & 151.331011 &  -7.688888 &     22.354 $\pm$   0.112 &    22.274 $\pm$   0.103 &    22.064 $\pm$   0.115 &      0.423 \\ 
   273 & 151.319124 &  -7.688338 &     21.592 $\pm$   0.053 &    21.707 $\pm$   0.060 &    21.870 $\pm$   0.091 &      0.860 \\ 
   274 & 151.288208 &  -7.689074 &     22.957 $\pm$   0.136 &    22.855 $\pm$   0.145 &    22.475 $\pm$   0.127 &      0.533 \\ 
   275 & 151.368217 &  -7.689423 &     20.052 $\pm$   0.011 &    19.871 $\pm$   0.011 &    19.151 $\pm$   0.007 &      0.037 \\ 
   276 & 151.275531 &  -7.689348 &     21.515 $\pm$   0.037 &    21.400 $\pm$   0.038 &    21.450 $\pm$   0.048 &      0.957 \\ 
   277 & 151.312659 &  -7.689321 &     21.445 $\pm$   0.045 &    21.217 $\pm$   0.038 &    20.739 $\pm$   0.032 &      0.820 \\ 
   278 & 151.347170 &  -7.689250 &     22.857 $\pm$   0.141 &    22.720 $\pm$   0.138 &    22.608 $\pm$   0.157 &      0.543 \\ 
   279 & 151.320942 &  -7.689654 &     21.706 $\pm$   0.062 &    21.680 $\pm$   0.059 &    21.804 $\pm$   0.089 &      0.860 \\ 
   280 & 151.320046 &  -7.689734 &     20.813 $\pm$   0.029 &    20.589 $\pm$   0.023 &    19.982 $\pm$   0.018 &      0.850 \\ 
   281 & 151.308173 &  -7.689933 &     20.799 $\pm$   0.025 &    20.682 $\pm$   0.023 &    20.678 $\pm$   0.029 &      0.973 \\ 
   282 & 151.323973 &  -7.689903 &     22.531 $\pm$   0.133 &    22.648 $\pm$   0.144 &    22.300 $\pm$   0.143 &      0.500 \\ 
   283 & 151.324669 &  -7.689989 &     21.854 $\pm$   0.074 &    21.822 $\pm$   0.069 &    21.024 $\pm$   0.045 &      0.063 \\ 
   284 & 151.349218 &  -7.690066 &     21.553 $\pm$   0.043 &    21.466 $\pm$   0.044 &    21.245 $\pm$   0.044 &      0.520 \\ 
   285 & 151.265126 &  -7.690468 &     22.534 $\pm$   0.086 &    22.467 $\pm$   0.096 &    21.883 $\pm$   0.068 &      0.753 \\ 
   286 & 151.363306 &  -7.690592 &     22.481 $\pm$   0.078 &    22.568 $\pm$   0.099 &    22.338 $\pm$   0.093 &      0.507 \\ 
   287 & 151.335920 &  -7.690868 &     20.054 $\pm$   0.016 &    19.891 $\pm$   0.013 &    19.981 $\pm$   0.018 &      0.973 \\ 
   288 & 151.263491 &  -7.690841 &     22.666 $\pm$   0.097 &    22.871 $\pm$   0.137 &    21.732 $\pm$   0.059 &      0.460 \\ 
   289 & 151.323194 &  -7.690958 &     21.338 $\pm$   0.047 &    21.303 $\pm$   0.044 &    21.356 $\pm$   0.061 &      0.720 \\ 
   290 & 151.348446 &  -7.690952 &     22.489 $\pm$   0.100 &    22.017 $\pm$   0.073 &    21.234 $\pm$   0.045 &      0.383 \\ 
   291 & 151.373340 &  -7.691072 &     23.267 $\pm$   0.152 &    23.025 $\pm$   0.143 &    22.163 $\pm$   0.077 &      0.530 \\ 
   292 & 151.346564 &  -7.691132 &     22.794 $\pm$   0.136 &    22.729 $\pm$   0.140 &    21.481 $\pm$   0.058 &      0.457 \\ 
   293 & 151.361872 &  -7.691197 &     22.402 $\pm$   0.074 &    22.310 $\pm$   0.080 &    21.787 $\pm$   0.058 &      0.747 \\ 
   294 & 151.323879 &  -7.691333 &     21.317 $\pm$   0.047 &    21.194 $\pm$   0.040 &    21.228 $\pm$   0.055 &      0.837 \\ 
   295 & 151.351548 &  -7.691377 &     21.481 $\pm$   0.039 &    21.690 $\pm$   0.052 &    21.146 $\pm$   0.039 &      0.853 \\ 
   296 & 151.260031 &  -7.691290 &     22.148 $\pm$   0.061 &    22.151 $\pm$   0.071 &    21.667 $\pm$   0.055 &      0.417 \\ 
   297 & 151.316184 &  -7.691765 &     20.980 $\pm$   0.033 &    20.963 $\pm$   0.032 &    20.828 $\pm$   0.037 &      0.550 \\ 
   298 & 151.315012 &  -7.691748 &     22.087 $\pm$   0.085 &    22.136 $\pm$   0.089 &    21.551 $\pm$   0.070 &      0.703 \\ 
   299 & 151.294988 &  -7.692172 &     21.403 $\pm$   0.037 &    21.429 $\pm$   0.042 &    21.536 $\pm$   0.058 &      0.907 \\ 
   300 & 151.336104 &  -7.692168 &     21.051 $\pm$   0.036 &    21.045 $\pm$   0.034 &    21.234 $\pm$   0.054 &      0.863 \\ 
   301 & 151.350410 &  -7.692361 &     20.229 $\pm$   0.015 &    20.196 $\pm$   0.015 &    19.477 $\pm$   0.010 &      0.030 \\ 
   302 & 151.320005 &  -7.692170 &     22.198 $\pm$   0.101 &    22.532 $\pm$   0.131 &    22.004 $\pm$   0.111 &      0.620 \\ 
   303 & 151.257944 &  -7.692572 &     20.016 $\pm$   0.012 &    20.002 $\pm$   0.012 &    19.343 $\pm$   0.008 &      0.030 \\ 
   304 & 151.355567 &  -7.692290 &     21.364 $\pm$   0.033 &    21.456 $\pm$   0.040 &    21.500 $\pm$   0.050 &      0.787 \\ 
   305 & 151.252378 &  -7.692323 &     22.945 $\pm$   0.119 &    22.845 $\pm$   0.131 &    22.494 $\pm$   0.108 &      0.583 \\ 
   306 & 151.342626 &  -7.692323 &     22.101 $\pm$   0.080 &    22.040 $\pm$   0.078 &    21.909 $\pm$   0.090 &      0.283 \\ 
   307 & 151.272544 &  -7.692590 &     22.119 $\pm$   0.062 &    22.261 $\pm$   0.082 &    21.630 $\pm$   0.056 &      0.483 \\ 
   308 & 151.285830 &  -7.692663 &     21.574 $\pm$   0.041 &    21.456 $\pm$   0.042 &    20.896 $\pm$   0.031 &      0.847 \\ 
   309 & 151.373327 &  -7.692769 &     19.344 $\pm$   0.008 &    19.301 $\pm$   0.007 &    19.024 $\pm$   0.007 &      0.980 \\ 
   310 & 151.340363 &  -7.692691 &     21.651 $\pm$   0.056 &    21.718 $\pm$   0.060 &    21.683 $\pm$   0.076 &      0.590 \\ 
   311 & 151.319174 &  -7.692755 &     21.565 $\pm$   0.058 &    21.504 $\pm$   0.052 &    21.608 $\pm$   0.078 &      0.887 \\ 
   312 & 151.308597 &  -7.692127 &     22.624 $\pm$   0.127 &    22.250 $\pm$   0.095 &    21.639 $\pm$   0.072 &      0.693 \\ 
   313 & 151.364520 &  -7.693166 &     21.662 $\pm$   0.038 &    21.724 $\pm$   0.047 &    21.808 $\pm$   0.058 &      0.927 \\ 
   314 & 151.371245 &  -7.693129 &     23.004 $\pm$   0.119 &    22.479 $\pm$   0.088 &    22.070 $\pm$   0.071 &      0.577 \\ 
   315 & 151.276020 &  -7.693476 &     22.291 $\pm$   0.073 &    22.560 $\pm$   0.108 &    21.371 $\pm$   0.046 &      0.120 \\ 
   316 & 151.336230 &  -7.693407 &     21.340 $\pm$   0.047 &    21.187 $\pm$   0.039 &    20.767 $\pm$   0.036 &      0.850 \\ 
   317 & 151.259918 &  -7.693434 &     22.795 $\pm$   0.107 &    22.789 $\pm$   0.127 &    22.594 $\pm$   0.126 &      0.527 \\ 
   318 & 151.286136 &  -7.693518 &     21.623 $\pm$   0.043 &    21.416 $\pm$   0.041 &    20.754 $\pm$   0.028 &      0.770 \\ 
   319 & 151.329065 &  -7.693539 &     22.281 $\pm$   0.117 &    22.310 $\pm$   0.111 &    21.948 $\pm$   0.110 &      0.557 \\ 
   320 & 151.338186 &  -7.693729 &     18.741 $\pm$   0.007 &    18.696 $\pm$   0.006 &    18.820 $\pm$   0.007 &      0.977 \\ 
   321 & 151.255173 &  -7.694167 &     21.549 $\pm$   0.036 &    21.333 $\pm$   0.035 &    20.487 $\pm$   0.020 &      0.280 \\ 
   322 & 151.332219 &  -7.694101 &     21.215 $\pm$   0.045 &    21.088 $\pm$   0.037 &    21.180 $\pm$   0.054 &      0.967 \\ 
   323 & 151.335455 &  -7.694224 &     19.807 $\pm$   0.014 &    19.792 $\pm$   0.012 &    19.794 $\pm$   0.015 &      0.987 \\ 
   324 & 151.287081 &  -7.694089 &     22.900 $\pm$   0.131 &    22.477 $\pm$   0.104 &    22.138 $\pm$   0.096 &      0.627 \\ 
   325 & 151.363457 &  -7.694276 &     22.778 $\pm$   0.102 &    22.755 $\pm$   0.118 &    22.099 $\pm$   0.075 &      0.653 \\ 
   326 & 151.339622 &  -7.694504 &     19.943 $\pm$   0.015 &    19.795 $\pm$   0.012 &    19.961 $\pm$   0.017 &      0.977 \\ 
   327 & 151.300269 &  -7.694485 &     22.492 $\pm$   0.104 &    22.666 $\pm$   0.133 &    21.809 $\pm$   0.079 &      0.700 \\ 
   328 & 151.260552 &  -7.694518 &     22.429 $\pm$   0.078 &    22.734 $\pm$   0.122 &    22.093 $\pm$   0.081 &      0.717 \\ 
   329 & 151.362246 &  -7.694574 &     21.405 $\pm$   0.032 &    21.184 $\pm$   0.030 &    20.554 $\pm$   0.021 &      0.313 \\ 
   330 & 151.328803 &  -7.694495 &     22.346 $\pm$   0.126 &    22.443 $\pm$   0.127 &    22.142 $\pm$   0.134 &      0.580 \\ 
   331 & 151.333033 &  -7.694749 &     20.979 $\pm$   0.037 &    20.908 $\pm$   0.032 &    21.240 $\pm$   0.057 &      0.967 \\ 
   332 & 151.336603 &  -7.694603 &     22.071 $\pm$   0.088 &    21.938 $\pm$   0.076 &    22.147 $\pm$   0.123 &      0.697 \\ 
   333 & 151.312464 &  -7.694803 &     20.419 $\pm$   0.022 &    20.329 $\pm$   0.019 &    19.900 $\pm$   0.017 &      0.563 \\ 
   334 & 151.273807 &  -7.694957 &     19.544 $\pm$   0.009 &    19.395 $\pm$   0.008 &    19.430 $\pm$   0.009 &      0.980 \\ 
   335 & 151.373928 &  -7.694802 &     22.042 $\pm$   0.048 &    21.978 $\pm$   0.054 &    20.638 $\pm$   0.021 &      0.747 \\ 
   336 & 151.306337 &  -7.694897 &     22.185 $\pm$   0.088 &    22.360 $\pm$   0.106 &    22.103 $\pm$   0.111 &      0.700 \\ 
   337 & 151.322737 &  -7.694925 &     20.994 $\pm$   0.039 &    20.853 $\pm$   0.031 &    20.898 $\pm$   0.044 &      0.947 \\ 
   338 & 151.331191 &  -7.694818 &     22.421 $\pm$   0.132 &    22.122 $\pm$   0.094 &    21.879 $\pm$   0.104 &      0.623 \\ 
   339 & 151.324818 &  -7.694928 &     22.385 $\pm$   0.133 &    22.596 $\pm$   0.146 &    22.041 $\pm$   0.123 &      0.623 \\ 
   340 & 151.369169 &  -7.695147 &     21.706 $\pm$   0.039 &    21.622 $\pm$   0.043 &    20.731 $\pm$   0.023 &      0.093 \\ 
   341 & 151.341724 &  -7.695130 &     22.282 $\pm$   0.095 &    22.070 $\pm$   0.081 &    21.424 $\pm$   0.059 &      0.807 \\ 
   342 & 151.303397 &  -7.695135 &     22.755 $\pm$   0.140 &    22.446 $\pm$   0.113 &    22.038 $\pm$   0.102 &      0.563 \\ 
   343 & 151.328041 &  -7.695308 &     22.172 $\pm$   0.110 &    22.236 $\pm$   0.106 &    21.937 $\pm$   0.112 &      0.670 \\ 
   344 & 151.333939 &  -7.695604 &     18.609 $\pm$   0.007 &    18.446 $\pm$   0.005 &    18.567 $\pm$   0.006 &      0.980 \\ 
   345 & 151.312410 &  -7.695598 &     20.883 $\pm$   0.032 &    20.841 $\pm$   0.029 &    20.996 $\pm$   0.044 &      0.967 \\ 
   346 & 151.359220 &  -7.695643 &     20.386 $\pm$   0.015 &    20.541 $\pm$   0.018 &    20.803 $\pm$   0.026 &      0.973 \\ 
   347 & 151.286297 &  -7.695770 &     22.065 $\pm$   0.063 &    22.655 $\pm$   0.123 &    22.053 $\pm$   0.089 &      0.147 \\ 
   348 & 151.247053 &  -7.695991 &     21.595 $\pm$   0.037 &    22.061 $\pm$   0.064 &    21.720 $\pm$   0.053 &      0.117 \\ 
   349 & 151.357624 &  -7.695851 &     22.463 $\pm$   0.083 &    22.494 $\pm$   0.097 &    22.723 $\pm$   0.140 &      0.673 \\ 
   350 & 151.329217 &  -7.696002 &     20.782 $\pm$   0.033 &    20.793 $\pm$   0.030 &    20.891 $\pm$   0.044 &      0.947 \\ 
   351 & 151.324271 &  -7.695997 &     22.388 $\pm$   0.136 &    22.447 $\pm$   0.129 &    22.116 $\pm$   0.134 &      0.503 \\ 
   352 & 151.308196 &  -7.696131 &     21.751 $\pm$   0.064 &    21.505 $\pm$   0.051 &    20.971 $\pm$   0.042 &      0.960 \\ 
   353 & 151.336070 &  -7.696095 &     22.578 $\pm$   0.140 &    22.519 $\pm$   0.129 &    22.202 $\pm$   0.131 &      0.557 \\ 
   354 & 151.258351 &  -7.696273 &     22.430 $\pm$   0.078 &    22.741 $\pm$   0.121 &    21.776 $\pm$   0.060 &      0.267 \\ 
   355 & 151.251665 &  -7.696463 &     21.878 $\pm$   0.047 &    21.838 $\pm$   0.054 &    21.965 $\pm$   0.068 &      0.787 \\ 
   356 & 151.315426 &  -7.696405 &     22.333 $\pm$   0.121 &    22.157 $\pm$   0.096 &    22.060 $\pm$   0.121 &      0.440 \\ 
   357 & 151.359156 &  -7.696679 &     19.934 $\pm$   0.011 &    19.914 $\pm$   0.011 &    19.288 $\pm$   0.008 &      0.033 \\ 
   358 & 151.284420 &  -7.696906 &     20.183 $\pm$   0.014 &    20.112 $\pm$   0.014 &    19.394 $\pm$   0.009 &      0.030 \\ 
   359 & 151.328585 &  -7.696469 &     22.316 $\pm$   0.127 &    22.438 $\pm$   0.128 &    22.020 $\pm$   0.122 &      0.590 \\ 
   360 & 151.319851 &  -7.696605 &     22.037 $\pm$   0.099 &    22.074 $\pm$   0.092 &    21.806 $\pm$   0.100 &      0.290 \\ 
   361 & 151.327164 &  -7.696537 &     22.340 $\pm$   0.131 &    22.318 $\pm$   0.116 &    22.049 $\pm$   0.127 &      0.583 \\ 
   362 & 151.373333 &  -7.696721 &     20.702 $\pm$   0.018 &    20.625 $\pm$   0.019 &    19.973 $\pm$   0.013 &      0.593 \\ 
   363 & 151.312191 &  -7.697179 &     19.276 $\pm$   0.010 &    19.414 $\pm$   0.010 &    18.831 $\pm$   0.007 &      0.030 \\ 
   364 & 151.346198 &  -7.696916 &     21.730 $\pm$   0.053 &    22.046 $\pm$   0.076 &    22.189 $\pm$   0.109 &      0.810 \\ 
   365 & 151.257165 &  -7.697096 &     20.926 $\pm$   0.022 &    21.090 $\pm$   0.029 &    20.579 $\pm$   0.022 &      0.053 \\ 
   366 & 151.305001 &  -7.697125 &     20.435 $\pm$   0.021 &    20.378 $\pm$   0.019 &    20.472 $\pm$   0.026 &      0.983 \\ 
   367 & 151.332125 &  -7.697119 &     22.165 $\pm$   0.106 &    22.244 $\pm$   0.105 &    21.674 $\pm$   0.086 &      0.353 \\ 
   368 & 151.306325 &  -7.697272 &     22.213 $\pm$   0.095 &    22.394 $\pm$   0.112 &    22.310 $\pm$   0.139 &      0.643 \\ 
   369 & 151.252005 &  -7.697517 &     22.678 $\pm$   0.095 &    22.928 $\pm$   0.141 &    22.764 $\pm$   0.140 &      0.530 \\ 
   370 & 151.302063 &  -7.697437 &     22.823 $\pm$   0.153 &    22.731 $\pm$   0.147 &    22.418 $\pm$   0.146 &      0.553 \\ 
   371 & 151.322524 &  -7.697563 &     22.421 $\pm$   0.145 &    22.146 $\pm$   0.100 &    22.154 $\pm$   0.142 &      0.693 \\ 
   372 & 151.254114 &  -7.697909 &     21.681 $\pm$   0.041 &    21.689 $\pm$   0.047 &    21.204 $\pm$   0.036 &      0.420 \\ 
   373 & 151.346043 &  -7.697935 &     21.793 $\pm$   0.056 &    21.819 $\pm$   0.062 &    21.851 $\pm$   0.080 &      0.847 \\ 
   374 & 151.281412 &  -7.697959 &     22.570 $\pm$   0.097 &    22.370 $\pm$   0.094 &    22.534 $\pm$   0.136 &      0.637 \\ 
   375 & 151.320780 &  -7.697964 &     22.221 $\pm$   0.121 &    22.366 $\pm$   0.122 &    22.082 $\pm$   0.133 &      0.613 \\ 
   376 & 151.348461 &  -7.698383 &     18.989 $\pm$   0.007 &    19.016 $\pm$   0.006 &    19.146 $\pm$   0.008 &      0.957 \\ 
   377 & 151.348542 &  -7.698911 &     22.099 $\pm$   0.070 &    22.276 $\pm$   0.091 &    22.266 $\pm$   0.111 &      0.757 \\ 
   378 & 151.252125 &  -7.698234 &     21.913 $\pm$   0.049 &    21.479 $\pm$   0.040 &    20.781 $\pm$   0.025 &      0.223 \\ 
   379 & 151.319492 &  -7.698194 &     22.393 $\pm$   0.141 &    21.986 $\pm$   0.087 &    21.822 $\pm$   0.105 &      0.570 \\ 
   380 & 151.273481 &  -7.698433 &     22.127 $\pm$   0.064 &    22.363 $\pm$   0.091 &    21.384 $\pm$   0.046 &      0.093 \\ 
   381 & 151.362969 &  -7.698363 &     22.083 $\pm$   0.056 &    22.274 $\pm$   0.077 &    22.345 $\pm$   0.093 &      0.583 \\ 
   382 & 151.330895 &  -7.698589 &     19.965 $\pm$   0.018 &    19.904 $\pm$   0.014 &    20.038 $\pm$   0.021 &      0.983 \\ 
   383 & 151.359200 &  -7.698784 &     18.373 $\pm$   0.005 &    18.277 $\pm$   0.004 &    18.337 $\pm$   0.004 &      0.980 \\ 
   384 & 151.329972 &  -7.698633 &     20.915 $\pm$   0.038 &    20.741 $\pm$   0.029 &    20.924 $\pm$   0.045 &      0.973 \\ 
   385 & 151.299607 &  -7.698781 &     19.723 $\pm$   0.012 &    19.684 $\pm$   0.011 &    19.737 $\pm$   0.014 &      0.987 \\ 
   386 & 151.251186 &  -7.698766 &     21.697 $\pm$   0.041 &    22.111 $\pm$   0.068 &    21.543 $\pm$   0.047 &      0.037 \\ 
   387 & 151.325135 &  -7.698858 &     20.991 $\pm$   0.043 &    20.907 $\pm$   0.034 &    20.940 $\pm$   0.048 &      0.977 \\ 
   388 & 151.323256 &  -7.698921 &     20.996 $\pm$   0.043 &    20.986 $\pm$   0.036 &    21.365 $\pm$   0.071 &      0.963 \\ 
   389 & 151.314202 &  -7.699068 &     22.262 $\pm$   0.119 &    22.553 $\pm$   0.141 &    22.008 $\pm$   0.120 &      0.567 \\ 
   390 & 151.325709 &  -7.699017 &     22.189 $\pm$   0.121 &    22.188 $\pm$   0.105 &    21.912 $\pm$   0.116 &      0.407 \\ 
   391 & 151.306073 &  -7.699145 &     21.824 $\pm$   0.070 &    21.662 $\pm$   0.059 &    21.048 $\pm$   0.045 &      0.693 \\ 
   392 & 151.247462 &  -7.699168 &     22.338 $\pm$   0.070 &    21.702 $\pm$   0.047 &    20.875 $\pm$   0.026 &      0.657 \\ 
   393 & 151.317253 &  -7.699107 &     22.063 $\pm$   0.105 &    22.192 $\pm$   0.104 &    21.618 $\pm$   0.087 &      0.673 \\ 
   394 & 151.272126 &  -7.699621 &     19.609 $\pm$   0.009 &    19.493 $\pm$   0.009 &    18.888 $\pm$   0.006 &      0.057 \\ 
   395 & 151.355799 &  -7.699418 &     21.576 $\pm$   0.040 &    21.630 $\pm$   0.046 &    20.967 $\pm$   0.031 &      0.010 \\ 
   396 & 151.347336 &  -7.699553 &     20.326 $\pm$   0.017 &    20.456 $\pm$   0.019 &    20.660 $\pm$   0.027 &      0.977 \\ 
   397 & 151.327479 &  -7.699556 &     20.473 $\pm$   0.028 &    20.406 $\pm$   0.022 &    20.381 $\pm$   0.029 &      0.957 \\ 
   398 & 151.320201 &  -7.699438 &     22.361 $\pm$   0.142 &    22.138 $\pm$   0.101 &    22.120 $\pm$   0.141 &      0.453 \\ 
   399 & 151.330599 &  -7.699568 &     21.426 $\pm$   0.058 &    21.400 $\pm$   0.051 &    21.519 $\pm$   0.077 &      0.917 \\ 
   400 & 151.328200 &  -7.699600 &     22.245 $\pm$   0.124 &    22.223 $\pm$   0.108 &    22.081 $\pm$   0.134 &      0.690 \\ 
   401 & 151.296238 &  -7.699738 &     21.874 $\pm$   0.062 &    21.951 $\pm$   0.071 &    21.792 $\pm$   0.080 &      0.843 \\ 
   402 & 151.352267 &  -7.699817 &     22.740 $\pm$   0.115 &    22.755 $\pm$   0.134 &    22.271 $\pm$   0.103 &      0.497 \\ 
   403 & 151.314308 &  -7.699843 &     22.341 $\pm$   0.131 &    22.349 $\pm$   0.119 &    22.186 $\pm$   0.143 &      0.647 \\ 
   404 & 151.326162 &  -7.699840 &     22.263 $\pm$   0.131 &    21.899 $\pm$   0.081 &    21.816 $\pm$   0.107 &      0.643 \\ 
   405 & 151.331724 &  -7.699939 &     22.129 $\pm$   0.105 &    22.294 $\pm$   0.111 &    21.917 $\pm$   0.109 &      0.140 \\ 
   406 & 151.289999 &  -7.700241 &     18.637 $\pm$   0.006 &    18.490 $\pm$   0.005 &    18.585 $\pm$   0.005 &      0.980 \\ 
   407 & 151.316998 &  -7.700097 &     22.087 $\pm$   0.110 &    22.264 $\pm$   0.112 &    21.972 $\pm$   0.122 &      0.720 \\ 
   408 & 151.342937 &  -7.700234 &     21.024 $\pm$   0.031 &    20.905 $\pm$   0.029 &    21.132 $\pm$   0.044 &      0.967 \\ 
   409 & 151.272156 &  -7.700569 &     21.529 $\pm$   0.038 &    21.283 $\pm$   0.035 &    20.232 $\pm$   0.018 &      0.153 \\ 
   410 & 151.261602 &  -7.700660 &     22.362 $\pm$   0.075 &    22.300 $\pm$   0.083 &    21.393 $\pm$   0.044 &      0.040 \\ 
   411 & 151.369893 &  -7.700666 &     22.358 $\pm$   0.068 &    22.463 $\pm$   0.088 &    21.704 $\pm$   0.052 &      0.513 \\ 
   412 & 151.328176 &  -7.700684 &     22.226 $\pm$   0.123 &    22.156 $\pm$   0.102 &    21.718 $\pm$   0.096 &      0.533 \\ 
   413 & 151.275534 &  -7.700866 &     22.050 $\pm$   0.060 &    22.003 $\pm$   0.067 &    21.275 $\pm$   0.043 &      0.173 \\ 
   414 & 151.322972 &  -7.700762 &     21.978 $\pm$   0.105 &    22.009 $\pm$   0.091 &    21.633 $\pm$   0.092 &      0.577 \\ 
   415 & 151.327538 &  -7.700787 &     21.264 $\pm$   0.054 &    21.474 $\pm$   0.055 &    21.664 $\pm$   0.092 &      0.780 \\ 
   416 & 151.308105 &  -7.700783 &     22.355 $\pm$   0.121 &    22.345 $\pm$   0.113 &    21.730 $\pm$   0.089 &      0.387 \\ 
   417 & 151.325648 &  -7.700933 &     22.063 $\pm$   0.111 &    22.223 $\pm$   0.110 &    21.770 $\pm$   0.104 &      0.257 \\ 
   418 & 151.248214 &  -7.701415 &     19.346 $\pm$   0.008 &    19.401 $\pm$   0.008 &    18.687 $\pm$   0.005 &      0.030 \\ 
   419 & 151.328414 &  -7.701008 &     22.144 $\pm$   0.114 &    21.946 $\pm$   0.084 &    21.871 $\pm$   0.110 &      0.637 \\ 
   420 & 151.319457 &  -7.701203 &     20.324 $\pm$   0.026 &    20.178 $\pm$   0.019 &    20.133 $\pm$   0.024 &      0.980 \\ 
   421 & 151.310996 &  -7.701164 &     22.328 $\pm$   0.127 &    22.173 $\pm$   0.100 &    22.177 $\pm$   0.140 &      0.613 \\ 
   422 & 151.283283 &  -7.701245 &     21.983 $\pm$   0.060 &    22.035 $\pm$   0.071 &    22.127 $\pm$   0.097 &      0.820 \\ 
   423 & 151.323313 &  -7.701122 &     22.336 $\pm$   0.144 &    22.115 $\pm$   0.101 &    21.732 $\pm$   0.101 &      0.633 \\ 
   424 & 151.363295 &  -7.701256 &     21.394 $\pm$   0.032 &    21.333 $\pm$   0.034 &    20.569 $\pm$   0.021 &      0.230 \\ 
   425 & 151.363546 &  -7.701435 &     21.203 $\pm$   0.027 &    21.156 $\pm$   0.030 &    20.354 $\pm$   0.017 &      0.283 \\ 
   426 & 151.335168 &  -7.701214 &     22.173 $\pm$   0.100 &    22.234 $\pm$   0.101 &    21.714 $\pm$   0.085 &      0.660 \\ 
   427 & 151.279360 &  -7.701466 &     21.203 $\pm$   0.030 &    21.093 $\pm$   0.031 &    21.178 $\pm$   0.041 &      0.970 \\ 
   428 & 151.273762 &  -7.701484 &     22.182 $\pm$   0.068 &    22.581 $\pm$   0.112 &    21.863 $\pm$   0.072 &      0.153 \\ 
   429 & 151.252665 &  -7.701838 &     19.988 $\pm$   0.011 &    19.983 $\pm$   0.012 &    19.275 $\pm$   0.008 &      0.030 \\ 
   430 & 151.316680 &  -7.701629 &     21.621 $\pm$   0.076 &    21.481 $\pm$   0.057 &    21.430 $\pm$   0.077 &      0.763 \\ 
   431 & 151.327164 &  -7.701615 &     22.016 $\pm$   0.104 &    21.635 $\pm$   0.064 &    21.728 $\pm$   0.098 &      0.833 \\ 
   432 & 151.309940 &  -7.701822 &     20.095 $\pm$   0.019 &    20.159 $\pm$   0.017 &    20.364 $\pm$   0.027 &      0.983 \\ 
   433 & 151.335612 &  -7.701715 &     21.778 $\pm$   0.069 &    21.839 $\pm$   0.070 &    22.015 $\pm$   0.111 &      0.837 \\ 
   434 & 151.324651 &  -7.701806 &     22.185 $\pm$   0.127 &    22.371 $\pm$   0.127 &    21.964 $\pm$   0.125 &      0.137 \\ 
   435 & 151.328560 &  -7.701997 &     19.916 $\pm$   0.018 &    19.806 $\pm$   0.013 &    19.865 $\pm$   0.018 &      0.977 \\ 
   436 & 151.320432 &  -7.701872 &     22.290 $\pm$   0.142 &    22.066 $\pm$   0.097 &    21.623 $\pm$   0.093 &      0.767 \\ 
   437 & 151.265922 &  -7.702305 &     20.019 $\pm$   0.012 &    19.949 $\pm$   0.012 &    19.385 $\pm$   0.009 &      0.210 \\ 
   438 & 151.306600 &  -7.702169 &     22.100 $\pm$   0.097 &    22.025 $\pm$   0.085 &    21.614 $\pm$   0.080 &      0.807 \\ 
   439 & 151.301020 &  -7.702141 &     22.554 $\pm$   0.131 &    22.634 $\pm$   0.140 &    22.245 $\pm$   0.132 &      0.583 \\ 
   440 & 151.344768 &  -7.702289 &     20.757 $\pm$   0.024 &    20.783 $\pm$   0.025 &    20.785 $\pm$   0.031 &      0.973 \\ 
   441 & 151.329633 &  -7.702237 &     22.231 $\pm$   0.120 &    22.265 $\pm$   0.110 &    22.062 $\pm$   0.129 &      0.637 \\ 
   442 & 151.323646 &  -7.702524 &     22.111 $\pm$   0.122 &    21.798 $\pm$   0.076 &    21.647 $\pm$   0.095 &      0.043 \\ 
   443 & 151.347269 &  -7.702847 &     14.960 $\pm$   0.002 &    15.096 $\pm$   0.001 &    15.398 $\pm$   0.001 &      0.990 \\ 
   444 & 151.311109 &  -7.702370 &     21.925 $\pm$   0.092 &    21.642 $\pm$   0.063 &    22.081 $\pm$   0.132 &      0.813 \\ 
   445 & 151.337366 &  -7.702503 &     22.398 $\pm$   0.114 &    22.179 $\pm$   0.093 &    21.381 $\pm$   0.060 &      0.207 \\ 
   446 & 151.286097 &  -7.702580 &     21.224 $\pm$   0.032 &    21.162 $\pm$   0.034 &    21.248 $\pm$   0.045 &      0.967 \\ 
   447 & 151.302384 &  -7.702677 &     22.437 $\pm$   0.122 &    22.262 $\pm$   0.102 &    21.648 $\pm$   0.079 &      0.793 \\ 
   448 & 151.324863 &  -7.702792 &     22.382 $\pm$   0.152 &    22.177 $\pm$   0.107 &    22.021 $\pm$   0.133 &      0.670 \\ 
   449 & 151.277485 &  -7.702856 &     22.740 $\pm$   0.113 &    22.338 $\pm$   0.092 &    21.470 $\pm$   0.052 &      0.560 \\ 
   450 & 151.295529 &  -7.702890 &     22.463 $\pm$   0.111 &    22.288 $\pm$   0.098 &    21.791 $\pm$   0.082 &      0.673 \\ 
   451 & 151.304937 &  -7.702882 &     22.507 $\pm$   0.137 &    22.436 $\pm$   0.122 &    22.117 $\pm$   0.125 &      0.613 \\ 
   452 & 151.317898 &  -7.701861 &     22.404 $\pm$   0.155 &    22.097 $\pm$   0.099 &    21.862 $\pm$   0.115 &      0.513 \\ 
   453 & 151.301017 &  -7.703022 &     22.307 $\pm$   0.107 &    22.111 $\pm$   0.088 &    21.653 $\pm$   0.078 &      0.600 \\ 
   454 & 151.322613 &  -7.703321 &     21.847 $\pm$   0.099 &    21.964 $\pm$   0.090 &    21.310 $\pm$   0.071 &      0.007 \\ 
   455 & 151.316110 &  -7.703222 &     22.139 $\pm$   0.125 &    21.845 $\pm$   0.080 &    21.653 $\pm$   0.096 &      0.830 \\ 
   456 & 151.313905 &  -7.703241 &     22.202 $\pm$   0.128 &    22.127 $\pm$   0.102 &    21.886 $\pm$   0.116 &      0.600 \\ 
   457 & 151.285091 &  -7.703389 &     22.075 $\pm$   0.066 &    22.227 $\pm$   0.086 &    22.248 $\pm$   0.111 &      0.763 \\ 
   458 & 151.284836 &  -7.703442 &     22.516 $\pm$   0.098 &    22.628 $\pm$   0.124 &    22.248 $\pm$   0.111 &      0.560 \\ 
   459 & 151.308266 &  -7.703401 &     21.990 $\pm$   0.095 &    22.002 $\pm$   0.086 &    21.805 $\pm$   0.100 &      0.903 \\ 
   460 & 151.299518 &  -7.703576 &     19.792 $\pm$   0.013 &    19.734 $\pm$   0.011 &    19.834 $\pm$   0.015 &      0.990 \\ 
   461 & 151.276134 &  -7.703524 &     21.571 $\pm$   0.041 &    21.317 $\pm$   0.037 &    20.664 $\pm$   0.026 &      0.900 \\ 
   462 & 151.276379 &  -7.703750 &     22.891 $\pm$   0.130 &    22.712 $\pm$   0.128 &    22.218 $\pm$   0.102 &      0.517 \\ 
   463 & 151.246947 &  -7.703882 &     17.620 $\pm$   0.004 &    17.536 $\pm$   0.003 &    17.667 $\pm$   0.003 &      0.983 \\ 
   464 & 151.323540 &  -7.704110 &     21.255 $\pm$   0.058 &    21.357 $\pm$   0.052 &    21.973 $\pm$   0.130 &      0.873 \\ 
   465 & 151.251617 &  -7.703735 &     22.417 $\pm$   0.077 &    22.258 $\pm$   0.078 &    21.623 $\pm$   0.051 &      0.270 \\ 
   466 & 151.254972 &  -7.704224 &     16.926 $\pm$   0.003 &    16.896 $\pm$   0.002 &    17.045 $\pm$   0.002 &      0.983 \\ 
   467 & 151.332834 &  -7.703722 &     22.559 $\pm$   0.148 &    22.436 $\pm$   0.124 &    22.232 $\pm$   0.140 &      0.487 \\ 
   468 & 151.352045 &  -7.703725 &     22.932 $\pm$   0.136 &    22.806 $\pm$   0.140 &    21.707 $\pm$   0.062 &      0.433 \\ 
   469 & 151.311685 &  -7.703855 &     22.242 $\pm$   0.130 &    22.156 $\pm$   0.103 &    21.635 $\pm$   0.091 &      0.610 \\ 
   470 & 151.315987 &  -7.704082 &     19.647 $\pm$   0.016 &    19.572 $\pm$   0.012 &    19.572 $\pm$   0.015 &      0.967 \\ 
   471 & 151.348364 &  -7.704103 &     21.831 $\pm$   0.055 &    21.572 $\pm$   0.048 &    20.745 $\pm$   0.028 &      0.160 \\ 
   472 & 151.321649 &  -7.704082 &     21.116 $\pm$   0.053 &    21.001 $\pm$   0.038 &    21.362 $\pm$   0.076 &      0.967 \\ 
   473 & 151.333879 &  -7.704083 &     20.339 $\pm$   0.022 &    20.379 $\pm$   0.020 &    20.546 $\pm$   0.030 &      0.980 \\ 
   474 & 151.317574 &  -7.704153 &     20.303 $\pm$   0.027 &    20.130 $\pm$   0.018 &    20.295 $\pm$   0.029 &      0.973 \\ 
   475 & 151.337113 &  -7.704118 &     21.785 $\pm$   0.066 &    21.647 $\pm$   0.058 &    20.797 $\pm$   0.035 &      0.400 \\ 
   476 & 151.359413 &  -7.704131 &     22.261 $\pm$   0.068 &    22.245 $\pm$   0.077 &    21.622 $\pm$   0.051 &      0.763 \\ 
   477 & 151.271382 &  -7.704351 &     19.281 $\pm$   0.008 &    19.446 $\pm$   0.008 &    19.691 $\pm$   0.011 &      0.980 \\ 
   478 & 151.292728 &  -7.704382 &     21.392 $\pm$   0.042 &    21.139 $\pm$   0.035 &    20.536 $\pm$   0.026 &      0.820 \\ 
   479 & 151.327253 &  -7.704230 &     22.358 $\pm$   0.142 &    22.265 $\pm$   0.114 &    21.768 $\pm$   0.102 &      0.323 \\ 
   480 & 151.322440 &  -7.704425 &     21.977 $\pm$   0.113 &    22.239 $\pm$   0.116 &    21.634 $\pm$   0.097 &      0.013 \\ 
   481 & 151.326352 &  -7.704480 &     20.548 $\pm$   0.030 &    20.507 $\pm$   0.024 &    20.580 $\pm$   0.035 &      0.970 \\ 
   482 & 151.283620 &  -7.704638 &     20.188 $\pm$   0.015 &    20.039 $\pm$   0.013 &    20.139 $\pm$   0.017 &      0.977 \\ 
   483 & 151.328178 &  -7.704600 &     20.969 $\pm$   0.041 &    20.906 $\pm$   0.033 &    21.222 $\pm$   0.061 &      0.960 \\ 
   484 & 151.349479 &  -7.704730 &     19.535 $\pm$   0.009 &    19.471 $\pm$   0.009 &    19.565 $\pm$   0.011 &      0.980 \\ 
   485 & 151.304933 &  -7.704846 &     18.851 $\pm$   0.008 &    18.758 $\pm$   0.006 &    18.847 $\pm$   0.008 &      0.980 \\ 
   486 & 151.309660 &  -7.704601 &     22.503 $\pm$   0.162 &    22.130 $\pm$   0.100 &    22.114 $\pm$   0.139 &      0.530 \\ 
   487 & 151.310570 &  -7.704814 &     19.651 $\pm$   0.015 &    19.562 $\pm$   0.011 &    19.701 $\pm$   0.017 &      0.987 \\ 
   488 & 151.371502 &  -7.704726 &     21.461 $\pm$   0.032 &    21.552 $\pm$   0.040 &    21.530 $\pm$   0.044 &      0.963 \\ 
   489 & 151.321601 &  -7.704787 &     21.915 $\pm$   0.108 &    22.024 $\pm$   0.096 &    21.554 $\pm$   0.091 &      0.010 \\ 
   490 & 151.248806 &  -7.704858 &     22.246 $\pm$   0.065 &    22.467 $\pm$   0.093 &    22.143 $\pm$   0.080 &      0.693 \\ 
   491 & 151.305550 &  -7.704951 &     19.660 $\pm$   0.014 &    19.510 $\pm$   0.010 &    19.562 $\pm$   0.014 &      0.980 \\ 
   492 & 151.306768 &  -7.704963 &     21.278 $\pm$   0.052 &    21.542 $\pm$   0.057 &    21.926 $\pm$   0.112 &      0.800 \\ 
   493 & 151.320801 &  -7.704950 &     21.788 $\pm$   0.097 &    21.968 $\pm$   0.092 &    21.563 $\pm$   0.092 &      0.180 \\ 
   494 & 151.361555 &  -7.705135 &     22.396 $\pm$   0.075 &    22.901 $\pm$   0.136 &    22.126 $\pm$   0.077 &      0.320 \\ 
   495 & 151.342720 &  -7.705322 &     20.472 $\pm$   0.019 &    20.527 $\pm$   0.021 &    20.569 $\pm$   0.026 &      0.973 \\ 
   496 & 151.321255 &  -7.705276 &     22.105 $\pm$   0.129 &    21.974 $\pm$   0.092 &    21.638 $\pm$   0.099 &      0.480 \\ 
   497 & 151.320649 &  -7.705353 &     21.743 $\pm$   0.094 &    21.610 $\pm$   0.067 &    21.245 $\pm$   0.069 &      0.497 \\ 
   498 & 151.311993 &  -7.705333 &     22.427 $\pm$   0.162 &    22.053 $\pm$   0.097 &    21.808 $\pm$   0.111 &      0.570 \\ 
   499 & 151.315945 &  -7.705398 &     21.907 $\pm$   0.108 &    21.892 $\pm$   0.086 &    21.986 $\pm$   0.136 &      0.840 \\ 
   500 & 151.315913 &  -7.705660 &     21.311 $\pm$   0.065 &    21.189 $\pm$   0.046 &    21.506 $\pm$   0.088 &      0.883 \\ 
   501 & 151.268871 &  -7.705453 &     22.580 $\pm$   0.095 &    22.395 $\pm$   0.094 &    22.661 $\pm$   0.145 &      0.590 \\ 
   502 & 151.348501 &  -7.705438 &     22.297 $\pm$   0.081 &    22.179 $\pm$   0.083 &    21.917 $\pm$   0.079 &      0.573 \\ 
   503 & 151.305699 &  -7.705523 &     22.277 $\pm$   0.123 &    22.060 $\pm$   0.091 &    21.169 $\pm$   0.056 &      0.287 \\ 
   504 & 151.318293 &  -7.705843 &     19.794 $\pm$   0.019 &    19.700 $\pm$   0.013 &    19.626 $\pm$   0.017 &      0.983 \\ 
   505 & 151.251711 &  -7.705778 &     21.945 $\pm$   0.051 &    22.146 $\pm$   0.071 &    21.618 $\pm$   0.051 &      0.443 \\ 
   506 & 151.330685 &  -7.705824 &     21.497 $\pm$   0.060 &    21.306 $\pm$   0.046 &    21.306 $\pm$   0.062 &      0.623 \\ 
   507 & 151.297092 &  -7.705988 &     19.626 $\pm$   0.012 &    19.626 $\pm$   0.011 &    19.817 $\pm$   0.015 &      0.980 \\ 
   508 & 151.315535 &  -7.705773 &     22.157 $\pm$   0.136 &    22.027 $\pm$   0.097 &    21.963 $\pm$   0.134 &      0.357 \\ 
   509 & 151.332722 &  -7.706050 &     20.327 $\pm$   0.022 &    20.188 $\pm$   0.017 &    20.181 $\pm$   0.022 &      0.980 \\ 
   510 & 151.320314 &  -7.706939 &     21.597 $\pm$   0.085 &    21.515 $\pm$   0.062 &    21.674 $\pm$   0.104 &      0.257 \\ 
   511 & 151.320541 &  -7.706052 &     21.165 $\pm$   0.058 &    21.443 $\pm$   0.058 &    21.057 $\pm$   0.059 &      0.017 \\ 
   512 & 151.320198 &  -7.706437 &     21.239 $\pm$   0.063 &    21.284 $\pm$   0.051 &    20.876 $\pm$   0.051 &      0.010 \\ 
   513 & 151.319669 &  -7.706710 &     21.528 $\pm$   0.081 &    21.831 $\pm$   0.083 &    21.238 $\pm$   0.071 &      0.010 \\ 
   514 & 151.249908 &  -7.706121 &     21.511 $\pm$   0.035 &    21.782 $\pm$   0.051 &    22.049 $\pm$   0.073 &      0.820 \\ 
   515 & 151.323881 &  -7.706186 &     21.956 $\pm$   0.107 &    21.797 $\pm$   0.077 &    21.836 $\pm$   0.114 &      0.190 \\ 
   516 & 151.350339 &  -7.706246 &     21.594 $\pm$   0.043 &    21.619 $\pm$   0.049 &    21.675 $\pm$   0.061 &      0.907 \\ 
   517 & 151.251850 &  -7.706354 &     22.255 $\pm$   0.067 &    22.222 $\pm$   0.076 &    21.519 $\pm$   0.047 &      0.220 \\ 
   518 & 151.366777 &  -7.706607 &     18.206 $\pm$   0.005 &    18.102 $\pm$   0.004 &    18.156 $\pm$   0.004 &      0.980 \\ 
   519 & 151.316354 &  -7.706390 &     21.316 $\pm$   0.066 &    21.341 $\pm$   0.053 &    21.691 $\pm$   0.107 &      0.717 \\ 
   520 & 151.305898 &  -7.706558 &     21.655 $\pm$   0.073 &    21.492 $\pm$   0.056 &    21.581 $\pm$   0.084 &      0.920 \\ 
   521 & 151.267596 &  -7.706704 &     21.935 $\pm$   0.054 &    22.042 $\pm$   0.068 &    21.307 $\pm$   0.043 &      0.007 \\ 
   522 & 151.328962 &  -7.706642 &     22.155 $\pm$   0.112 &    22.480 $\pm$   0.133 &    22.204 $\pm$   0.146 &      0.597 \\ 
   523 & 151.307164 &  -7.706764 &     22.170 $\pm$   0.121 &    22.101 $\pm$   0.098 &    21.673 $\pm$   0.094 &      0.450 \\ 
   524 & 151.306582 &  -7.706756 &     22.192 $\pm$   0.122 &    22.146 $\pm$   0.101 &    22.017 $\pm$   0.127 &      0.697 \\ 
   525 & 151.335402 &  -7.706859 &     21.646 $\pm$   0.060 &    21.321 $\pm$   0.044 &    20.778 $\pm$   0.035 &      0.623 \\ 
   526 & 151.360076 &  -7.706883 &     22.092 $\pm$   0.059 &    22.072 $\pm$   0.066 &    21.316 $\pm$   0.038 &      0.050 \\ 
   527 & 151.258026 &  -7.707140 &     19.254 $\pm$   0.008 &    19.270 $\pm$   0.007 &    19.305 $\pm$   0.008 &      0.980 \\ 
   528 & 151.329531 &  -7.707072 &     22.366 $\pm$   0.132 &    22.248 $\pm$   0.108 &    21.952 $\pm$   0.114 &      0.670 \\ 
   529 & 151.311740 &  -7.707222 &     21.724 $\pm$   0.092 &    21.615 $\pm$   0.067 &    21.432 $\pm$   0.082 &      0.617 \\ 
   530 & 151.309670 &  -7.707241 &     21.829 $\pm$   0.097 &    21.904 $\pm$   0.085 &    21.626 $\pm$   0.095 &      0.637 \\ 
   531 & 151.325955 &  -7.707171 &     22.237 $\pm$   0.130 &    22.162 $\pm$   0.104 &    21.947 $\pm$   0.122 &      0.420 \\ 
   532 & 151.295582 &  -7.707436 &     19.909 $\pm$   0.014 &    19.990 $\pm$   0.014 &    20.033 $\pm$   0.018 &      0.980 \\ 
   533 & 151.296794 &  -7.707298 &     22.260 $\pm$   0.103 &    22.236 $\pm$   0.099 &    22.274 $\pm$   0.138 &      0.413 \\ 
   534 & 151.305531 &  -7.707460 &     20.508 $\pm$   0.029 &    20.409 $\pm$   0.022 &    20.417 $\pm$   0.030 &      0.943 \\ 
   535 & 151.288496 &  -7.707524 &     22.234 $\pm$   0.085 &    22.292 $\pm$   0.097 &    21.495 $\pm$   0.061 &      0.090 \\ 
   536 & 151.319606 &  -7.707496 &     21.973 $\pm$   0.120 &    22.005 $\pm$   0.097 &    21.673 $\pm$   0.106 &      0.313 \\ 
   537 & 151.293904 &  -7.707787 &     22.121 $\pm$   0.087 &    22.254 $\pm$   0.098 &    21.726 $\pm$   0.081 &      0.770 \\ 
   538 & 151.310517 &  -7.707706 &     22.243 $\pm$   0.145 &    22.353 $\pm$   0.130 &    21.981 $\pm$   0.134 &      0.620 \\ 
   539 & 151.334250 &  -7.707809 &     21.719 $\pm$   0.065 &    21.529 $\pm$   0.053 &    21.023 $\pm$   0.044 &      0.400 \\ 
   540 & 151.246335 &  -7.707992 &     22.667 $\pm$   0.095 &    22.469 $\pm$   0.093 &    21.199 $\pm$   0.035 &      0.280 \\ 
   541 & 151.357725 &  -7.708212 &     22.198 $\pm$   0.066 &    22.565 $\pm$   0.103 &    22.062 $\pm$   0.076 &      0.097 \\ 
   542 & 151.357899 &  -7.708762 &     20.586 $\pm$   0.018 &    20.401 $\pm$   0.016 &    19.744 $\pm$   0.011 &      0.140 \\ 
   543 & 151.314033 &  -7.708186 &     21.272 $\pm$   0.067 &    21.141 $\pm$   0.045 &    21.577 $\pm$   0.098 &      0.877 \\ 
   544 & 151.311052 &  -7.715053 &     15.698 $\pm$   0.003 &    15.757 $\pm$   0.001 &    17.875 $\pm$   0.006 &      0.670 \\ 
   545 & 151.332571 &  -7.709753 &     19.442 $\pm$   0.011 &    19.427 $\pm$   0.009 &    19.514 $\pm$   0.012 &      0.980 \\ 
   546 & 151.281804 &  -7.709675 &     22.721 $\pm$   0.120 &    22.766 $\pm$   0.142 &    22.288 $\pm$   0.117 &      0.503 \\ 
   547 & 151.325999 &  -7.709627 &     22.340 $\pm$   0.139 &    22.185 $\pm$   0.105 &    22.225 $\pm$   0.153 &      0.560 \\ 
   548 & 151.260685 &  -7.709794 &     21.480 $\pm$   0.036 &    21.615 $\pm$   0.046 &    21.719 $\pm$   0.060 &      0.940 \\ 
   549 & 151.343966 &  -7.709846 &     20.600 $\pm$   0.020 &    20.567 $\pm$   0.021 &    20.603 $\pm$   0.026 &      0.947 \\ 
   550 & 151.331202 &  -7.709776 &     22.535 $\pm$   0.141 &    22.208 $\pm$   0.100 &    21.701 $\pm$   0.085 &      0.723 \\ 
   551 & 151.310457 &  -7.709885 &     22.125 $\pm$   0.142 &    22.046 $\pm$   0.102 &    21.657 $\pm$   0.106 &      0.703 \\ 
   552 & 151.337618 &  -7.708097 &     22.027 $\pm$   0.077 &    22.014 $\pm$   0.078 &    22.093 $\pm$   0.109 &      0.757 \\ 
   553 & 151.345824 &  -7.708264 &     21.207 $\pm$   0.033 &    21.164 $\pm$   0.034 &    20.526 $\pm$   0.024 &      0.357 \\ 
   554 & 151.306409 &  -7.710324 &     21.075 $\pm$   0.051 &    21.038 $\pm$   0.040 &    21.060 $\pm$   0.058 &      0.927 \\ 
   555 & 151.307019 &  -7.710252 &     22.244 $\pm$   0.145 &    22.365 $\pm$   0.131 &    22.042 $\pm$   0.143 &      0.690 \\ 
   556 & 151.346149 &  -7.710286 &     22.764 $\pm$   0.123 &    22.652 $\pm$   0.127 &    22.453 $\pm$   0.129 &      0.500 \\ 
   557 & 151.292474 &  -7.710420 &     21.854 $\pm$   0.069 &    21.722 $\pm$   0.061 &    21.942 $\pm$   0.099 &      0.853 \\ 
   558 & 151.367043 &  -7.710519 &     21.704 $\pm$   0.040 &    21.586 $\pm$   0.042 &    20.624 $\pm$   0.021 &      0.060 \\ 
   559 & 151.288260 &  -7.708276 &     21.909 $\pm$   0.064 &    21.797 $\pm$   0.062 &    21.267 $\pm$   0.050 &      0.540 \\ 
   560 & 151.285034 &  -7.709031 &     21.637 $\pm$   0.048 &    21.456 $\pm$   0.045 &    20.851 $\pm$   0.033 &      0.707 \\ 
   561 & 151.313017 &  -7.710769 &     21.159 $\pm$   0.066 &    21.336 $\pm$   0.056 &    21.111 $\pm$   0.068 &      0.237 \\ 
   562 & 151.313311 &  -7.710843 &     21.223 $\pm$   0.070 &    21.425 $\pm$   0.061 &    21.196 $\pm$   0.074 &      0.027 \\ 
   563 & 151.307700 &  -7.710673 &     22.162 $\pm$   0.140 &    22.472 $\pm$   0.147 &    22.000 $\pm$   0.140 &      0.673 \\ 
   564 & 151.325215 &  -7.710678 &     22.283 $\pm$   0.133 &    21.852 $\pm$   0.078 &    21.633 $\pm$   0.090 &      0.770 \\ 
   565 & 151.348165 &  -7.710949 &     21.010 $\pm$   0.027 &    21.148 $\pm$   0.033 &    20.383 $\pm$   0.020 &      0.020 \\ 
   566 & 151.328881 &  -7.710907 &     21.301 $\pm$   0.050 &    21.203 $\pm$   0.042 &    20.651 $\pm$   0.034 &      0.193 \\ 
   567 & 151.335869 &  -7.710964 &     20.937 $\pm$   0.031 &    20.871 $\pm$   0.029 &    20.901 $\pm$   0.037 &      0.967 \\ 
   568 & 151.302685 &  -7.710904 &     22.415 $\pm$   0.151 &    22.522 $\pm$   0.144 &    22.090 $\pm$   0.137 &      0.567 \\ 
   569 & 151.293317 &  -7.711013 &     21.209 $\pm$   0.041 &    21.197 $\pm$   0.039 &    21.312 $\pm$   0.057 &      0.937 \\ 
   570 & 151.356229 &  -7.710690 &     21.689 $\pm$   0.043 &    21.657 $\pm$   0.047 &    21.818 $\pm$   0.062 &      0.873 \\ 
   571 & 151.264228 &  -7.711702 &     15.744 $\pm$   0.002 &    15.708 $\pm$   0.001 &    15.942 $\pm$   0.001 &      0.993 \\ 
   572 & 151.310587 &  -7.711162 &     21.824 $\pm$   0.115 &    21.715 $\pm$   0.078 &    21.814 $\pm$   0.127 &      0.750 \\ 
   573 & 151.373568 &  -7.711211 &     22.807 $\pm$   0.100 &    23.090 $\pm$   0.152 &    22.642 $\pm$   0.117 &      0.517 \\ 
   574 & 151.330497 &  -7.711193 &     22.597 $\pm$   0.149 &    22.470 $\pm$   0.126 &    22.352 $\pm$   0.154 &      0.503 \\ 
   575 & 151.318865 &  -7.711270 &     21.928 $\pm$   0.117 &    22.153 $\pm$   0.112 &    21.894 $\pm$   0.131 &      0.630 \\ 
   576 & 151.322908 &  -7.711308 &     22.157 $\pm$   0.127 &    21.931 $\pm$   0.086 &    21.904 $\pm$   0.120 &      0.560 \\ 
   577 & 151.372862 &  -7.711679 &     21.134 $\pm$   0.025 &    21.225 $\pm$   0.030 &    21.203 $\pm$   0.034 &      0.967 \\ 
   578 & 151.318116 &  -7.711585 &     21.765 $\pm$   0.103 &    21.794 $\pm$   0.082 &    21.433 $\pm$   0.087 &      0.690 \\ 
   579 & 151.363937 &  -7.711829 &     22.785 $\pm$   0.103 &    22.746 $\pm$   0.116 &    22.393 $\pm$   0.094 &      0.490 \\ 
   580 & 151.308413 &  -7.712013 &     21.593 $\pm$   0.092 &    21.284 $\pm$   0.053 &    21.337 $\pm$   0.081 &      0.850 \\ 
   581 & 151.311789 &  -7.712033 &     21.681 $\pm$   0.107 &    21.904 $\pm$   0.095 &    21.681 $\pm$   0.118 &      0.737 \\ 
   582 & 151.311564 &  -7.712058 &     21.646 $\pm$   0.103 &    21.715 $\pm$   0.080 &    21.640 $\pm$   0.113 &      0.637 \\ 
   583 & 151.326416 &  -7.712171 &     19.966 $\pm$   0.018 &    19.860 $\pm$   0.014 &    19.921 $\pm$   0.019 &      0.987 \\ 
   584 & 151.312719 &  -7.712177 &     21.305 $\pm$   0.078 &    21.269 $\pm$   0.054 &    20.919 $\pm$   0.059 &      0.443 \\ 
   585 & 151.297158 &  -7.712172 &     22.479 $\pm$   0.141 &    22.207 $\pm$   0.102 &    22.152 $\pm$   0.133 &      0.533 \\ 
   586 & 151.299515 &  -7.708376 &     20.411 $\pm$   0.023 &    20.348 $\pm$   0.020 &    20.483 $\pm$   0.029 &      0.980 \\ 
   587 & 151.321114 &  -7.712448 &     21.724 $\pm$   0.090 &    21.495 $\pm$   0.060 &    21.308 $\pm$   0.072 &      0.560 \\ 
   588 & 151.310665 &  -7.712592 &     21.435 $\pm$   0.088 &    21.504 $\pm$   0.067 &    21.110 $\pm$   0.071 &      0.783 \\ 
   589 & 151.315860 &  -7.712770 &     21.241 $\pm$   0.071 &    21.207 $\pm$   0.050 &    21.372 $\pm$   0.086 &      0.313 \\ 
   590 & 151.304599 &  -7.712825 &     21.637 $\pm$   0.086 &    21.550 $\pm$   0.063 &    21.594 $\pm$   0.095 &      0.880 \\ 
   591 & 151.342329 &  -7.713103 &     21.837 $\pm$   0.057 &    22.087 $\pm$   0.078 &    21.440 $\pm$   0.054 &      0.000 \\ 
   592 & 151.303536 &  -7.712947 &     19.704 $\pm$   0.017 &    19.554 $\pm$   0.012 &    19.652 $\pm$   0.017 &      0.980 \\ 
   593 & 151.327193 &  -7.712863 &     21.765 $\pm$   0.077 &    21.383 $\pm$   0.050 &    20.962 $\pm$   0.046 &      0.780 \\ 
   594 & 151.321609 &  -7.712947 &     21.384 $\pm$   0.065 &    21.297 $\pm$   0.050 &    21.953 $\pm$   0.128 &      0.877 \\ 
   595 & 151.321354 &  -7.713330 &     19.014 $\pm$   0.011 &    18.939 $\pm$   0.007 &    19.003 $\pm$   0.010 &      0.970 \\ 
   596 & 151.336414 &  -7.712928 &     22.152 $\pm$   0.084 &    22.253 $\pm$   0.095 &    22.412 $\pm$   0.142 &      0.753 \\ 
   597 & 151.311952 &  -7.713059 &     21.253 $\pm$   0.078 &    21.518 $\pm$   0.069 &    21.073 $\pm$   0.070 &      0.227 \\ 
   598 & 151.324770 &  -7.712999 &     22.091 $\pm$   0.110 &    22.157 $\pm$   0.102 &    21.850 $\pm$   0.108 &      0.573 \\ 
   599 & 151.314617 &  -7.713147 &     21.424 $\pm$   0.086 &    21.615 $\pm$   0.074 &    21.053 $\pm$   0.066 &      0.297 \\ 
   600 & 151.317797 &  -7.713188 &     19.921 $\pm$   0.022 &    19.639 $\pm$   0.013 &    19.760 $\pm$   0.020 &      0.983 \\ 
   601 & 151.252163 &  -7.713460 &     19.676 $\pm$   0.010 &    19.741 $\pm$   0.010 &    19.864 $\pm$   0.012 &      0.983 \\ 
   602 & 151.315106 &  -7.713396 &     20.955 $\pm$   0.057 &    20.532 $\pm$   0.028 &    20.306 $\pm$   0.034 &      0.937 \\ 
   603 & 151.309976 &  -7.713425 &     21.504 $\pm$   0.097 &    21.397 $\pm$   0.062 &    20.647 $\pm$   0.048 &      0.380 \\ 
   604 & 151.309765 &  -7.713519 &     21.316 $\pm$   0.083 &    21.232 $\pm$   0.054 &    20.647 $\pm$   0.048 &      0.407 \\ 
   605 & 151.304910 &  -7.713605 &     21.812 $\pm$   0.105 &    21.776 $\pm$   0.079 &    21.427 $\pm$   0.085 &      0.483 \\ 
   606 & 151.320578 &  -7.713475 &     22.314 $\pm$   0.153 &    22.196 $\pm$   0.112 &    21.911 $\pm$   0.125 &      0.677 \\ 
   607 & 151.306380 &  -7.713680 &     20.556 $\pm$   0.039 &    20.487 $\pm$   0.027 &    20.555 $\pm$   0.041 &      0.903 \\ 
   608 & 151.319818 &  -7.713555 &     22.232 $\pm$   0.146 &    21.841 $\pm$   0.083 &    22.001 $\pm$   0.138 &      0.633 \\ 
   609 & 151.314537 &  -7.713732 &     20.820 $\pm$   0.051 &    20.675 $\pm$   0.032 &    21.016 $\pm$   0.065 &      0.867 \\ 
   610 & 151.303322 &  -7.713710 &     21.962 $\pm$   0.114 &    22.252 $\pm$   0.118 &    21.875 $\pm$   0.122 &      0.803 \\ 
   611 & 151.324410 &  -7.713644 &     22.366 $\pm$   0.140 &    22.314 $\pm$   0.117 &    21.992 $\pm$   0.122 &      0.623 \\ 
   612 & 151.279586 &  -7.713899 &     22.496 $\pm$   0.100 &    22.710 $\pm$   0.137 &    22.380 $\pm$   0.129 &      0.590 \\ 
   613 & 151.318592 &  -7.713904 &     21.866 $\pm$   0.110 &    21.933 $\pm$   0.091 &    21.646 $\pm$   0.103 &      0.470 \\ 
   614 & 151.293102 &  -7.708437 &     21.280 $\pm$   0.042 &    21.564 $\pm$   0.053 &    21.017 $\pm$   0.042 &      0.123 \\ 
   615 & 151.282419 &  -7.714481 &     20.210 $\pm$   0.016 &    20.167 $\pm$   0.016 &    19.401 $\pm$   0.010 &      0.030 \\ 
   616 & 151.281820 &  -7.714644 &     20.684 $\pm$   0.023 &    20.752 $\pm$   0.025 &    19.919 $\pm$   0.015 &      0.027 \\ 
   617 & 151.304992 &  -7.714139 &     21.864 $\pm$   0.114 &    21.993 $\pm$   0.098 &    22.105 $\pm$   0.161 &      0.723 \\ 
   618 & 151.315664 &  -7.714390 &     16.899 $\pm$   0.004 &    16.841 $\pm$   0.002 &    16.909 $\pm$   0.003 &      0.980 \\ 
   619 & 151.338921 &  -7.714294 &     20.089 $\pm$   0.015 &    20.105 $\pm$   0.015 &    20.092 $\pm$   0.017 &      0.983 \\ 
   620 & 151.308685 &  -7.714215 &     21.873 $\pm$   0.138 &    21.556 $\pm$   0.072 &    21.667 $\pm$   0.123 &      0.627 \\ 
   621 & 151.341630 &  -7.714311 &     21.538 $\pm$   0.044 &    21.608 $\pm$   0.051 &    21.782 $\pm$   0.073 &      0.930 \\ 
   622 & 151.256972 &  -7.714472 &     19.718 $\pm$   0.010 &    19.706 $\pm$   0.010 &    19.789 $\pm$   0.012 &      0.977 \\ 
   623 & 151.362298 &  -7.714398 &     22.451 $\pm$   0.078 &    22.627 $\pm$   0.106 &    22.175 $\pm$   0.079 &      0.710 \\ 
   624 & 151.273293 &  -7.714523 &     21.936 $\pm$   0.057 &    22.131 $\pm$   0.078 &    21.421 $\pm$   0.051 &      0.183 \\ 
   625 & 151.303632 &  -7.714524 &     22.285 $\pm$   0.158 &    22.390 $\pm$   0.137 &    21.796 $\pm$   0.118 &      0.547 \\ 
   626 & 151.309478 &  -7.714407 &     21.164 $\pm$   0.076 &    20.502 $\pm$   0.029 &    20.959 $\pm$   0.066 &      0.873 \\ 
   627 & 151.324090 &  -7.714683 &     21.296 $\pm$   0.054 &    21.231 $\pm$   0.044 &    21.083 $\pm$   0.053 &      0.673 \\ 
   628 & 151.306140 &  -7.714641 &     21.558 $\pm$   0.094 &    21.354 $\pm$   0.058 &    20.775 $\pm$   0.051 &      0.670 \\ 
   629 & 151.308882 &  -7.714750 &     21.371 $\pm$   0.092 &    21.200 $\pm$   0.054 &    21.366 $\pm$   0.097 &      0.930 \\ 
   630 & 151.338052 &  -7.714758 &     20.565 $\pm$   0.021 &    20.589 $\pm$   0.022 &    20.668 $\pm$   0.029 &      0.963 \\ 
   631 & 151.257669 &  -7.714910 &     19.803 $\pm$   0.010 &    19.834 $\pm$   0.011 &    19.853 $\pm$   0.012 &      0.977 \\ 
   632 & 151.261987 &  -7.714818 &     22.625 $\pm$   0.098 &    22.385 $\pm$   0.092 &    21.292 $\pm$   0.042 &      0.297 \\ 
   633 & 151.267979 &  -7.714968 &     20.134 $\pm$   0.013 &    20.030 $\pm$   0.013 &    19.520 $\pm$   0.010 &      0.423 \\ 
   634 & 151.354089 &  -7.714963 &     20.376 $\pm$   0.015 &    20.218 $\pm$   0.014 &    19.545 $\pm$   0.010 &      0.467 \\ 
   635 & 151.326222 &  -7.714736 &     22.417 $\pm$   0.136 &    22.407 $\pm$   0.123 &    21.889 $\pm$   0.106 &      0.670 \\ 
   636 & 151.352276 &  -7.714889 &     22.478 $\pm$   0.087 &    22.951 $\pm$   0.151 &    21.852 $\pm$   0.067 &      0.307 \\ 
   637 & 151.290560 &  -7.714905 &     22.516 $\pm$   0.130 &    22.430 $\pm$   0.118 &    22.055 $\pm$   0.113 &      0.633 \\ 
   638 & 151.335657 &  -7.714929 &     22.639 $\pm$   0.129 &    22.551 $\pm$   0.124 &    22.456 $\pm$   0.147 &      0.557 \\ 
   639 & 151.296933 &  -7.715160 &     20.376 $\pm$   0.025 &    20.206 $\pm$   0.018 &    19.795 $\pm$   0.017 &      0.973 \\ 
   640 & 151.296778 &  -7.715468 &     20.031 $\pm$   0.019 &    19.759 $\pm$   0.013 &    19.247 $\pm$   0.011 &      0.893 \\ 
   641 & 151.285650 &  -7.708443 &     21.491 $\pm$   0.043 &    21.549 $\pm$   0.049 &    21.596 $\pm$   0.065 &      0.880 \\ 
   642 & 151.326699 &  -7.715065 &     22.256 $\pm$   0.115 &    22.381 $\pm$   0.119 &    21.987 $\pm$   0.113 &      0.607 \\ 
   643 & 151.305435 &  -7.715123 &     21.969 $\pm$   0.135 &    22.047 $\pm$   0.107 &    21.307 $\pm$   0.083 &      0.447 \\ 
   644 & 151.307407 &  -7.715397 &     20.768 $\pm$   0.054 &    20.794 $\pm$   0.038 &    21.541 $\pm$   0.111 &      0.407 \\ 
   645 & 151.307525 &  -7.715637 &     20.705 $\pm$   0.053 &    20.791 $\pm$   0.038 &    21.317 $\pm$   0.093 &      0.607 \\ 
   646 & 151.316884 &  -7.715229 &     21.938 $\pm$   0.122 &    21.840 $\pm$   0.086 &    21.683 $\pm$   0.110 &      0.543 \\ 
   647 & 151.305829 &  -7.715238 &     21.900 $\pm$   0.131 &    21.843 $\pm$   0.090 &    21.307 $\pm$   0.083 &      0.283 \\ 
   648 & 151.324957 &  -7.708337 &     22.392 $\pm$   0.152 &    22.475 $\pm$   0.139 &    21.920 $\pm$   0.120 &      0.503 \\ 
   649 & 151.343709 &  -7.715278 &     22.559 $\pm$   0.103 &    22.256 $\pm$   0.089 &    21.333 $\pm$   0.047 &      0.237 \\ 
   650 & 151.303508 &  -7.715360 &     21.824 $\pm$   0.109 &    21.926 $\pm$   0.092 &    21.401 $\pm$   0.084 &      0.020 \\ 
   651 & 151.328607 &  -7.715441 &     21.215 $\pm$   0.044 &    21.107 $\pm$   0.037 &    21.202 $\pm$   0.053 &      0.677 \\ 
   652 & 151.322041 &  -7.715259 &     22.261 $\pm$   0.134 &    22.302 $\pm$   0.118 &    22.073 $\pm$   0.136 &      0.697 \\ 
   653 & 151.290716 &  -7.715607 &     20.218 $\pm$   0.019 &    20.102 $\pm$   0.016 &    20.125 $\pm$   0.020 &      0.983 \\ 
   654 & 151.314465 &  -7.715562 &     21.727 $\pm$   0.113 &    21.921 $\pm$   0.097 &    21.690 $\pm$   0.119 &      0.840 \\ 
   655 & 151.278141 &  -7.715700 &     21.372 $\pm$   0.037 &    21.510 $\pm$   0.047 &    21.711 $\pm$   0.070 &      0.830 \\ 
   656 & 151.314030 &  -7.715688 &     20.280 $\pm$   0.034 &    19.909 $\pm$   0.017 &    19.930 $\pm$   0.025 &      0.973 \\ 
   657 & 151.308067 &  -7.708528 &     22.237 $\pm$   0.139 &    22.437 $\pm$   0.137 &    21.995 $\pm$   0.132 &      0.667 \\ 
   658 & 151.304697 &  -7.715937 &     21.650 $\pm$   0.103 &    21.867 $\pm$   0.091 &    21.627 $\pm$   0.110 &      0.247 \\ 
   659 & 151.305061 &  -7.715852 &     21.675 $\pm$   0.107 &    21.951 $\pm$   0.099 &    21.861 $\pm$   0.138 &      0.763 \\ 
   660 & 151.354469 &  -7.715777 &     20.947 $\pm$   0.023 &    21.082 $\pm$   0.029 &    21.280 $\pm$   0.039 &      0.827 \\ 
   661 & 151.308992 &  -7.715743 &     20.861 $\pm$   0.064 &    20.776 $\pm$   0.039 &    20.819 $\pm$   0.062 &      0.713 \\ 
   662 & 151.368999 &  -7.715823 &     21.572 $\pm$   0.035 &    21.442 $\pm$   0.036 &    21.527 $\pm$   0.044 &      0.913 \\ 
   663 & 151.270654 &  -7.715757 &     23.105 $\pm$   0.160 &    22.757 $\pm$   0.135 &    22.511 $\pm$   0.134 &      0.593 \\ 
   664 & 151.351601 &  -7.715997 &     22.013 $\pm$   0.058 &    21.901 $\pm$   0.060 &    21.413 $\pm$   0.046 &      0.573 \\ 
   665 & 151.308028 &  -7.716059 &     21.162 $\pm$   0.082 &    21.395 $\pm$   0.066 &    21.159 $\pm$   0.084 &      0.840 \\ 
   666 & 151.320960 &  -7.716134 &     21.449 $\pm$   0.066 &    21.322 $\pm$   0.049 &    21.384 $\pm$   0.074 &      0.703 \\ 
   667 & 151.315123 &  -7.716152 &     21.773 $\pm$   0.112 &    21.485 $\pm$   0.064 &    21.474 $\pm$   0.094 &      0.610 \\ 
   668 & 151.326125 &  -7.716246 &     20.380 $\pm$   0.023 &    20.406 $\pm$   0.021 &    20.769 $\pm$   0.038 &      0.970 \\ 
   669 & 151.328107 &  -7.716443 &     18.237 $\pm$   0.006 &    18.391 $\pm$   0.005 &    18.722 $\pm$   0.007 &      0.980 \\ 
   670 & 151.308415 &  -7.716535 &     19.727 $\pm$   0.028 &    19.917 $\pm$   0.020 &    20.425 $\pm$   0.045 &      0.343 \\ 
   671 & 151.370150 &  -7.716890 &     16.054 $\pm$   0.002 &    15.881 $\pm$   0.001 &    16.084 $\pm$   0.001 &      0.983 \\ 
   672 & 151.325465 &  -7.716407 &     22.373 $\pm$   0.129 &    22.357 $\pm$   0.116 &    22.149 $\pm$   0.133 &      0.587 \\ 
   673 & 151.318551 &  -7.716449 &     19.971 $\pm$   0.021 &    19.986 $\pm$   0.017 &    20.242 $\pm$   0.028 &      0.977 \\ 
   674 & 151.310229 &  -7.708534 &     22.048 $\pm$   0.125 &    22.220 $\pm$   0.116 &    21.814 $\pm$   0.117 &      0.600 \\ 
   675 & 151.302416 &  -7.716742 &     22.113 $\pm$   0.141 &    22.084 $\pm$   0.106 &    21.864 $\pm$   0.128 &      0.677 \\ 
   676 & 151.285104 &  -7.716982 &     21.338 $\pm$   0.043 &    21.548 $\pm$   0.052 &    20.872 $\pm$   0.037 &      0.017 \\ 
   677 & 151.293649 &  -7.716946 &     22.277 $\pm$   0.119 &    22.113 $\pm$   0.094 &    22.176 $\pm$   0.138 &      0.710 \\ 
   678 & 151.304861 &  -7.717112 &     21.841 $\pm$   0.133 &    22.019 $\pm$   0.109 &    21.323 $\pm$   0.089 &      0.643 \\ 
   679 & 151.354331 &  -7.717236 &     20.817 $\pm$   0.021 &    20.696 $\pm$   0.021 &    19.907 $\pm$   0.013 &      0.060 \\ 
   680 & 151.303392 &  -7.716210 &     22.135 $\pm$   0.148 &    21.970 $\pm$   0.097 &    21.948 $\pm$   0.141 &      0.617 \\ 
   681 & 151.312278 &  -7.717324 &     21.530 $\pm$   0.105 &    21.258 $\pm$   0.057 &    21.176 $\pm$   0.080 &      0.627 \\ 
   682 & 151.325196 &  -7.717217 &     21.470 $\pm$   0.058 &    21.554 $\pm$   0.057 &    21.833 $\pm$   0.099 &      0.847 \\ 
   683 & 151.341450 &  -7.717189 &     22.197 $\pm$   0.076 &    21.997 $\pm$   0.071 &    21.276 $\pm$   0.046 &      0.660 \\ 
   684 & 151.273546 &  -7.717344 &     21.021 $\pm$   0.027 &    20.963 $\pm$   0.028 &    21.226 $\pm$   0.044 &      0.963 \\ 
   685 & 151.315689 &  -7.717265 &     21.094 $\pm$   0.059 &    20.641 $\pm$   0.030 &    21.104 $\pm$   0.065 &      0.920 \\ 
   686 & 151.277968 &  -7.717564 &     21.981 $\pm$   0.064 &    22.226 $\pm$   0.089 &    21.613 $\pm$   0.065 &      0.100 \\ 
   687 & 151.347396 &  -7.708637 &     21.815 $\pm$   0.053 &    21.813 $\pm$   0.059 &    21.983 $\pm$   0.083 &      0.867 \\ 
   688 & 151.359724 &  -7.717484 &     21.888 $\pm$   0.048 &    21.769 $\pm$   0.050 &    20.776 $\pm$   0.024 &      0.267 \\ 
   689 & 151.301060 &  -7.717568 &     21.822 $\pm$   0.105 &    21.714 $\pm$   0.074 &    21.488 $\pm$   0.089 &      0.847 \\ 
   690 & 151.350655 &  -7.717535 &     22.025 $\pm$   0.058 &    22.170 $\pm$   0.076 &    22.531 $\pm$   0.124 &      0.687 \\ 
   691 & 151.253045 &  -7.717650 &     22.332 $\pm$   0.072 &    22.192 $\pm$   0.075 &    21.879 $\pm$   0.066 &      0.820 \\ 
   692 & 151.320002 &  -7.708664 &     21.957 $\pm$   0.117 &    21.672 $\pm$   0.072 &    21.920 $\pm$   0.132 &      0.757 \\ 
   693 & 151.316807 &  -7.717645 &     22.097 $\pm$   0.132 &    22.382 $\pm$   0.136 &    21.707 $\pm$   0.107 &      0.630 \\ 
   694 & 151.323070 &  -7.717803 &     22.100 $\pm$   0.106 &    22.269 $\pm$   0.110 &    21.921 $\pm$   0.111 &      0.697 \\ 
   695 & 151.349461 &  -7.718021 &     20.784 $\pm$   0.021 &    20.662 $\pm$   0.021 &    20.048 $\pm$   0.015 &      0.100 \\ 
   696 & 151.247142 &  -7.718376 &     18.027 $\pm$   0.005 &    17.932 $\pm$   0.003 &    18.003 $\pm$   0.003 &      0.950 \\ 
   697 & 151.295186 &  -7.717971 &     21.991 $\pm$   0.100 &    21.967 $\pm$   0.085 &    21.921 $\pm$   0.115 &      0.660 \\ 
   698 & 151.353509 &  -7.718265 &     20.320 $\pm$   0.015 &    20.182 $\pm$   0.014 &    19.557 $\pm$   0.010 &      0.057 \\ 
   699 & 151.302185 &  -7.718269 &     21.687 $\pm$   0.101 &    21.374 $\pm$   0.058 &    21.467 $\pm$   0.093 &      0.580 \\ 
   700 & 151.285150 &  -7.718594 &     21.095 $\pm$   0.036 &    21.506 $\pm$   0.050 &    20.805 $\pm$   0.035 &      0.020 \\ 
   701 & 151.319811 &  -7.718819 &     19.892 $\pm$   0.018 &    19.882 $\pm$   0.015 &    20.077 $\pm$   0.023 &      0.973 \\ 
   702 & 151.316520 &  -7.718664 &     22.308 $\pm$   0.157 &    22.235 $\pm$   0.118 &    21.854 $\pm$   0.121 &      0.657 \\ 
   703 & 151.280504 &  -7.718829 &     22.621 $\pm$   0.121 &    22.406 $\pm$   0.107 &    21.499 $\pm$   0.061 &      0.617 \\ 
   704 & 151.341358 &  -7.719528 &     20.079 $\pm$   0.014 &    20.325 $\pm$   0.017 &    19.700 $\pm$   0.012 &      0.030 \\ 
   705 & 151.337985 &  -7.719023 &     21.546 $\pm$   0.045 &    21.795 $\pm$   0.061 &    21.201 $\pm$   0.044 &      0.207 \\ 
   706 & 151.304693 &  -7.719277 &     20.666 $\pm$   0.053 &    20.693 $\pm$   0.036 &    20.530 $\pm$   0.047 &      0.147 \\ 
   707 & 151.304544 &  -7.719546 &     20.973 $\pm$   0.068 &    21.464 $\pm$   0.070 &    20.640 $\pm$   0.051 &      0.443 \\ 
   708 & 151.301906 &  -7.719151 &     21.669 $\pm$   0.101 &    21.903 $\pm$   0.093 &    21.530 $\pm$   0.099 &      0.570 \\ 
   709 & 151.279761 &  -7.719354 &     21.761 $\pm$   0.056 &    21.736 $\pm$   0.059 &    22.201 $\pm$   0.115 &      0.757 \\ 
   710 & 151.276100 &  -7.719423 &     22.078 $\pm$   0.069 &    22.410 $\pm$   0.104 &    22.230 $\pm$   0.113 &      0.707 \\ 
   711 & 151.293599 &  -7.719353 &     22.429 $\pm$   0.145 &    22.385 $\pm$   0.123 &    22.308 $\pm$   0.161 &      0.633 \\ 
   712 & 151.312343 &  -7.719853 &     21.730 $\pm$   0.113 &    21.958 $\pm$   0.100 &    21.807 $\pm$   0.132 &      0.870 \\ 
   713 & 151.368201 &  -7.719448 &     22.987 $\pm$   0.120 &    23.134 $\pm$   0.160 &    22.547 $\pm$   0.106 &      0.490 \\ 
   714 & 151.270856 &  -7.719692 &     21.406 $\pm$   0.036 &    21.283 $\pm$   0.037 &    20.549 $\pm$   0.024 &      0.193 \\ 
   715 & 151.343205 &  -7.719571 &     22.840 $\pm$   0.129 &    22.218 $\pm$   0.085 &    21.576 $\pm$   0.057 &      0.703 \\ 
   716 & 151.304782 &  -7.720570 &     20.283 $\pm$   0.041 &    20.654 $\pm$   0.035 &    21.205 $\pm$   0.088 &      0.267 \\ 
   717 & 151.321001 &  -7.719741 &     22.155 $\pm$   0.114 &    22.232 $\pm$   0.107 &    21.624 $\pm$   0.086 &      0.767 \\ 
   718 & 151.278246 &  -7.719843 &     21.968 $\pm$   0.065 &    21.946 $\pm$   0.070 &    21.772 $\pm$   0.076 &      0.800 \\ 
   719 & 151.298208 &  -7.719570 &     22.050 $\pm$   0.122 &    22.042 $\pm$   0.098 &    21.844 $\pm$   0.119 &      0.547 \\ 
   720 & 151.299388 &  -7.719807 &     22.282 $\pm$   0.159 &    22.241 $\pm$   0.120 &    22.050 $\pm$   0.149 &      0.603 \\ 
   721 & 151.311384 &  -7.719987 &     21.415 $\pm$   0.090 &    21.555 $\pm$   0.071 &    21.097 $\pm$   0.072 &      0.813 \\ 
   722 & 151.311402 &  -7.720408 &     21.363 $\pm$   0.085 &    21.204 $\pm$   0.052 &    21.140 $\pm$   0.074 &      0.343 \\ 
   723 & 151.303340 &  -7.719911 &     21.517 $\pm$   0.101 &    21.534 $\pm$   0.071 &    21.095 $\pm$   0.074 &      0.617 \\ 
   724 & 151.303172 &  -7.720111 &     21.440 $\pm$   0.093 &    21.277 $\pm$   0.057 &    20.887 $\pm$   0.060 &      0.540 \\ 
   725 & 151.345791 &  -7.719942 &     22.365 $\pm$   0.082 &    22.176 $\pm$   0.079 &    21.262 $\pm$   0.042 &      0.543 \\ 
   726 & 151.366729 &  -7.720155 &     21.825 $\pm$   0.044 &    21.818 $\pm$   0.051 &    21.719 $\pm$   0.052 &      0.897 \\ 
   727 & 151.313560 &  -7.708701 &     21.323 $\pm$   0.070 &    21.199 $\pm$   0.048 &    21.497 $\pm$   0.091 &      0.883 \\ 
   728 & 151.298362 &  -7.720207 &     21.890 $\pm$   0.109 &    21.837 $\pm$   0.083 &    22.028 $\pm$   0.142 &      0.743 \\ 
   729 & 151.299784 &  -7.720254 &     21.802 $\pm$   0.107 &    21.365 $\pm$   0.056 &    21.488 $\pm$   0.091 &      0.897 \\ 
   730 & 151.283680 &  -7.720410 &     21.667 $\pm$   0.057 &    21.612 $\pm$   0.055 &    21.150 $\pm$   0.047 &      0.610 \\ 
   731 & 151.290751 &  -7.720624 &     18.593 $\pm$   0.007 &    18.607 $\pm$   0.005 &    18.629 $\pm$   0.006 &      0.980 \\ 
   732 & 151.249529 &  -7.720565 &     21.115 $\pm$   0.026 &    21.381 $\pm$   0.036 &    21.331 $\pm$   0.039 &      0.807 \\ 
   733 & 151.300859 &  -7.720522 &     21.502 $\pm$   0.087 &    21.395 $\pm$   0.059 &    21.292 $\pm$   0.079 &      0.813 \\ 
   734 & 151.324928 &  -7.720606 &     20.644 $\pm$   0.027 &    20.703 $\pm$   0.026 &    20.907 $\pm$   0.041 &      0.970 \\ 
   735 & 151.352511 &  -7.708964 &     20.958 $\pm$   0.025 &    21.080 $\pm$   0.030 &    20.127 $\pm$   0.016 &      0.023 \\ 
   736 & 151.356270 &  -7.720708 &     21.120 $\pm$   0.027 &    20.967 $\pm$   0.026 &    20.343 $\pm$   0.017 &      0.487 \\ 
   737 & 151.297384 &  -7.720837 &     22.092 $\pm$   0.127 &    21.844 $\pm$   0.082 &    21.409 $\pm$   0.080 &      0.520 \\ 
   738 & 151.299212 &  -7.720835 &     21.968 $\pm$   0.122 &    22.063 $\pm$   0.104 &    21.887 $\pm$   0.129 &      0.693 \\ 
   739 & 151.353689 &  -7.721090 &     20.444 $\pm$   0.016 &    20.418 $\pm$   0.017 &    20.435 $\pm$   0.019 &      0.977 \\ 
   740 & 151.310336 &  -7.720982 &     21.915 $\pm$   0.142 &    21.893 $\pm$   0.098 &    21.502 $\pm$   0.104 &      0.850 \\ 
   741 & 151.364062 &  -7.721230 &     20.926 $\pm$   0.022 &    21.012 $\pm$   0.026 &    21.005 $\pm$   0.029 &      0.607 \\ 
   742 & 151.291683 &  -7.708815 &     21.395 $\pm$   0.045 &    21.572 $\pm$   0.053 &    20.918 $\pm$   0.038 &      0.227 \\ 
   743 & 151.310971 &  -7.721210 &     21.637 $\pm$   0.105 &    21.463 $\pm$   0.069 &    21.749 $\pm$   0.126 &      0.903 \\ 
   744 & 151.345449 &  -7.721348 &     21.213 $\pm$   0.031 &    21.148 $\pm$   0.032 &    20.568 $\pm$   0.023 &      0.420 \\ 
   745 & 151.292961 &  -7.721451 &     20.349 $\pm$   0.025 &    20.316 $\pm$   0.020 &    20.238 $\pm$   0.026 &      0.890 \\ 
   746 & 151.290029 &  -7.708827 &     20.869 $\pm$   0.028 &    20.762 $\pm$   0.026 &    20.818 $\pm$   0.034 &      0.973 \\ 
   747 & 151.289177 &  -7.721438 &     22.176 $\pm$   0.105 &    22.251 $\pm$   0.105 &    21.596 $\pm$   0.079 &      0.547 \\ 
   748 & 151.301078 &  -7.721490 &     21.713 $\pm$   0.108 &    22.043 $\pm$   0.107 &    21.957 $\pm$   0.149 &      0.613 \\ 
   749 & 151.334978 &  -7.721510 &     22.087 $\pm$   0.074 &    21.730 $\pm$   0.058 &    21.094 $\pm$   0.041 &      0.500 \\ 
   750 & 151.322796 &  -7.708864 &     22.060 $\pm$   0.120 &    21.792 $\pm$   0.077 &    21.579 $\pm$   0.091 &      0.493 \\ 
   751 & 151.369593 &  -7.721642 &     22.517 $\pm$   0.079 &    23.309 $\pm$   0.186 &    22.353 $\pm$   0.089 &      0.447 \\ 
   752 & 151.310232 &  -7.721866 &     20.613 $\pm$   0.044 &    20.315 $\pm$   0.024 &    20.203 $\pm$   0.032 &      0.543 \\ 
   753 & 151.321431 &  -7.722059 &     19.147 $\pm$   0.010 &    19.125 $\pm$   0.008 &    19.194 $\pm$   0.010 &      0.970 \\ 
   754 & 151.324382 &  -7.721958 &     21.396 $\pm$   0.050 &    21.367 $\pm$   0.046 &    21.690 $\pm$   0.082 &      0.897 \\ 
   755 & 151.352931 &  -7.721927 &     21.778 $\pm$   0.046 &    21.870 $\pm$   0.057 &    21.985 $\pm$   0.071 &      0.683 \\ 
   756 & 151.293784 &  -7.722044 &     21.110 $\pm$   0.049 &    20.983 $\pm$   0.036 &    21.269 $\pm$   0.066 &      0.960 \\ 
   757 & 151.310984 &  -7.722055 &     21.598 $\pm$   0.096 &    22.357 $\pm$   0.140 &    21.840 $\pm$   0.131 &      0.627 \\ 
   758 & 151.311271 &  -7.722316 &     20.587 $\pm$   0.039 &    20.372 $\pm$   0.024 &    20.393 $\pm$   0.035 &      0.800 \\ 
   759 & 151.352098 &  -7.722004 &     22.469 $\pm$   0.085 &    22.729 $\pm$   0.123 &    22.703 $\pm$   0.136 &      0.523 \\ 
   760 & 151.315455 &  -7.722085 &     22.056 $\pm$   0.118 &    22.377 $\pm$   0.130 &    22.064 $\pm$   0.140 &      0.717 \\ 
   761 & 151.301521 &  -7.722173 &     21.571 $\pm$   0.099 &    21.571 $\pm$   0.071 &    21.730 $\pm$   0.123 &      0.470 \\ 
   762 & 151.309048 &  -7.722202 &     22.201 $\pm$   0.182 &    21.640 $\pm$   0.078 &    21.438 $\pm$   0.098 &      0.530 \\ 
   763 & 151.309533 &  -7.708930 &     22.132 $\pm$   0.134 &    21.797 $\pm$   0.079 &    22.043 $\pm$   0.144 &      0.660 \\ 
   764 & 151.292383 &  -7.722329 &     22.207 $\pm$   0.122 &    22.116 $\pm$   0.098 &    21.764 $\pm$   0.100 &      0.533 \\ 
   765 & 151.301435 &  -7.722577 &     21.429 $\pm$   0.087 &    21.737 $\pm$   0.083 &    21.546 $\pm$   0.105 &      0.253 \\ 
   766 & 151.290217 &  -7.722455 &     22.306 $\pm$   0.125 &    22.581 $\pm$   0.144 &    22.009 $\pm$   0.119 &      0.653 \\ 
   767 & 151.299716 &  -7.722504 &     21.355 $\pm$   0.076 &    21.588 $\pm$   0.069 &    21.706 $\pm$   0.114 &      0.447 \\ 
   768 & 151.252470 &  -7.722616 &     22.292 $\pm$   0.069 &    22.278 $\pm$   0.080 &    21.283 $\pm$   0.038 &      0.350 \\ 
   769 & 151.313427 &  -7.722496 &     22.250 $\pm$   0.148 &    22.251 $\pm$   0.120 &    21.878 $\pm$   0.124 &      0.590 \\ 
   770 & 151.307477 &  -7.722846 &     20.809 $\pm$   0.056 &    20.639 $\pm$   0.033 &    20.485 $\pm$   0.043 &      0.660 \\ 
   771 & 151.300140 &  -7.722750 &     21.174 $\pm$   0.066 &    21.193 $\pm$   0.049 &    21.441 $\pm$   0.091 &      0.923 \\ 
   772 & 151.320461 &  -7.722646 &     22.541 $\pm$   0.151 &    22.469 $\pm$   0.129 &    21.991 $\pm$   0.115 &      0.547 \\ 
   773 & 151.276712 &  -7.722804 &     19.841 $\pm$   0.012 &    19.724 $\pm$   0.011 &    19.787 $\pm$   0.014 &      0.980 \\ 
   774 & 151.350210 &  -7.723114 &     21.245 $\pm$   0.030 &    21.201 $\pm$   0.032 &    20.542 $\pm$   0.022 &      0.177 \\ 
   775 & 151.316745 &  -7.723029 &     22.216 $\pm$   0.126 &    22.241 $\pm$   0.111 &    22.284 $\pm$   0.162 &      0.473 \\ 
   776 & 151.321924 &  -7.708858 &     22.107 $\pm$   0.128 &    21.807 $\pm$   0.079 &    21.113 $\pm$   0.061 &      0.460 \\ 
   777 & 151.357949 &  -7.723414 &     21.931 $\pm$   0.051 &    22.209 $\pm$   0.074 &    21.485 $\pm$   0.044 &      0.057 \\ 
   778 & 151.310354 &  -7.723449 &     20.589 $\pm$   0.039 &    20.563 $\pm$   0.028 &    20.696 $\pm$   0.045 &      0.897 \\ 
   779 & 151.306970 &  -7.723409 &     21.617 $\pm$   0.108 &    21.822 $\pm$   0.091 &    21.062 $\pm$   0.070 &      0.797 \\ 
   780 & 151.301396 &  -7.723581 &     21.224 $\pm$   0.073 &    21.225 $\pm$   0.052 &    21.706 $\pm$   0.121 &      0.253 \\ 
   781 & 151.269285 &  -7.723744 &     20.919 $\pm$   0.025 &    20.996 $\pm$   0.029 &    21.015 $\pm$   0.036 &      0.977 \\ 
   782 & 151.297003 &  -7.723626 &     22.113 $\pm$   0.135 &    21.808 $\pm$   0.081 &    21.747 $\pm$   0.111 &      0.570 \\ 
   783 & 151.315524 &  -7.723699 &     21.998 $\pm$   0.106 &    22.127 $\pm$   0.101 &    21.626 $\pm$   0.090 &      0.480 \\ 
   784 & 151.344458 &  -7.723778 &     20.811 $\pm$   0.022 &    20.663 $\pm$   0.021 &    20.694 $\pm$   0.026 &      0.927 \\ 
   785 & 151.321992 &  -7.723908 &     19.169 $\pm$   0.009 &    19.267 $\pm$   0.008 &    19.603 $\pm$   0.013 &      0.980 \\ 
   786 & 151.254235 &  -7.724010 &     21.911 $\pm$   0.050 &    21.746 $\pm$   0.051 &    20.909 $\pm$   0.029 &      0.243 \\ 
   787 & 151.254576 &  -7.724088 &     22.051 $\pm$   0.057 &    22.008 $\pm$   0.064 &    20.918 $\pm$   0.029 &      0.127 \\ 
   788 & 151.297507 &  -7.723888 &     21.883 $\pm$   0.112 &    21.937 $\pm$   0.092 &    21.921 $\pm$   0.133 &      0.453 \\ 
   789 & 151.296509 &  -7.724062 &     22.079 $\pm$   0.130 &    21.957 $\pm$   0.092 &    21.903 $\pm$   0.128 &      0.610 \\ 
   790 & 151.308244 &  -7.724193 &     21.816 $\pm$   0.117 &    21.447 $\pm$   0.062 &    21.320 $\pm$   0.081 &      0.623 \\ 
   791 & 151.307107 &  -7.724103 &     21.350 $\pm$   0.082 &    21.253 $\pm$   0.054 &    21.048 $\pm$   0.067 &      0.360 \\ 
   792 & 151.325989 &  -7.724280 &     21.104 $\pm$   0.036 &    21.040 $\pm$   0.034 &    20.557 $\pm$   0.028 &      0.453 \\ 
   793 & 151.319186 &  -7.724375 &     20.064 $\pm$   0.019 &    19.997 $\pm$   0.015 &    20.151 $\pm$   0.022 &      0.983 \\ 
   794 & 151.337467 &  -7.709098 &     20.547 $\pm$   0.022 &    20.486 $\pm$   0.021 &    19.842 $\pm$   0.015 &      0.043 \\ 
   795 & 151.291306 &  -7.724493 &     20.147 $\pm$   0.022 &    20.160 $\pm$   0.018 &    20.370 $\pm$   0.029 &      0.977 \\ 
   796 & 151.306667 &  -7.724572 &     21.565 $\pm$   0.096 &    21.275 $\pm$   0.054 &    21.528 $\pm$   0.101 &      0.533 \\ 
   797 & 151.309319 &  -7.724569 &     21.793 $\pm$   0.107 &    22.018 $\pm$   0.100 &    22.032 $\pm$   0.150 &      0.540 \\ 
   798 & 151.271193 &  -7.724704 &     21.749 $\pm$   0.050 &    21.352 $\pm$   0.040 &    20.662 $\pm$   0.027 &      0.470 \\ 
   799 & 151.349362 &  -7.724848 &     19.174 $\pm$   0.007 &    19.209 $\pm$   0.007 &    19.428 $\pm$   0.009 &      0.980 \\ 
   800 & 151.285173 &  -7.724690 &     22.521 $\pm$   0.135 &    22.265 $\pm$   0.103 &    21.170 $\pm$   0.052 &      0.430 \\ 
   801 & 151.323378 &  -7.724665 &     22.412 $\pm$   0.119 &    22.404 $\pm$   0.116 &    22.285 $\pm$   0.138 &      0.570 \\ 
   802 & 151.305608 &  -7.724747 &     21.908 $\pm$   0.133 &    21.420 $\pm$   0.062 &    21.418 $\pm$   0.093 &      0.300 \\ 
   803 & 151.347548 &  -7.724893 &     21.365 $\pm$   0.034 &    21.456 $\pm$   0.041 &    21.547 $\pm$   0.052 &      0.943 \\ 
   804 & 151.303627 &  -7.724826 &     21.727 $\pm$   0.115 &    20.523 $\pm$   0.029 &    20.738 $\pm$   0.051 &      0.763 \\ 
   805 & 151.305088 &  -7.724965 &     21.974 $\pm$   0.142 &    21.444 $\pm$   0.064 &    22.253 $\pm$   0.199 &      0.340 \\ 
   806 & 151.338528 &  -7.724898 &     22.242 $\pm$   0.078 &    22.253 $\pm$   0.088 &    21.577 $\pm$   0.058 &      0.623 \\ 
   807 & 151.296601 &  -7.724865 &     22.118 $\pm$   0.135 &    22.065 $\pm$   0.102 &    21.873 $\pm$   0.126 &      0.587 \\ 
   808 & 151.271857 &  -7.725075 &     21.627 $\pm$   0.046 &    21.693 $\pm$   0.054 &    21.813 $\pm$   0.076 &      0.930 \\ 
   809 & 151.303543 &  -7.725373 &     21.351 $\pm$   0.081 &    21.267 $\pm$   0.054 &    21.064 $\pm$   0.067 &      0.037 \\ 
   810 & 151.310082 &  -7.724590 &     21.311 $\pm$   0.068 &    21.068 $\pm$   0.042 &    21.480 $\pm$   0.088 &      0.923 \\ 
   811 & 151.304134 &  -7.725023 &     22.074 $\pm$   0.156 &    21.647 $\pm$   0.076 &    21.432 $\pm$   0.094 &      0.410 \\ 
   812 & 151.262700 &  -7.709303 &     20.054 $\pm$   0.012 &    20.057 $\pm$   0.013 &    19.485 $\pm$   0.010 &      0.103 \\ 
   813 & 151.304646 &  -7.725292 &     21.885 $\pm$   0.129 &    21.505 $\pm$   0.067 &    21.426 $\pm$   0.093 &      0.377 \\ 
   814 & 151.306431 &  -7.725404 &     21.157 $\pm$   0.065 &    21.213 $\pm$   0.050 &    21.753 $\pm$   0.121 &      0.577 \\ 
   815 & 151.270901 &  -7.725450 &     20.926 $\pm$   0.026 &    21.045 $\pm$   0.031 &    20.163 $\pm$   0.018 &      0.023 \\ 
   816 & 151.346148 &  -7.725455 &     20.057 $\pm$   0.013 &    20.170 $\pm$   0.014 &    20.443 $\pm$   0.020 &      0.980 \\ 
   817 & 151.295017 &  -7.725440 &     22.055 $\pm$   0.123 &    22.042 $\pm$   0.098 &    21.823 $\pm$   0.116 &      0.540 \\ 
   818 & 151.299134 &  -7.725539 &     20.844 $\pm$   0.049 &    20.750 $\pm$   0.033 &    21.023 $\pm$   0.061 &      0.940 \\ 
   819 & 151.314865 &  -7.725458 &     22.445 $\pm$   0.152 &    22.344 $\pm$   0.121 &    22.134 $\pm$   0.139 &      0.600 \\ 
   820 & 151.298338 &  -7.725615 &     21.464 $\pm$   0.081 &    21.475 $\pm$   0.062 &    21.678 $\pm$   0.109 &      0.410 \\ 
   821 & 151.313166 &  -7.725721 &     20.163 $\pm$   0.023 &    20.083 $\pm$   0.017 &    20.266 $\pm$   0.027 &      0.983 \\ 
   822 & 151.286800 &  -7.725788 &     22.033 $\pm$   0.094 &    22.130 $\pm$   0.095 &    21.668 $\pm$   0.085 &      0.187 \\ 
   823 & 151.305612 &  -7.709109 &     21.765 $\pm$   0.087 &    21.373 $\pm$   0.052 &    21.606 $\pm$   0.090 &      0.880 \\ 
   824 & 151.306577 &  -7.726035 &     20.974 $\pm$   0.054 &    20.580 $\pm$   0.029 &    20.822 $\pm$   0.051 &      0.950 \\ 
   825 & 151.309925 &  -7.726097 &     19.607 $\pm$   0.017 &    19.723 $\pm$   0.014 &    19.789 $\pm$   0.019 &      0.647 \\ 
   826 & 151.363509 &  -7.726113 &     20.827 $\pm$   0.020 &    20.987 $\pm$   0.026 &    20.670 $\pm$   0.022 &      0.060 \\ 
   827 & 151.322333 &  -7.725977 &     22.489 $\pm$   0.128 &    22.518 $\pm$   0.128 &    22.161 $\pm$   0.123 &      0.620 \\ 
   828 & 151.313797 &  -7.726110 &     21.381 $\pm$   0.060 &    21.384 $\pm$   0.051 &    21.419 $\pm$   0.074 &      0.920 \\ 
   829 & 151.275661 &  -7.726204 &     21.154 $\pm$   0.033 &    21.128 $\pm$   0.034 &    21.219 $\pm$   0.047 &      0.947 \\ 
   830 & 151.257121 &  -7.726210 &     22.072 $\pm$   0.059 &    22.393 $\pm$   0.091 &    21.500 $\pm$   0.049 &      0.077 \\ 
   831 & 151.282810 &  -7.726235 &     22.395 $\pm$   0.116 &    22.558 $\pm$   0.132 &    22.436 $\pm$   0.159 &      0.507 \\ 
   832 & 151.294760 &  -7.726360 &     20.789 $\pm$   0.041 &    20.689 $\pm$   0.030 &    20.890 $\pm$   0.050 &      0.973 \\ 
   833 & 151.356572 &  -7.709219 &     20.622 $\pm$   0.018 &    20.616 $\pm$   0.019 &    20.773 $\pm$   0.025 &      0.970 \\ 
   834 & 151.247227 &  -7.726555 &     21.338 $\pm$   0.030 &    21.388 $\pm$   0.036 &    21.628 $\pm$   0.049 &      0.940 \\ 
   835 & 151.294306 &  -7.725920 &     22.148 $\pm$   0.131 &    22.116 $\pm$   0.103 &    21.887 $\pm$   0.122 &      0.640 \\ 
   836 & 151.367557 &  -7.727062 &     19.155 $\pm$   0.007 &    19.275 $\pm$   0.007 &    18.654 $\pm$   0.005 &      0.030 \\ 
   837 & 151.298807 &  -7.726676 &     19.172 $\pm$   0.013 &    19.113 $\pm$   0.009 &    19.120 $\pm$   0.012 &      0.980 \\ 
   838 & 151.350193 &  -7.727104 &     20.556 $\pm$   0.018 &    20.264 $\pm$   0.015 &    19.464 $\pm$   0.009 &      0.030 \\ 
   839 & 151.258871 &  -7.726869 &     20.715 $\pm$   0.020 &    20.679 $\pm$   0.021 &    19.985 $\pm$   0.014 &      0.377 \\ 
   840 & 151.345650 &  -7.726750 &     22.559 $\pm$   0.095 &    22.592 $\pm$   0.112 &    21.764 $\pm$   0.063 &      0.610 \\ 
   841 & 151.358226 &  -7.726774 &     22.218 $\pm$   0.065 &    22.066 $\pm$   0.065 &    21.524 $\pm$   0.045 &      0.787 \\ 
   842 & 151.304339 &  -7.727270 &     20.057 $\pm$   0.026 &    20.018 $\pm$   0.018 &    20.101 $\pm$   0.027 &      0.693 \\ 
   843 & 151.295529 &  -7.727183 &     21.968 $\pm$   0.117 &    22.065 $\pm$   0.102 &    21.906 $\pm$   0.127 &      0.503 \\ 
   844 & 151.305624 &  -7.726993 &     21.930 $\pm$   0.121 &    21.655 $\pm$   0.072 &    22.063 $\pm$   0.154 &      0.787 \\ 
   845 & 151.328182 &  -7.727262 &     21.317 $\pm$   0.040 &    21.342 $\pm$   0.042 &    21.610 $\pm$   0.067 &      0.943 \\ 
   846 & 151.340621 &  -7.727366 &     22.154 $\pm$   0.069 &    21.973 $\pm$   0.067 &    21.212 $\pm$   0.041 &      0.107 \\ 
   847 & 151.284721 &  -7.727471 &     22.511 $\pm$   0.138 &    22.509 $\pm$   0.130 &    21.968 $\pm$   0.109 &      0.623 \\ 
   848 & 151.348168 &  -7.727528 &     22.048 $\pm$   0.060 &    21.810 $\pm$   0.055 &    21.030 $\pm$   0.033 &      0.410 \\ 
   849 & 151.355717 &  -7.727538 &     21.860 $\pm$   0.049 &    21.673 $\pm$   0.047 &    21.070 $\pm$   0.031 &      0.177 \\ 
   850 & 151.300151 &  -7.727604 &     21.433 $\pm$   0.081 &    21.563 $\pm$   0.068 &    20.931 $\pm$   0.056 &      0.090 \\ 
   851 & 151.301298 &  -7.727700 &     21.565 $\pm$   0.091 &    21.771 $\pm$   0.077 &    21.744 $\pm$   0.118 &      0.260 \\ 
   852 & 151.303877 &  -7.727749 &     20.208 $\pm$   0.028 &    20.120 $\pm$   0.019 &    20.493 $\pm$   0.037 &      0.973 \\ 
   853 & 151.302065 &  -7.727679 &     22.100 $\pm$   0.144 &    22.010 $\pm$   0.100 &    21.639 $\pm$   0.107 &      0.550 \\ 
   854 & 151.297372 &  -7.727948 &     21.471 $\pm$   0.080 &    21.246 $\pm$   0.050 &    21.452 $\pm$   0.087 &      0.293 \\ 
   855 & 151.280767 &  -7.728156 &     19.930 $\pm$   0.015 &    19.905 $\pm$   0.013 &    19.931 $\pm$   0.017 &      0.977 \\ 
   856 & 151.304744 &  -7.728187 &     21.812 $\pm$   0.106 &    22.220 $\pm$   0.118 &    22.143 $\pm$   0.163 &      0.680 \\ 
   857 & 151.301781 &  -7.728112 &     21.826 $\pm$   0.112 &    21.683 $\pm$   0.075 &    21.945 $\pm$   0.139 &      0.517 \\ 
   858 & 151.355933 &  -7.728256 &     22.384 $\pm$   0.077 &    22.869 $\pm$   0.135 &    22.076 $\pm$   0.075 &      0.233 \\ 
   859 & 151.355524 &  -7.728409 &     21.789 $\pm$   0.046 &    22.358 $\pm$   0.086 &    21.741 $\pm$   0.056 &      0.000 \\ 
   860 & 151.347252 &  -7.728229 &     21.591 $\pm$   0.040 &    21.595 $\pm$   0.046 &    20.943 $\pm$   0.030 &      0.030 \\ 
   861 & 151.267204 &  -7.728294 &     22.606 $\pm$   0.103 &    22.459 $\pm$   0.105 &    21.513 $\pm$   0.056 &      0.550 \\ 
   862 & 151.288106 &  -7.709369 &     21.214 $\pm$   0.036 &    21.210 $\pm$   0.037 &    21.287 $\pm$   0.051 &      0.970 \\ 
   863 & 151.342812 &  -7.728376 &     21.558 $\pm$   0.041 &    21.459 $\pm$   0.042 &    20.761 $\pm$   0.027 &      0.463 \\ 
   864 & 151.343151 &  -7.728460 &     21.127 $\pm$   0.028 &    20.943 $\pm$   0.027 &    20.321 $\pm$   0.019 &      0.703 \\ 
   865 & 151.296115 &  -7.728422 &     21.573 $\pm$   0.084 &    21.725 $\pm$   0.075 &    21.754 $\pm$   0.113 &      0.563 \\ 
   866 & 151.305228 &  -7.728408 &     21.393 $\pm$   0.072 &    21.215 $\pm$   0.048 &    21.164 $\pm$   0.066 &      0.940 \\ 
   867 & 151.308943 &  -7.728381 &     22.014 $\pm$   0.112 &    22.104 $\pm$   0.101 &    21.741 $\pm$   0.103 &      0.687 \\ 
   868 & 151.365622 &  -7.728289 &     20.409 $\pm$   0.015 &    20.501 $\pm$   0.017 &    20.561 $\pm$   0.020 &      0.977 \\ 
   869 & 151.295103 &  -7.728813 &     18.864 $\pm$   0.010 &    18.774 $\pm$   0.007 &    18.932 $\pm$   0.009 &      0.980 \\ 
   870 & 151.344749 &  -7.728658 &     22.827 $\pm$   0.121 &    22.701 $\pm$   0.123 &    21.963 $\pm$   0.075 &      0.477 \\ 
   871 & 151.290658 &  -7.728800 &     21.478 $\pm$   0.067 &    21.715 $\pm$   0.070 &    21.769 $\pm$   0.104 &      0.330 \\ 
   872 & 151.314799 &  -7.728806 &     22.277 $\pm$   0.119 &    22.542 $\pm$   0.137 &    22.136 $\pm$   0.130 &      0.563 \\ 
   873 & 151.308704 &  -7.728822 &     22.077 $\pm$   0.118 &    22.402 $\pm$   0.132 &    22.048 $\pm$   0.136 &      0.583 \\ 
   874 & 151.321427 &  -7.728961 &     22.352 $\pm$   0.109 &    22.314 $\pm$   0.105 &    22.119 $\pm$   0.114 &      0.723 \\ 
   875 & 151.332655 &  -7.729064 &     22.122 $\pm$   0.072 &    22.077 $\pm$   0.077 &    22.109 $\pm$   0.097 &      0.483 \\ 
   876 & 151.304773 &  -7.729061 &     22.048 $\pm$   0.126 &    22.488 $\pm$   0.148 &    21.999 $\pm$   0.140 &      0.653 \\ 
   877 & 151.272492 &  -7.729220 &     20.692 $\pm$   0.022 &    20.825 $\pm$   0.026 &    20.986 $\pm$   0.037 &      0.973 \\ 
   878 & 151.307140 &  -7.729187 &     21.671 $\pm$   0.085 &    21.574 $\pm$   0.063 &    21.641 $\pm$   0.096 &      0.770 \\ 
   879 & 151.290066 &  -7.729347 &     21.147 $\pm$   0.050 &    20.931 $\pm$   0.035 &    21.047 $\pm$   0.054 &      0.970 \\ 
   880 & 151.298754 &  -7.729329 &     21.343 $\pm$   0.071 &    21.345 $\pm$   0.055 &    21.124 $\pm$   0.065 &      0.420 \\ 
   881 & 151.288339 &  -7.729255 &     22.510 $\pm$   0.158 &    22.343 $\pm$   0.119 &    22.132 $\pm$   0.139 &      0.583 \\ 
   882 & 151.295945 &  -7.729317 &     21.627 $\pm$   0.087 &    21.480 $\pm$   0.060 &    20.979 $\pm$   0.056 &      0.350 \\ 
   883 & 151.317380 &  -7.729442 &     21.994 $\pm$   0.086 &    22.399 $\pm$   0.117 &    21.861 $\pm$   0.097 &      0.013 \\ 
   884 & 151.307486 &  -7.729423 &     21.930 $\pm$   0.105 &    21.987 $\pm$   0.091 &    21.919 $\pm$   0.122 &      0.513 \\ 
   885 & 151.310404 &  -7.729526 &     21.270 $\pm$   0.054 &    21.312 $\pm$   0.048 &    21.597 $\pm$   0.086 &      0.930 \\ 
   886 & 151.302825 &  -7.729602 &     20.900 $\pm$   0.047 &    21.015 $\pm$   0.040 &    21.258 $\pm$   0.072 &      0.957 \\ 
   887 & 151.369881 &  -7.729566 &     23.036 $\pm$   0.124 &    22.503 $\pm$   0.090 &    22.182 $\pm$   0.078 &      0.583 \\ 
   888 & 151.318232 &  -7.729699 &     21.725 $\pm$   0.066 &    21.821 $\pm$   0.069 &    21.435 $\pm$   0.064 &      0.177 \\ 
   889 & 151.279086 &  -7.729820 &     21.137 $\pm$   0.037 &    21.050 $\pm$   0.034 &    21.103 $\pm$   0.046 &      0.970 \\ 
   890 & 151.292621 &  -7.729853 &     20.655 $\pm$   0.036 &    20.590 $\pm$   0.027 &    19.975 $\pm$   0.022 &      0.063 \\ 
   891 & 151.296818 &  -7.729838 &     22.001 $\pm$   0.124 &    22.032 $\pm$   0.099 &    21.901 $\pm$   0.129 &      0.387 \\ 
   892 & 151.298457 &  -7.729828 &     21.886 $\pm$   0.113 &    21.954 $\pm$   0.093 &    21.476 $\pm$   0.089 &      0.633 \\ 
   893 & 151.298661 &  -7.729958 &     21.811 $\pm$   0.105 &    21.762 $\pm$   0.078 &    21.476 $\pm$   0.089 &      0.773 \\ 
   894 & 151.297869 &  -7.729995 &     21.632 $\pm$   0.090 &    21.350 $\pm$   0.054 &    21.507 $\pm$   0.091 &      0.703 \\ 
   895 & 151.336960 &  -7.730085 &     21.874 $\pm$   0.055 &    21.861 $\pm$   0.061 &    22.082 $\pm$   0.089 &      0.893 \\ 
   896 & 151.351147 &  -7.730273 &     21.209 $\pm$   0.029 &    21.053 $\pm$   0.028 &    20.361 $\pm$   0.018 &      0.213 \\ 
   897 & 151.365961 &  -7.730503 &     21.915 $\pm$   0.048 &    22.648 $\pm$   0.104 &    22.151 $\pm$   0.076 &      0.000 \\ 
   898 & 151.296227 &  -7.730626 &     21.092 $\pm$   0.056 &    21.501 $\pm$   0.062 &    21.320 $\pm$   0.075 &      0.010 \\ 
   899 & 151.295680 &  -7.731189 &     21.299 $\pm$   0.066 &    21.801 $\pm$   0.080 &    21.293 $\pm$   0.073 &      0.010 \\ 
   900 & 151.298853 &  -7.730278 &     22.002 $\pm$   0.123 &    21.909 $\pm$   0.089 &    22.267 $\pm$   0.180 &      0.570 \\ 
   901 & 151.299209 &  -7.730258 &     22.019 $\pm$   0.125 &    21.812 $\pm$   0.082 &    21.913 $\pm$   0.131 &      0.723 \\ 
   902 & 151.268657 &  -7.730613 &     18.882 $\pm$   0.007 &    18.791 $\pm$   0.006 &    18.961 $\pm$   0.007 &      0.980 \\ 
   903 & 151.325452 &  -7.730392 &     22.548 $\pm$   0.117 &    22.539 $\pm$   0.121 &    22.307 $\pm$   0.125 &      0.560 \\ 
   904 & 151.275753 &  -7.730525 &     22.447 $\pm$   0.107 &    22.528 $\pm$   0.121 &    22.404 $\pm$   0.141 &      0.607 \\ 
   905 & 151.288011 &  -7.730835 &     20.654 $\pm$   0.032 &    20.888 $\pm$   0.033 &    20.174 $\pm$   0.024 &      0.027 \\ 
   906 & 151.297510 &  -7.730624 &     22.112 $\pm$   0.136 &    21.683 $\pm$   0.072 &    21.331 $\pm$   0.077 &      0.667 \\ 
   907 & 151.320997 &  -7.731360 &     21.082 $\pm$   0.035 &    21.242 $\pm$   0.040 &    20.912 $\pm$   0.038 &      0.170 \\ 
   908 & 151.321471 &  -7.731926 &     18.887 $\pm$   0.007 &    18.814 $\pm$   0.006 &    18.324 $\pm$   0.005 &      0.503 \\ 
   909 & 151.310746 &  -7.730875 &     22.312 $\pm$   0.129 &    22.211 $\pm$   0.105 &    22.030 $\pm$   0.123 &      0.597 \\ 
   910 & 151.294636 &  -7.730948 &     22.153 $\pm$   0.136 &    22.160 $\pm$   0.109 &    21.782 $\pm$   0.113 &      0.697 \\ 
   911 & 151.367266 &  -7.731068 &     21.950 $\pm$   0.049 &    21.866 $\pm$   0.052 &    21.282 $\pm$   0.036 &      0.660 \\ 
   912 & 151.274429 &  -7.731162 &     21.412 $\pm$   0.042 &    21.403 $\pm$   0.044 &    21.371 $\pm$   0.055 &      0.973 \\ 
   913 & 151.323022 &  -7.731204 &     20.470 $\pm$   0.021 &    20.450 $\pm$   0.020 &    20.638 $\pm$   0.029 &      0.977 \\ 
   914 & 151.293975 &  -7.731154 &     22.115 $\pm$   0.128 &    21.765 $\pm$   0.076 &    21.513 $\pm$   0.087 &      0.517 \\ 
   915 & 151.321855 &  -7.731273 &     21.583 $\pm$   0.053 &    21.275 $\pm$   0.040 &    21.459 $\pm$   0.060 &      0.943 \\ 
   916 & 151.297273 &  -7.731260 &     21.919 $\pm$   0.113 &    21.767 $\pm$   0.078 &    21.158 $\pm$   0.065 &      0.377 \\ 
   917 & 151.299363 &  -7.731233 &     21.745 $\pm$   0.096 &    22.014 $\pm$   0.096 &    21.888 $\pm$   0.126 &      0.713 \\ 
   918 & 151.305621 &  -7.731367 &     21.687 $\pm$   0.083 &    21.537 $\pm$   0.060 &    21.096 $\pm$   0.057 &      0.717 \\ 
   919 & 151.265745 &  -7.731486 &     21.550 $\pm$   0.041 &    21.910 $\pm$   0.064 &    20.998 $\pm$   0.035 &      0.007 \\ 
   920 & 151.359399 &  -7.731525 &     20.301 $\pm$   0.014 &    20.329 $\pm$   0.015 &    20.532 $\pm$   0.020 &      0.980 \\ 
   921 & 151.289487 &  -7.731406 &     22.270 $\pm$   0.133 &    22.070 $\pm$   0.096 &    22.155 $\pm$   0.146 &      0.567 \\ 
   922 & 151.296608 &  -7.731558 &     21.701 $\pm$   0.093 &    22.067 $\pm$   0.101 &    21.596 $\pm$   0.096 &      0.230 \\ 
   923 & 151.351169 &  -7.731409 &     23.079 $\pm$   0.143 &    22.719 $\pm$   0.119 &    22.108 $\pm$   0.078 &      0.593 \\ 
   924 & 151.282719 &  -7.731580 &     22.048 $\pm$   0.090 &    21.871 $\pm$   0.073 &    22.294 $\pm$   0.145 &      0.783 \\ 
   925 & 151.298433 &  -7.731655 &     20.419 $\pm$   0.031 &    20.084 $\pm$   0.018 &    20.311 $\pm$   0.030 &      0.967 \\ 
   926 & 151.258319 &  -7.731720 &     21.570 $\pm$   0.039 &    21.570 $\pm$   0.045 &    20.795 $\pm$   0.027 &      0.293 \\ 
   927 & 151.311022 &  -7.731793 &     20.166 $\pm$   0.020 &    20.007 $\pm$   0.015 &    20.299 $\pm$   0.025 &      0.980 \\ 
   928 & 151.291358 &  -7.731740 &     22.224 $\pm$   0.134 &    21.992 $\pm$   0.091 &    21.839 $\pm$   0.113 &      0.470 \\ 
   929 & 151.295110 &  -7.731834 &     21.778 $\pm$   0.097 &    21.942 $\pm$   0.090 &    21.552 $\pm$   0.091 &      0.150 \\ 
   930 & 151.364034 &  -7.731817 &     22.489 $\pm$   0.079 &    22.577 $\pm$   0.098 &    22.051 $\pm$   0.070 &      0.400 \\ 
   931 & 151.294566 &  -7.732079 &     21.846 $\pm$   0.102 &    22.300 $\pm$   0.123 &    21.926 $\pm$   0.127 &      0.297 \\ 
   932 & 151.293919 &  -7.732259 &     21.167 $\pm$   0.056 &    21.395 $\pm$   0.055 &    21.072 $\pm$   0.058 &      0.017 \\ 
   933 & 151.361989 &  -7.731392 &     22.589 $\pm$   0.087 &    22.785 $\pm$   0.120 &    22.302 $\pm$   0.088 &      0.527 \\ 
   934 & 151.262498 &  -7.732235 &     21.645 $\pm$   0.043 &    21.794 $\pm$   0.056 &    22.039 $\pm$   0.085 &      0.870 \\ 
   935 & 151.303617 &  -7.732131 &     22.301 $\pm$   0.145 &    22.280 $\pm$   0.118 &    22.009 $\pm$   0.132 &      0.667 \\ 
   936 & 151.319087 &  -7.732279 &     20.635 $\pm$   0.025 &    20.729 $\pm$   0.026 &    20.789 $\pm$   0.034 &      0.967 \\ 
   937 & 151.347688 &  -7.732215 &     22.711 $\pm$   0.105 &    22.653 $\pm$   0.115 &    21.723 $\pm$   0.059 &      0.583 \\ 
   938 & 151.300502 &  -7.732327 &     21.012 $\pm$   0.049 &    21.037 $\pm$   0.040 &    21.156 $\pm$   0.063 &      0.950 \\ 
   939 & 151.285705 &  -7.732473 &     20.998 $\pm$   0.040 &    20.835 $\pm$   0.031 &    20.117 $\pm$   0.022 &      0.097 \\ 
   940 & 151.259921 &  -7.732404 &     22.515 $\pm$   0.090 &    22.612 $\pm$   0.113 &    22.521 $\pm$   0.128 &      0.617 \\ 
   941 & 151.299458 &  -7.732477 &     21.930 $\pm$   0.109 &    21.958 $\pm$   0.091 &    21.423 $\pm$   0.080 &      0.290 \\ 
   942 & 151.304498 &  -7.732756 &     18.528 $\pm$   0.008 &    18.508 $\pm$   0.005 &    18.619 $\pm$   0.007 &      0.980 \\ 
   943 & 151.349200 &  -7.732709 &     19.797 $\pm$   0.010 &    19.997 $\pm$   0.012 &    20.332 $\pm$   0.018 &      0.980 \\ 
   944 & 151.260387 &  -7.732729 &     20.523 $\pm$   0.017 &    20.629 $\pm$   0.020 &    20.707 $\pm$   0.026 &      0.967 \\ 
   945 & 151.292629 &  -7.732717 &     19.764 $\pm$   0.018 &    19.767 $\pm$   0.014 &    19.858 $\pm$   0.019 &      0.983 \\ 
   946 & 151.315730 &  -7.732822 &     21.130 $\pm$   0.039 &    21.071 $\pm$   0.035 &    21.133 $\pm$   0.048 &      0.840 \\ 
   947 & 151.286718 &  -7.732779 &     22.152 $\pm$   0.113 &    22.095 $\pm$   0.095 &    21.895 $\pm$   0.111 &      0.667 \\ 
   948 & 151.308985 &  -7.732889 &     21.148 $\pm$   0.046 &    21.255 $\pm$   0.044 &    21.229 $\pm$   0.059 &      0.803 \\ 
   949 & 151.296209 &  -7.732906 &     22.010 $\pm$   0.117 &    22.097 $\pm$   0.102 &    21.927 $\pm$   0.127 &      0.430 \\ 
   950 & 151.294983 &  -7.733130 &     22.116 $\pm$   0.128 &    21.767 $\pm$   0.076 &    21.108 $\pm$   0.060 &      0.177 \\ 
   951 & 151.293603 &  -7.733216 &     21.293 $\pm$   0.061 &    21.408 $\pm$   0.055 &    21.311 $\pm$   0.072 &      0.027 \\ 
   952 & 151.367841 &  -7.733067 &     22.580 $\pm$   0.084 &    22.530 $\pm$   0.093 &    21.788 $\pm$   0.055 &      0.147 \\ 
   953 & 151.365813 &  -7.733247 &     22.168 $\pm$   0.059 &    22.553 $\pm$   0.095 &    21.645 $\pm$   0.049 &      0.043 \\ 
   954 & 151.343247 &  -7.733234 &     22.348 $\pm$   0.078 &    22.217 $\pm$   0.079 &    22.589 $\pm$   0.131 &      0.650 \\ 
   955 & 151.291046 &  -7.733251 &     22.197 $\pm$   0.129 &    22.226 $\pm$   0.112 &    21.828 $\pm$   0.111 &      0.687 \\ 
   956 & 151.321822 &  -7.733451 &     20.280 $\pm$   0.018 &    20.243 $\pm$   0.017 &    20.503 $\pm$   0.025 &      0.980 \\ 
   957 & 151.311336 &  -7.733438 &     21.649 $\pm$   0.066 &    21.459 $\pm$   0.051 &    21.599 $\pm$   0.078 &      0.893 \\ 
   958 & 151.313387 &  -7.733501 &     21.041 $\pm$   0.037 &    20.954 $\pm$   0.032 &    21.170 $\pm$   0.051 &      0.973 \\ 
   959 & 151.349148 &  -7.733468 &     21.764 $\pm$   0.045 &    21.824 $\pm$   0.054 &    22.271 $\pm$   0.092 &      0.853 \\ 
   960 & 151.297467 &  -7.733550 &     21.010 $\pm$   0.048 &    21.032 $\pm$   0.040 &    21.085 $\pm$   0.059 &      0.657 \\ 
   961 & 151.292368 &  -7.733492 &     22.005 $\pm$   0.111 &    21.945 $\pm$   0.087 &    21.628 $\pm$   0.094 &      0.313 \\ 
   962 & 151.364476 &  -7.733526 &     22.014 $\pm$   0.052 &    22.066 $\pm$   0.062 &    22.095 $\pm$   0.073 &      0.833 \\ 
   963 & 151.342469 &  -7.733769 &     20.232 $\pm$   0.014 &    20.119 $\pm$   0.014 &    19.478 $\pm$   0.010 &      0.043 \\ 
   964 & 151.293111 &  -7.733983 &     18.921 $\pm$   0.010 &    18.894 $\pm$   0.007 &    19.103 $\pm$   0.010 &      0.947 \\ 
   965 & 151.294238 &  -7.733869 &     21.994 $\pm$   0.112 &    21.781 $\pm$   0.076 &    21.558 $\pm$   0.089 &      0.540 \\ 
   966 & 151.330332 &  -7.733929 &     22.038 $\pm$   0.065 &    22.312 $\pm$   0.093 &    22.419 $\pm$   0.126 &      0.753 \\ 
   967 & 151.318350 &  -7.734086 &     20.436 $\pm$   0.021 &    20.531 $\pm$   0.022 &    20.670 $\pm$   0.030 &      0.617 \\ 
   968 & 151.282895 &  -7.734221 &     21.648 $\pm$   0.066 &    21.836 $\pm$   0.072 &    21.253 $\pm$   0.058 &      0.107 \\ 
   969 & 151.306581 &  -7.734142 &     22.199 $\pm$   0.116 &    22.189 $\pm$   0.103 &    21.783 $\pm$   0.098 &      0.750 \\ 
   970 & 151.309262 &  -7.734147 &     22.322 $\pm$   0.122 &    22.215 $\pm$   0.102 &    22.151 $\pm$   0.131 &      0.630 \\ 
   971 & 151.273475 &  -7.734311 &     21.077 $\pm$   0.032 &    21.204 $\pm$   0.037 &    20.635 $\pm$   0.029 &      0.227 \\ 
   972 & 151.293671 &  -7.734336 &     21.239 $\pm$   0.058 &    21.305 $\pm$   0.050 &    21.381 $\pm$   0.076 &      0.250 \\ 
   973 & 151.298965 &  -7.734261 &     22.283 $\pm$   0.143 &    22.087 $\pm$   0.099 &    21.681 $\pm$   0.098 &      0.607 \\ 
   974 & 151.291304 &  -7.734365 &     22.160 $\pm$   0.125 &    22.040 $\pm$   0.094 &    22.068 $\pm$   0.138 &      0.737 \\ 
   975 & 151.297299 &  -7.734629 &     19.987 $\pm$   0.021 &    19.888 $\pm$   0.015 &    19.943 $\pm$   0.021 &      0.957 \\ 
   976 & 151.305159 &  -7.734619 &     20.068 $\pm$   0.020 &    19.998 $\pm$   0.015 &    20.084 $\pm$   0.022 &      0.980 \\ 
   977 & 151.344846 &  -7.734580 &     21.535 $\pm$   0.038 &    21.627 $\pm$   0.046 &    21.750 $\pm$   0.060 &      0.880 \\ 
   978 & 151.333679 &  -7.709532 &     22.367 $\pm$   0.114 &    22.358 $\pm$   0.110 &    21.891 $\pm$   0.097 &      0.687 \\ 
   979 & 151.290775 &  -7.734696 &     22.348 $\pm$   0.147 &    22.167 $\pm$   0.105 &    22.203 $\pm$   0.155 &      0.677 \\ 
   980 & 151.284901 &  -7.734722 &     22.437 $\pm$   0.140 &    22.093 $\pm$   0.093 &    21.806 $\pm$   0.099 &      0.463 \\ 
   981 & 151.347674 &  -7.735127 &     17.445 $\pm$   0.004 &    17.306 $\pm$   0.002 &    17.511 $\pm$   0.003 &      0.980 \\ 
   982 & 151.292847 &  -7.735015 &     22.274 $\pm$   0.141 &    22.205 $\pm$   0.110 &    21.983 $\pm$   0.129 &      0.380 \\ 
   983 & 151.303178 &  -7.735022 &     21.578 $\pm$   0.071 &    21.442 $\pm$   0.054 &    21.740 $\pm$   0.098 &      0.867 \\ 
   984 & 151.303448 &  -7.735227 &     20.434 $\pm$   0.027 &    20.412 $\pm$   0.022 &    20.679 $\pm$   0.037 &      0.967 \\ 
   985 & 151.353613 &  -7.735128 &     20.610 $\pm$   0.018 &    20.517 $\pm$   0.018 &    20.566 $\pm$   0.021 &      0.960 \\ 
   986 & 151.299780 &  -7.735117 &     22.375 $\pm$   0.150 &    22.287 $\pm$   0.117 &    22.165 $\pm$   0.150 &      0.603 \\ 
   987 & 151.302247 &  -7.735608 &     18.160 $\pm$   0.006 &    18.271 $\pm$   0.005 &    18.331 $\pm$   0.005 &      0.737 \\ 
   988 & 151.332445 &  -7.735199 &     22.891 $\pm$   0.136 &    22.642 $\pm$   0.124 &    21.809 $\pm$   0.070 &      0.433 \\ 
   989 & 151.337620 &  -7.735342 &     22.192 $\pm$   0.070 &    22.625 $\pm$   0.117 &    21.904 $\pm$   0.073 &      0.307 \\ 
   990 & 151.294143 &  -7.735274 &     22.194 $\pm$   0.131 &    21.961 $\pm$   0.088 &    22.021 $\pm$   0.134 &      0.507 \\ 
   991 & 151.325928 &  -7.735545 &     18.471 $\pm$   0.006 &    18.377 $\pm$   0.004 &    18.513 $\pm$   0.005 &      0.980 \\ 
   992 & 151.296190 &  -7.735376 &     21.861 $\pm$   0.097 &    21.870 $\pm$   0.081 &    21.956 $\pm$   0.125 &      0.493 \\ 
   993 & 151.292967 &  -7.735371 &     22.308 $\pm$   0.144 &    21.911 $\pm$   0.084 &    21.936 $\pm$   0.124 &      0.670 \\ 
   994 & 151.317011 &  -7.735521 &     19.928 $\pm$   0.014 &    20.051 $\pm$   0.014 &    20.348 $\pm$   0.023 &      0.980 \\ 
   995 & 151.289309 &  -7.735406 &     22.318 $\pm$   0.138 &    22.063 $\pm$   0.095 &    22.186 $\pm$   0.150 &      0.417 \\ 
   996 & 151.337099 &  -7.735627 &     20.940 $\pm$   0.025 &    20.856 $\pm$   0.025 &    20.184 $\pm$   0.017 &      0.047 \\ 
   997 & 151.362750 &  -7.735558 &     22.479 $\pm$   0.078 &    22.511 $\pm$   0.093 &    22.127 $\pm$   0.075 &      0.413 \\ 
   998 & 151.313055 &  -7.735732 &     21.194 $\pm$   0.041 &    21.160 $\pm$   0.038 &    21.389 $\pm$   0.060 &      0.927 \\ 
   999 & 151.359478 &  -7.735815 &     21.585 $\pm$   0.037 &    21.763 $\pm$   0.049 &    21.400 $\pm$   0.040 &      0.177 \\ 
  1000 & 151.290842 &  -7.735799 &     22.310 $\pm$   0.140 &    22.309 $\pm$   0.119 &    21.759 $\pm$   0.103 &      0.570 \\ 
  1001 & 151.279556 &  -7.736127 &     20.958 $\pm$   0.034 &    21.304 $\pm$   0.043 &    20.727 $\pm$   0.034 &      0.023 \\ 
  1002 & 151.363443 &  -7.736021 &     22.092 $\pm$   0.056 &    22.010 $\pm$   0.060 &    21.124 $\pm$   0.032 &      0.063 \\ 
  1003 & 151.293852 &  -7.736208 &     20.330 $\pm$   0.026 &    20.316 $\pm$   0.021 &    20.388 $\pm$   0.030 &      0.963 \\ 
  1004 & 151.354169 &  -7.736305 &     21.172 $\pm$   0.027 &    21.388 $\pm$   0.036 &    20.883 $\pm$   0.027 &      0.013 \\ 
  1005 & 151.292350 &  -7.736170 &     22.000 $\pm$   0.108 &    22.056 $\pm$   0.095 &    21.873 $\pm$   0.115 &      0.407 \\ 
  1006 & 151.270587 &  -7.736273 &     21.865 $\pm$   0.059 &    21.862 $\pm$   0.064 &    21.951 $\pm$   0.089 &      0.833 \\ 
  1007 & 151.306433 &  -7.736361 &     20.661 $\pm$   0.029 &    20.697 $\pm$   0.027 &    20.861 $\pm$   0.041 &      0.973 \\ 
  1008 & 151.285034 &  -7.736452 &     21.811 $\pm$   0.081 &    21.950 $\pm$   0.082 &    21.560 $\pm$   0.080 &      0.083 \\ 
  1009 & 151.326627 &  -7.736464 &     20.594 $\pm$   0.020 &    20.567 $\pm$   0.021 &    20.798 $\pm$   0.030 &      0.973 \\ 
  1010 & 151.346926 &  -7.736372 &     21.871 $\pm$   0.050 &    21.915 $\pm$   0.059 &    22.484 $\pm$   0.112 &      0.790 \\ 
  1011 & 151.321709 &  -7.736412 &     22.039 $\pm$   0.072 &    21.887 $\pm$   0.066 &    21.468 $\pm$   0.057 &      0.830 \\ 
  1012 & 151.291590 &  -7.736547 &     22.370 $\pm$   0.148 &    22.241 $\pm$   0.112 &    22.249 $\pm$   0.161 &      0.620 \\ 
  1013 & 151.309006 &  -7.736914 &     18.445 $\pm$   0.006 &    18.481 $\pm$   0.005 &    18.642 $\pm$   0.006 &      0.980 \\ 
  1014 & 151.314177 &  -7.736848 &     20.653 $\pm$   0.025 &    20.667 $\pm$   0.024 &    20.828 $\pm$   0.035 &      0.927 \\ 
  1015 & 151.366563 &  -7.736686 &     22.729 $\pm$   0.096 &    22.642 $\pm$   0.102 &    22.533 $\pm$   0.107 &      0.653 \\ 
  1016 & 151.299229 &  -7.736839 &     21.974 $\pm$   0.101 &    22.018 $\pm$   0.090 &    22.305 $\pm$   0.165 &      0.713 \\ 
  1017 & 151.345238 &  -7.736879 &     23.069 $\pm$   0.144 &    22.852 $\pm$   0.137 &    22.173 $\pm$   0.087 &      0.530 \\ 
  1018 & 151.295641 &  -7.736996 &     21.399 $\pm$   0.062 &    21.457 $\pm$   0.055 &    21.354 $\pm$   0.071 &      0.373 \\ 
  1019 & 151.307174 &  -7.737122 &     19.935 $\pm$   0.016 &    19.884 $\pm$   0.013 &    19.955 $\pm$   0.018 &      0.980 \\ 
  1020 & 151.290275 &  -7.736997 &     22.243 $\pm$   0.129 &    22.127 $\pm$   0.100 &    22.035 $\pm$   0.131 &      0.507 \\ 
  1021 & 151.253043 &  -7.737202 &     22.431 $\pm$   0.080 &    22.319 $\pm$   0.083 &    22.174 $\pm$   0.084 &      0.693 \\ 
  1022 & 151.286728 &  -7.737225 &     22.051 $\pm$   0.103 &    22.165 $\pm$   0.101 &    22.033 $\pm$   0.126 &      0.627 \\ 
  1023 & 151.301327 &  -7.737057 &     21.266 $\pm$   0.052 &    21.360 $\pm$   0.049 &    21.562 $\pm$   0.081 &      0.940 \\ 
  1024 & 151.296320 &  -7.737456 &     20.599 $\pm$   0.032 &    20.536 $\pm$   0.025 &    20.050 $\pm$   0.022 &      0.507 \\ 
  1025 & 151.303899 &  -7.737401 &     22.605 $\pm$   0.160 &    22.222 $\pm$   0.103 &    22.122 $\pm$   0.129 &      0.393 \\ 
  1026 & 151.290275 &  -7.737537 &     22.341 $\pm$   0.140 &    22.052 $\pm$   0.093 &    21.733 $\pm$   0.099 &      0.400 \\ 
  1027 & 151.288701 &  -7.737765 &     22.259 $\pm$   0.128 &    22.150 $\pm$   0.101 &    21.952 $\pm$   0.119 &      0.597 \\ 
  1028 & 151.295070 &  -7.737755 &     21.982 $\pm$   0.103 &    22.217 $\pm$   0.108 &    21.990 $\pm$   0.125 &      0.360 \\ 
  1029 & 151.285924 &  -7.737769 &     22.298 $\pm$   0.127 &    22.233 $\pm$   0.107 &    21.937 $\pm$   0.113 &      0.720 \\ 
  1030 & 151.299048 &  -7.737894 &     22.444 $\pm$   0.148 &    22.497 $\pm$   0.137 &    21.806 $\pm$   0.102 &      0.597 \\ 
  1031 & 151.289888 &  -7.738032 &     22.079 $\pm$   0.110 &    22.066 $\pm$   0.094 &    21.753 $\pm$   0.100 &      0.487 \\ 
  1032 & 151.296987 &  -7.738028 &     22.176 $\pm$   0.120 &    22.368 $\pm$   0.123 &    22.217 $\pm$   0.150 &      0.703 \\ 
  1033 & 151.255913 &  -7.738548 &     16.376 $\pm$   0.003 &    16.569 $\pm$   0.002 &    16.888 $\pm$   0.002 &      0.983 \\ 
  1034 & 151.355168 &  -7.738576 &     22.746 $\pm$   0.102 &    22.894 $\pm$   0.135 &    22.451 $\pm$   0.101 &      0.483 \\ 
  1035 & 151.330377 &  -7.738827 &     20.023 $\pm$   0.013 &    20.014 $\pm$   0.013 &    20.249 $\pm$   0.018 &      0.980 \\ 
  1036 & 151.261699 &  -7.738746 &     23.051 $\pm$   0.149 &    22.857 $\pm$   0.145 &    22.642 $\pm$   0.148 &      0.467 \\ 
  1037 & 151.266568 &  -7.738927 &     22.346 $\pm$   0.084 &    22.013 $\pm$   0.071 &    21.142 $\pm$   0.041 &      0.680 \\ 
  1038 & 151.308372 &  -7.738966 &     21.077 $\pm$   0.037 &    21.116 $\pm$   0.036 &    21.056 $\pm$   0.045 &      0.927 \\ 
  1039 & 151.349447 &  -7.739399 &     20.489 $\pm$   0.016 &    20.331 $\pm$   0.016 &    19.626 $\pm$   0.010 &      0.053 \\ 
  1040 & 151.274532 &  -7.739077 &     22.497 $\pm$   0.115 &    22.605 $\pm$   0.131 &    22.389 $\pm$   0.142 &      0.570 \\ 
  1041 & 151.329259 &  -7.739361 &     19.637 $\pm$   0.010 &    19.677 $\pm$   0.010 &    19.903 $\pm$   0.014 &      0.983 \\ 
  1042 & 151.331554 &  -7.739295 &     22.158 $\pm$   0.069 &    22.134 $\pm$   0.077 &    22.498 $\pm$   0.128 &      0.737 \\ 
  1043 & 151.290576 &  -7.739410 &     21.184 $\pm$   0.049 &    21.080 $\pm$   0.039 &    21.304 $\pm$   0.066 &      0.970 \\ 
  1044 & 151.269062 &  -7.739474 &     21.207 $\pm$   0.033 &    21.326 $\pm$   0.040 &    21.336 $\pm$   0.051 &      0.957 \\ 
  1045 & 151.267486 &  -7.739431 &     22.415 $\pm$   0.092 &    22.638 $\pm$   0.126 &    22.151 $\pm$   0.103 &      0.563 \\ 
  1046 & 151.261195 &  -7.739531 &     22.065 $\pm$   0.062 &    22.096 $\pm$   0.073 &    22.160 $\pm$   0.095 &      0.760 \\ 
  1047 & 151.304524 &  -7.740523 &     13.570 $\pm$   0.001 &    13.713 $\pm$   0.001 &    14.075 $\pm$   0.001 &      1.000 \\ 
  1048 & 151.335835 &  -7.739690 &     19.333 $\pm$   0.008 &    19.442 $\pm$   0.008 &    19.794 $\pm$   0.012 &      0.980 \\ 
  1049 & 151.347892 &  -7.739664 &     20.213 $\pm$   0.013 &    20.136 $\pm$   0.013 &    20.299 $\pm$   0.017 &      0.977 \\ 
  1050 & 151.336839 &  -7.739796 &     21.346 $\pm$   0.033 &    21.196 $\pm$   0.033 &    20.757 $\pm$   0.026 &      0.367 \\ 
  1051 & 151.294339 &  -7.739769 &     22.024 $\pm$   0.102 &    21.842 $\pm$   0.076 &    21.737 $\pm$   0.096 &      0.790 \\ 
  1052 & 151.281868 &  -7.739852 &     21.982 $\pm$   0.086 &    22.252 $\pm$   0.104 &    21.920 $\pm$   0.104 &      0.750 \\ 
  1053 & 151.292565 &  -7.739808 &     22.351 $\pm$   0.137 &    22.268 $\pm$   0.111 &    21.959 $\pm$   0.118 &      0.680 \\ 
  1054 & 151.294434 &  -7.740204 &     20.210 $\pm$   0.022 &    20.225 $\pm$   0.019 &    20.323 $\pm$   0.027 &      0.983 \\ 
  1055 & 151.251191 &  -7.740137 &     22.536 $\pm$   0.086 &    22.469 $\pm$   0.093 &    21.927 $\pm$   0.066 &      0.633 \\ 
  1056 & 151.272142 &  -7.740219 &     22.209 $\pm$   0.085 &    22.207 $\pm$   0.090 &    21.692 $\pm$   0.073 &      0.073 \\ 
  1057 & 151.342244 &  -7.740362 &     21.949 $\pm$   0.054 &    22.224 $\pm$   0.078 &    21.543 $\pm$   0.050 &      0.047 \\ 
  1058 & 151.302552 &  -7.740746 &     18.762 $\pm$   0.007 &    18.701 $\pm$   0.006 &    18.820 $\pm$   0.007 &      0.980 \\ 
  1059 & 151.310259 &  -7.740644 &     21.194 $\pm$   0.038 &    21.034 $\pm$   0.033 &    20.441 $\pm$   0.025 &      0.243 \\ 
  1060 & 151.351832 &  -7.740673 &     22.563 $\pm$   0.087 &    22.605 $\pm$   0.106 &    22.013 $\pm$   0.070 &      0.260 \\ 
  1061 & 151.289854 &  -7.740879 &     19.497 $\pm$   0.013 &    19.471 $\pm$   0.010 &    19.556 $\pm$   0.014 &      0.963 \\ 
  1062 & 151.289604 &  -7.741181 &     20.845 $\pm$   0.036 &    20.940 $\pm$   0.034 &    20.500 $\pm$   0.031 &      0.723 \\ 
  1063 & 151.275319 &  -7.741193 &     19.149 $\pm$   0.009 &    19.129 $\pm$   0.007 &    19.224 $\pm$   0.009 &      0.973 \\ 
  1064 & 151.345384 &  -7.740950 &     23.025 $\pm$   0.136 &    23.011 $\pm$   0.156 &    22.541 $\pm$   0.117 &      0.533 \\ 
  1065 & 151.250226 &  -7.741120 &     22.973 $\pm$   0.126 &    22.635 $\pm$   0.107 &    22.464 $\pm$   0.106 &      0.660 \\ 
  1066 & 151.277485 &  -7.741072 &     22.958 $\pm$   0.188 &    22.642 $\pm$   0.141 &    22.219 $\pm$   0.127 &      0.577 \\ 
  1067 & 151.261851 &  -7.741413 &     22.263 $\pm$   0.074 &    22.478 $\pm$   0.103 &    22.582 $\pm$   0.140 &      0.653 \\ 
  1068 & 151.271070 &  -7.741453 &     22.608 $\pm$   0.118 &    22.647 $\pm$   0.132 &    21.769 $\pm$   0.077 &      0.517 \\ 
  1069 & 151.293185 &  -7.741551 &     21.941 $\pm$   0.091 &    22.121 $\pm$   0.095 &    21.600 $\pm$   0.082 &      0.600 \\ 
  1070 & 151.259128 &  -7.741648 &     22.252 $\pm$   0.072 &    22.614 $\pm$   0.113 &    22.342 $\pm$   0.107 &      0.693 \\ 
  1071 & 151.281725 &  -7.741569 &     22.476 $\pm$   0.133 &    22.520 $\pm$   0.131 &    22.066 $\pm$   0.118 &      0.620 \\ 
  1072 & 151.287394 &  -7.741664 &     22.282 $\pm$   0.122 &    22.580 $\pm$   0.143 &    21.894 $\pm$   0.107 &      0.680 \\ 
  1073 & 151.251407 &  -7.741929 &     18.904 $\pm$   0.006 &    18.909 $\pm$   0.006 &    19.012 $\pm$   0.007 &      0.980 \\ 
  1074 & 151.289443 &  -7.741662 &     22.270 $\pm$   0.121 &    22.386 $\pm$   0.121 &    21.833 $\pm$   0.102 &      0.693 \\ 
  1075 & 151.363283 &  -7.741683 &     22.820 $\pm$   0.104 &    23.005 $\pm$   0.142 &    22.261 $\pm$   0.084 &      0.550 \\ 
  1076 & 151.284192 &  -7.741823 &     22.218 $\pm$   0.110 &    22.095 $\pm$   0.091 &    21.973 $\pm$   0.112 &      0.660 \\ 
  1077 & 151.311494 &  -7.741823 &     22.691 $\pm$   0.137 &    22.339 $\pm$   0.103 &    22.040 $\pm$   0.100 &      0.633 \\ 
  1078 & 151.256227 &  -7.742347 &     20.952 $\pm$   0.024 &    21.127 $\pm$   0.030 &    21.383 $\pm$   0.044 &      0.970 \\ 
  1079 & 151.371693 &  -7.743557 &     14.059 $\pm$   0.001 &    14.084 $\pm$   0.001 &    14.440 $\pm$   0.001 &      1.000 \\ 
  1080 & 151.328710 &  -7.743294 &     20.927 $\pm$   0.025 &    20.738 $\pm$   0.023 &    19.957 $\pm$   0.014 &      0.037 \\ 
  1081 & 151.303103 &  -7.743295 &     21.650 $\pm$   0.059 &    21.718 $\pm$   0.061 &    22.038 $\pm$   0.108 &      0.870 \\ 
  1082 & 151.327315 &  -7.743874 &     21.229 $\pm$   0.031 &    21.442 $\pm$   0.042 &    20.677 $\pm$   0.026 &      0.007 \\ 
  1083 & 151.256201 &  -7.743642 &     17.797 $\pm$   0.004 &    17.981 $\pm$   0.003 &    18.321 $\pm$   0.004 &      0.980 \\ 
  1084 & 151.265788 &  -7.743690 &     21.771 $\pm$   0.051 &    21.941 $\pm$   0.067 &    21.325 $\pm$   0.048 &      0.000 \\ 
  1085 & 151.300339 &  -7.743650 &     22.152 $\pm$   0.095 &    22.262 $\pm$   0.102 &    22.417 $\pm$   0.157 &      0.587 \\ 
  1086 & 151.290950 &  -7.743625 &     22.551 $\pm$   0.150 &    22.532 $\pm$   0.136 &    22.227 $\pm$   0.141 &      0.583 \\ 
  1087 & 151.248724 &  -7.743792 &     22.673 $\pm$   0.095 &    22.938 $\pm$   0.139 &    22.233 $\pm$   0.085 &      0.483 \\ 
  1088 & 151.366135 &  -7.743891 &     22.512 $\pm$   0.079 &    22.390 $\pm$   0.082 &    21.893 $\pm$   0.061 &      0.497 \\ 
  1089 & 151.351049 &  -7.744029 &     22.279 $\pm$   0.068 &    22.273 $\pm$   0.078 &    21.369 $\pm$   0.040 &      0.023 \\ 
  1090 & 151.300720 &  -7.744116 &     22.674 $\pm$   0.149 &    22.337 $\pm$   0.108 &    22.181 $\pm$   0.125 &      0.677 \\ 
  1091 & 151.272934 &  -7.744267 &     21.590 $\pm$   0.050 &    21.880 $\pm$   0.067 &    21.961 $\pm$   0.094 &      0.843 \\ 
  1092 & 151.373261 &  -7.744264 &     21.949 $\pm$   0.049 &    22.235 $\pm$   0.072 &    21.518 $\pm$   0.044 &      0.253 \\ 
  1093 & 151.344308 &  -7.744522 &     20.964 $\pm$   0.023 &    21.016 $\pm$   0.027 &    21.132 $\pm$   0.034 &      0.977 \\ 
  1094 & 151.283463 &  -7.744465 &     22.415 $\pm$   0.125 &    22.573 $\pm$   0.137 &    21.950 $\pm$   0.106 &      0.653 \\ 
  1095 & 151.269108 &  -7.744569 &     22.424 $\pm$   0.096 &    22.156 $\pm$   0.083 &    21.150 $\pm$   0.043 &      0.203 \\ 
  1096 & 151.328421 &  -7.744788 &     21.202 $\pm$   0.030 &    21.084 $\pm$   0.030 &    20.657 $\pm$   0.025 &      0.427 \\ 
  1097 & 151.325858 &  -7.742851 &     21.991 $\pm$   0.061 &    21.869 $\pm$   0.061 &    21.985 $\pm$   0.082 &      0.847 \\ 
  1098 & 151.366126 &  -7.744754 &     22.495 $\pm$   0.077 &    22.554 $\pm$   0.094 &    21.932 $\pm$   0.063 &      0.550 \\ 
  1099 & 151.259818 &  -7.745046 &     19.074 $\pm$   0.007 &    19.112 $\pm$   0.007 &    19.124 $\pm$   0.007 &      0.980 \\ 
  1100 & 151.258651 &  -7.744987 &     21.790 $\pm$   0.048 &    21.820 $\pm$   0.056 &    20.916 $\pm$   0.030 &      0.060 \\ 
  1101 & 151.247958 &  -7.744943 &     22.639 $\pm$   0.092 &    22.915 $\pm$   0.136 &    22.332 $\pm$   0.092 &      0.550 \\ 
  1102 & 151.321156 &  -7.744978 &     21.735 $\pm$   0.049 &    21.821 $\pm$   0.059 &    22.019 $\pm$   0.086 &      0.883 \\ 
  1103 & 151.289224 &  -7.745109 &     21.051 $\pm$   0.039 &    21.066 $\pm$   0.036 &    21.130 $\pm$   0.051 &      0.803 \\ 
  1104 & 151.303483 &  -7.742999 &     21.622 $\pm$   0.058 &    21.549 $\pm$   0.053 &    21.763 $\pm$   0.084 &      0.897 \\ 
  1105 & 151.266235 &  -7.745267 &     21.758 $\pm$   0.051 &    21.855 $\pm$   0.062 &    21.179 $\pm$   0.043 &      0.070 \\ 
  1106 & 151.278195 &  -7.745157 &     22.429 $\pm$   0.117 &    22.537 $\pm$   0.128 &    22.335 $\pm$   0.142 &      0.590 \\ 
  1107 & 151.268972 &  -7.745601 &     22.154 $\pm$   0.075 &    22.314 $\pm$   0.095 &    22.265 $\pm$   0.117 &      0.767 \\ 
  1108 & 151.303782 &  -7.745745 &     20.970 $\pm$   0.031 &    20.979 $\pm$   0.031 &    21.027 $\pm$   0.041 &      0.887 \\ 
  1109 & 151.369665 &  -7.745652 &     22.699 $\pm$   0.092 &    22.853 $\pm$   0.124 &    22.109 $\pm$   0.074 &      0.687 \\ 
  1110 & 151.260125 &  -7.745725 &     22.792 $\pm$   0.117 &    22.334 $\pm$   0.088 &    21.216 $\pm$   0.040 &      0.483 \\ 
  1111 & 151.357446 &  -7.745820 &     22.369 $\pm$   0.071 &    22.499 $\pm$   0.093 &    21.862 $\pm$   0.060 &      0.160 \\ 
  1112 & 151.290956 &  -7.745815 &     21.670 $\pm$   0.065 &    21.632 $\pm$   0.059 &    21.739 $\pm$   0.087 &      0.860 \\ 
  1113 & 151.295984 &  -7.746000 &     21.603 $\pm$   0.058 &    21.793 $\pm$   0.066 &    21.197 $\pm$   0.052 &      0.410 \\ 
  1114 & 151.307758 &  -7.746082 &     22.452 $\pm$   0.106 &    22.519 $\pm$   0.118 &    22.140 $\pm$   0.108 &      0.610 \\ 
  1115 & 151.371787 &  -7.746082 &     21.817 $\pm$   0.044 &    21.880 $\pm$   0.053 &    21.359 $\pm$   0.039 &      0.400 \\ 
  1116 & 151.289498 &  -7.746092 &     21.460 $\pm$   0.054 &    21.414 $\pm$   0.048 &    21.772 $\pm$   0.089 &      0.870 \\ 
  1117 & 151.261743 &  -7.746165 &     22.221 $\pm$   0.072 &    22.287 $\pm$   0.087 &    21.365 $\pm$   0.047 &      0.127 \\ 
  1118 & 151.286933 &  -7.746280 &     21.998 $\pm$   0.086 &    21.741 $\pm$   0.064 &    21.321 $\pm$   0.059 &      0.797 \\ 
  1119 & 151.369376 &  -7.746307 &     21.308 $\pm$   0.028 &    21.163 $\pm$   0.029 &    20.610 $\pm$   0.021 &      0.090 \\ 
  1120 & 151.300123 &  -7.746284 &     22.355 $\pm$   0.107 &    22.420 $\pm$   0.113 &    22.458 $\pm$   0.154 &      0.660 \\ 
  1121 & 151.296497 &  -7.746421 &     21.447 $\pm$   0.050 &    21.368 $\pm$   0.045 &    20.761 $\pm$   0.035 &      0.377 \\ 
  1122 & 151.343902 &  -7.747151 &     19.857 $\pm$   0.011 &    20.277 $\pm$   0.015 &    19.701 $\pm$   0.011 &      0.027 \\ 
  1123 & 151.276389 &  -7.747031 &     20.993 $\pm$   0.032 &    21.108 $\pm$   0.035 &    20.204 $\pm$   0.021 &      0.017 \\ 
  1124 & 151.363408 &  -7.747064 &     21.984 $\pm$   0.050 &    21.977 $\pm$   0.057 &    22.199 $\pm$   0.080 &      0.840 \\ 
  1125 & 151.303685 &  -7.747336 &     19.861 $\pm$   0.013 &    19.879 $\pm$   0.012 &    19.919 $\pm$   0.015 &      0.977 \\ 
  1126 & 151.311440 &  -7.747423 &     22.272 $\pm$   0.084 &    22.038 $\pm$   0.074 &    21.435 $\pm$   0.054 &      0.827 \\ 
  1127 & 151.365952 &  -7.747410 &     23.093 $\pm$   0.130 &    22.659 $\pm$   0.104 &    22.111 $\pm$   0.074 &      0.640 \\ 
  1128 & 151.337304 &  -7.747893 &     19.433 $\pm$   0.008 &    19.373 $\pm$   0.008 &    19.565 $\pm$   0.010 &      0.973 \\ 
  1129 & 151.297208 &  -7.747946 &     20.431 $\pm$   0.021 &    20.280 $\pm$   0.018 &    19.754 $\pm$   0.014 &      0.437 \\ 
  1130 & 151.247867 &  -7.747864 &     22.828 $\pm$   0.108 &    22.816 $\pm$   0.123 &    22.517 $\pm$   0.109 &      0.580 \\ 
  1131 & 151.258070 &  -7.748130 &     22.387 $\pm$   0.079 &    22.269 $\pm$   0.081 &    21.667 $\pm$   0.056 &      0.610 \\ 
  1132 & 151.280747 &  -7.746492 &     22.726 $\pm$   0.156 &    22.541 $\pm$   0.129 &    22.365 $\pm$   0.148 &      0.487 \\ 
  1133 & 151.363679 &  -7.748281 &     20.658 $\pm$   0.017 &    20.811 $\pm$   0.022 &    21.109 $\pm$   0.031 &      0.977 \\ 
  1134 & 151.272249 &  -7.748427 &     22.161 $\pm$   0.081 &    22.430 $\pm$   0.109 &    21.640 $\pm$   0.069 &      0.083 \\ 
  1135 & 151.302509 &  -7.748353 &     21.585 $\pm$   0.050 &    21.561 $\pm$   0.051 &    21.558 $\pm$   0.064 &      0.900 \\ 
  1136 & 151.280218 &  -7.748705 &     20.019 $\pm$   0.015 &    19.909 $\pm$   0.013 &    19.521 $\pm$   0.012 &      0.967 \\ 
  1137 & 151.263681 &  -7.748734 &     22.379 $\pm$   0.084 &    22.372 $\pm$   0.095 &    22.099 $\pm$   0.093 &      0.297 \\ 
  1138 & 151.283979 &  -7.748815 &     21.456 $\pm$   0.050 &    21.379 $\pm$   0.045 &    21.471 $\pm$   0.065 &      0.943 \\ 
  1139 & 151.309253 &  -7.748878 &     22.248 $\pm$   0.083 &    22.033 $\pm$   0.074 &    21.265 $\pm$   0.046 &      0.653 \\ 
  1140 & 151.305287 &  -7.748931 &     21.875 $\pm$   0.062 &    21.864 $\pm$   0.065 &    21.473 $\pm$   0.058 &      0.897 \\ 
  1141 & 151.348641 &  -7.749333 &     17.671 $\pm$   0.004 &    17.705 $\pm$   0.003 &    17.865 $\pm$   0.003 &      0.983 \\ 
  1142 & 151.272259 &  -7.749279 &     22.664 $\pm$   0.125 &    22.648 $\pm$   0.132 &    22.275 $\pm$   0.122 &      0.517 \\ 
  1143 & 151.247554 &  -7.749834 &     17.723 $\pm$   0.004 &    17.767 $\pm$   0.003 &    17.937 $\pm$   0.003 &      0.980 \\ 
  1144 & 151.277143 &  -7.749758 &     20.152 $\pm$   0.016 &    20.189 $\pm$   0.016 &    20.231 $\pm$   0.021 &      0.623 \\ 
  1145 & 151.297522 &  -7.749822 &     19.176 $\pm$   0.009 &    19.207 $\pm$   0.008 &    19.403 $\pm$   0.010 &      0.980 \\ 
  1146 & 151.291168 &  -7.749882 &     18.530 $\pm$   0.006 &    18.701 $\pm$   0.005 &    19.069 $\pm$   0.008 &      0.980 \\ 
  1147 & 151.315541 &  -7.749869 &     20.981 $\pm$   0.027 &    20.862 $\pm$   0.026 &    20.394 $\pm$   0.021 &      0.117 \\ 
  1148 & 151.284350 &  -7.749850 &     21.717 $\pm$   0.062 &    21.443 $\pm$   0.048 &    20.869 $\pm$   0.037 &      0.313 \\ 
  1149 & 151.295720 &  -7.749773 &     22.534 $\pm$   0.122 &    22.380 $\pm$   0.108 &    22.181 $\pm$   0.118 &      0.603 \\ 
  1150 & 151.355113 &  -7.750057 &     18.621 $\pm$   0.005 &    18.718 $\pm$   0.005 &    19.087 $\pm$   0.007 &      0.980 \\ 
  1151 & 151.265861 &  -7.750005 &     22.129 $\pm$   0.069 &    21.826 $\pm$   0.060 &    20.927 $\pm$   0.034 &      0.210 \\ 
  1152 & 151.258527 &  -7.750366 &     20.676 $\pm$   0.019 &    20.927 $\pm$   0.026 &    20.485 $\pm$   0.020 &      0.083 \\ 
  1153 & 151.252668 &  -7.750267 &     22.181 $\pm$   0.063 &    21.879 $\pm$   0.055 &    21.233 $\pm$   0.036 &      0.897 \\ 
  1154 & 151.365161 &  -7.750357 &     20.252 $\pm$   0.013 &    20.510 $\pm$   0.017 &    20.857 $\pm$   0.026 &      0.980 \\ 
  1155 & 151.334984 &  -7.750437 &     22.622 $\pm$   0.096 &    22.629 $\pm$   0.112 &    21.906 $\pm$   0.068 &      0.350 \\ 
  1156 & 151.254142 &  -7.751090 &     21.109 $\pm$   0.026 &    21.528 $\pm$   0.041 &    20.905 $\pm$   0.028 &      0.013 \\ 
  1157 & 151.371243 &  -7.750815 &     22.579 $\pm$   0.084 &    22.739 $\pm$   0.111 &    22.259 $\pm$   0.084 &      0.697 \\ 
  1158 & 151.264620 &  -7.751009 &     22.066 $\pm$   0.064 &    22.293 $\pm$   0.088 &    22.465 $\pm$   0.129 &      0.667 \\ 
  1159 & 151.357209 &  -7.751210 &     19.246 $\pm$   0.007 &    19.256 $\pm$   0.007 &    19.482 $\pm$   0.009 &      0.980 \\ 
  1160 & 151.311954 &  -7.751333 &     20.977 $\pm$   0.027 &    20.793 $\pm$   0.024 &    21.001 $\pm$   0.035 &      0.977 \\ 
  1161 & 151.312417 &  -7.751364 &     20.916 $\pm$   0.025 &    20.977 $\pm$   0.029 &    20.437 $\pm$   0.022 &      0.023 \\ 
  1162 & 151.250737 &  -7.751525 &     20.916 $\pm$   0.022 &    21.002 $\pm$   0.026 &    20.110 $\pm$   0.015 &      0.023 \\ 
  1163 & 151.264400 &  -7.751367 &     20.949 $\pm$   0.025 &    21.087 $\pm$   0.031 &    21.183 $\pm$   0.041 &      0.973 \\ 
  1164 & 151.273333 &  -7.751667 &     21.662 $\pm$   0.052 &    21.692 $\pm$   0.056 &    21.699 $\pm$   0.072 &      0.803 \\ 
  1165 & 151.256477 &  -7.751899 &     21.251 $\pm$   0.030 &    21.331 $\pm$   0.035 &    21.444 $\pm$   0.045 &      0.590 \\ 
  1166 & 151.328012 &  -7.752142 &     19.895 $\pm$   0.011 &    19.897 $\pm$   0.011 &    20.073 $\pm$   0.015 &      0.977 \\ 
  1167 & 151.303393 &  -7.752277 &     20.415 $\pm$   0.018 &    20.287 $\pm$   0.017 &    19.685 $\pm$   0.012 &      0.170 \\ 
  1168 & 151.299916 &  -7.752370 &     20.417 $\pm$   0.019 &    20.351 $\pm$   0.018 &    20.489 $\pm$   0.024 &      0.980 \\ 
  1169 & 151.312708 &  -7.752554 &     21.493 $\pm$   0.040 &    21.427 $\pm$   0.042 &    21.160 $\pm$   0.040 &      0.370 \\ 
  1170 & 151.348523 &  -7.752461 &     22.954 $\pm$   0.122 &    22.540 $\pm$   0.098 &    21.895 $\pm$   0.062 &      0.510 \\ 
  1171 & 151.304156 &  -7.752544 &     22.514 $\pm$   0.103 &    22.604 $\pm$   0.123 &    21.760 $\pm$   0.072 &      0.577 \\ 
  1172 & 151.269831 &  -7.752862 &     19.955 $\pm$   0.013 &    20.009 $\pm$   0.013 &    20.157 $\pm$   0.018 &      0.980 \\ 
  1173 & 151.370058 &  -7.753082 &     22.025 $\pm$   0.051 &    22.261 $\pm$   0.073 &    22.684 $\pm$   0.123 &      0.737 \\ 
  1174 & 151.314122 &  -7.753194 &     22.426 $\pm$   0.088 &    22.661 $\pm$   0.123 &    22.123 $\pm$   0.092 &      0.563 \\ 
  1175 & 151.311034 &  -7.753334 &     22.124 $\pm$   0.069 &    22.184 $\pm$   0.081 &    21.882 $\pm$   0.075 &      0.183 \\ 
  1176 & 151.279585 &  -7.753404 &     20.659 $\pm$   0.023 &    20.566 $\pm$   0.021 &    20.770 $\pm$   0.032 &      0.977 \\ 
  1177 & 151.328768 &  -7.753400 &     22.051 $\pm$   0.059 &    22.210 $\pm$   0.078 &    21.717 $\pm$   0.059 &      0.237 \\ 
  1178 & 151.272751 &  -7.753444 &     21.889 $\pm$   0.061 &    21.983 $\pm$   0.071 &    21.342 $\pm$   0.051 &      0.030 \\ 
  1179 & 151.355464 &  -7.753551 &     20.648 $\pm$   0.018 &    20.689 $\pm$   0.020 &    20.378 $\pm$   0.018 &      0.143 \\ 
  1180 & 151.277930 &  -7.753456 &     22.494 $\pm$   0.111 &    22.716 $\pm$   0.141 &    22.190 $\pm$   0.114 &      0.547 \\ 
  1181 & 151.323133 &  -7.753679 &     22.349 $\pm$   0.078 &    22.330 $\pm$   0.088 &    21.386 $\pm$   0.045 &      0.160 \\ 
  1182 & 151.338797 &  -7.753801 &     21.332 $\pm$   0.031 &    21.309 $\pm$   0.034 &    21.585 $\pm$   0.050 &      0.947 \\ 
  1183 & 151.359905 &  -7.753900 &     22.418 $\pm$   0.072 &    22.080 $\pm$   0.063 &    21.654 $\pm$   0.050 &      0.863 \\ 
  1184 & 151.355429 &  -7.754465 &     17.233 $\pm$   0.003 &    17.089 $\pm$   0.002 &    17.352 $\pm$   0.002 &      0.983 \\ 
  1185 & 151.310016 &  -7.754328 &     21.459 $\pm$   0.039 &    21.654 $\pm$   0.051 &    20.834 $\pm$   0.030 &      0.010 \\ 
  1186 & 151.291594 &  -7.754271 &     22.600 $\pm$   0.121 &    22.712 $\pm$   0.140 &    21.882 $\pm$   0.085 &      0.450 \\ 
  1187 & 151.247933 &  -7.755377 &     20.267 $\pm$   0.013 &    20.211 $\pm$   0.014 &    19.531 $\pm$   0.009 &      0.030 \\ 
  1188 & 151.286056 &  -7.755407 &     21.980 $\pm$   0.069 &    21.779 $\pm$   0.060 &    21.527 $\pm$   0.062 &      0.880 \\ 
  1189 & 151.286770 &  -7.755665 &     22.142 $\pm$   0.079 &    21.999 $\pm$   0.073 &    21.471 $\pm$   0.058 &      0.890 \\ 
  1190 & 151.272784 &  -7.755729 &     22.541 $\pm$   0.105 &    22.674 $\pm$   0.130 &    22.404 $\pm$   0.130 &      0.500 \\ 
  1191 & 151.270152 &  -7.755776 &     22.512 $\pm$   0.099 &    22.539 $\pm$   0.113 &    22.232 $\pm$   0.108 &      0.637 \\ 
  1192 & 151.257841 &  -7.756417 &     14.911 $\pm$   0.002 &    15.056 $\pm$   0.001 &    15.376 $\pm$   0.001 &      0.987 \\ 
  1193 & 151.264436 &  -7.756047 &     22.080 $\pm$   0.063 &    21.790 $\pm$   0.055 &    21.038 $\pm$   0.034 &      0.177 \\ 
  1194 & 151.355201 &  -7.756580 &     16.109 $\pm$   0.002 &    16.015 $\pm$   0.001 &    16.264 $\pm$   0.001 &      0.990 \\ 
  1195 & 151.290645 &  -7.756201 &     22.580 $\pm$   0.114 &    22.700 $\pm$   0.136 &    22.391 $\pm$   0.131 &      0.593 \\ 
  1196 & 151.325317 &  -7.756208 &     22.343 $\pm$   0.076 &    22.625 $\pm$   0.113 &    21.931 $\pm$   0.072 &      0.363 \\ 
  1197 & 151.323034 &  -7.756373 &     20.896 $\pm$   0.023 &    20.804 $\pm$   0.023 &    20.149 $\pm$   0.016 &      0.347 \\ 
  1198 & 151.292770 &  -7.756525 &     21.587 $\pm$   0.047 &    21.643 $\pm$   0.052 &    20.999 $\pm$   0.037 &      0.210 \\ 
  1199 & 151.344968 &  -7.756949 &     20.970 $\pm$   0.023 &    21.125 $\pm$   0.029 &    20.532 $\pm$   0.020 &      0.020 \\ 
  1200 & 151.348492 &  -7.756974 &     20.534 $\pm$   0.016 &    20.444 $\pm$   0.017 &    19.951 $\pm$   0.013 &      0.093 \\ 
  1201 & 151.263319 &  -7.757036 &     23.048 $\pm$   0.145 &    22.770 $\pm$   0.129 &    22.223 $\pm$   0.094 &      0.597 \\ 
  1202 & 151.339519 &  -7.757144 &     19.263 $\pm$   0.007 &    19.287 $\pm$   0.007 &    19.493 $\pm$   0.009 &      0.983 \\ 
  1203 & 151.315700 &  -7.755941 &     22.800 $\pm$   0.119 &    22.893 $\pm$   0.149 &    22.295 $\pm$   0.104 &      0.440 \\ 
  1204 & 151.353957 &  -7.757046 &     22.502 $\pm$   0.079 &    22.746 $\pm$   0.114 &    22.041 $\pm$   0.070 &      0.010 \\ 
  1205 & 151.284411 &  -7.757245 &     22.525 $\pm$   0.109 &    22.431 $\pm$   0.106 &    22.205 $\pm$   0.110 &      0.627 \\ 
  1206 & 151.292925 &  -7.757461 &     20.439 $\pm$   0.018 &    20.460 $\pm$   0.019 &    20.765 $\pm$   0.030 &      0.983 \\ 
  1207 & 151.326477 &  -7.757427 &     21.433 $\pm$   0.035 &    21.672 $\pm$   0.048 &    22.083 $\pm$   0.081 &      0.893 \\ 
  1208 & 151.297992 &  -7.757437 &     22.024 $\pm$   0.065 &    21.963 $\pm$   0.068 &    22.248 $\pm$   0.108 &      0.783 \\ 
  1209 & 151.344827 &  -7.757682 &     20.644 $\pm$   0.018 &    20.795 $\pm$   0.022 &    21.234 $\pm$   0.035 &      0.967 \\ 
  1210 & 151.373307 &  -7.757556 &     23.175 $\pm$   0.142 &    22.744 $\pm$   0.112 &    21.554 $\pm$   0.045 &      0.497 \\ 
  1211 & 151.291569 &  -7.757635 &     23.063 $\pm$   0.169 &    22.894 $\pm$   0.158 &    22.571 $\pm$   0.149 &      0.500 \\ 
  1212 & 151.310172 &  -7.757816 &     23.072 $\pm$   0.153 &    22.909 $\pm$   0.152 &    22.214 $\pm$   0.098 &      0.647 \\ 
  1213 & 151.326106 &  -7.758045 &     21.396 $\pm$   0.034 &    21.374 $\pm$   0.037 &    20.638 $\pm$   0.023 &      0.017 \\ 
  1214 & 151.352535 &  -7.758113 &     22.470 $\pm$   0.077 &    22.625 $\pm$   0.102 &    21.788 $\pm$   0.056 &      0.357 \\ 
  1215 & 151.350296 &  -7.758435 &     20.220 $\pm$   0.013 &    20.234 $\pm$   0.014 &    20.465 $\pm$   0.019 &      0.973 \\ 
  1216 & 151.299509 &  -7.758768 &     20.945 $\pm$   0.025 &    21.007 $\pm$   0.029 &    21.106 $\pm$   0.038 &      0.937 \\ 
  1217 & 151.306777 &  -7.758739 &     21.242 $\pm$   0.031 &    21.442 $\pm$   0.041 &    21.672 $\pm$   0.061 &      0.963 \\ 
  1218 & 151.300599 &  -7.758844 &     20.463 $\pm$   0.018 &    20.365 $\pm$   0.017 &    20.530 $\pm$   0.023 &      0.980 \\ 
  1219 & 151.295627 &  -7.759140 &     20.880 $\pm$   0.025 &    20.369 $\pm$   0.017 &    19.557 $\pm$   0.011 &      0.083 \\ 
  1220 & 151.358686 &  -7.759107 &     19.310 $\pm$   0.008 &    19.237 $\pm$   0.007 &    19.500 $\pm$   0.009 &      0.980 \\ 
  1221 & 151.322406 &  -7.758916 &     22.942 $\pm$   0.129 &    22.823 $\pm$   0.136 &    22.690 $\pm$   0.140 &      0.510 \\ 
  1222 & 151.250146 &  -7.759420 &     20.311 $\pm$   0.014 &    20.310 $\pm$   0.015 &    19.570 $\pm$   0.010 &      0.030 \\ 
  1223 & 151.256404 &  -7.759182 &     21.922 $\pm$   0.050 &    22.133 $\pm$   0.068 &    21.496 $\pm$   0.046 &      0.040 \\ 
  1224 & 151.248304 &  -7.759367 &     21.495 $\pm$   0.033 &    21.365 $\pm$   0.034 &    20.512 $\pm$   0.019 &      0.260 \\ 
  1225 & 151.300645 &  -7.759472 &     19.997 $\pm$   0.012 &    19.924 $\pm$   0.012 &    20.105 $\pm$   0.016 &      0.980 \\ 
  1226 & 151.251899 &  -7.759674 &     22.276 $\pm$   0.066 &    22.143 $\pm$   0.067 &    21.677 $\pm$   0.053 &      0.107 \\ 
  1227 & 151.319441 &  -7.759875 &     22.308 $\pm$   0.074 &    22.243 $\pm$   0.081 &    21.652 $\pm$   0.056 &      0.183 \\ 
  1228 & 151.309692 &  -7.760007 &     21.127 $\pm$   0.028 &    21.100 $\pm$   0.031 &    21.531 $\pm$   0.053 &      0.740 \\ 
  1229 & 151.366431 &  -7.760037 &     22.518 $\pm$   0.079 &    22.556 $\pm$   0.095 &    22.093 $\pm$   0.073 &      0.440 \\ 
  1230 & 151.360653 &  -7.760115 &     21.735 $\pm$   0.040 &    21.862 $\pm$   0.052 &    22.402 $\pm$   0.095 &      0.813 \\ 
  1231 & 151.344495 &  -7.760084 &     23.119 $\pm$   0.139 &    22.879 $\pm$   0.131 &    22.782 $\pm$   0.136 &      0.477 \\ 
  1232 & 151.245876 &  -7.760301 &     20.926 $\pm$   0.021 &    21.029 $\pm$   0.026 &    22.381 $\pm$   0.086 &      0.877 \\ 
  1233 & 151.286845 &  -7.760459 &     21.362 $\pm$   0.037 &    21.437 $\pm$   0.042 &    21.466 $\pm$   0.054 &      0.920 \\ 
  1234 & 151.299886 &  -7.760794 &     16.630 $\pm$   0.003 &    16.544 $\pm$   0.002 &    16.841 $\pm$   0.002 &      0.980 \\ 
  1235 & 151.326717 &  -7.760482 &     22.205 $\pm$   0.066 &    21.822 $\pm$   0.055 &    21.366 $\pm$   0.042 &      0.763 \\ 
  1236 & 151.329298 &  -7.760497 &     23.052 $\pm$   0.138 &    22.913 $\pm$   0.143 &    22.414 $\pm$   0.106 &      0.560 \\ 
  1237 & 151.275563 &  -7.760685 &     22.389 $\pm$   0.088 &    22.394 $\pm$   0.098 &    21.743 $\pm$   0.068 &      0.497 \\ 
  1238 & 151.369316 &  -7.760960 &     20.519 $\pm$   0.016 &    20.385 $\pm$   0.016 &    19.991 $\pm$   0.013 &      0.223 \\ 
  1239 & 151.354196 &  -7.760836 &     23.106 $\pm$   0.133 &    22.844 $\pm$   0.123 &    21.969 $\pm$   0.065 &      0.467 \\ 
  1240 & 151.257864 &  -7.760942 &     22.918 $\pm$   0.119 &    23.039 $\pm$   0.152 &    22.558 $\pm$   0.118 &      0.480 \\ 
  1241 & 151.333416 &  -7.761235 &     19.542 $\pm$   0.009 &    19.541 $\pm$   0.009 &    19.758 $\pm$   0.011 &      0.980 \\ 
  1242 & 151.331887 &  -7.761412 &     20.515 $\pm$   0.016 &    20.475 $\pm$   0.017 &    20.691 $\pm$   0.024 &      0.977 \\ 
  1243 & 151.320101 &  -7.761596 &     22.978 $\pm$   0.132 &    22.898 $\pm$   0.144 &    22.615 $\pm$   0.131 &      0.437 \\ 
  1244 & 151.295457 &  -7.761870 &     22.236 $\pm$   0.074 &    22.374 $\pm$   0.095 &    21.811 $\pm$   0.070 &      0.547 \\ 
  1245 & 151.268963 &  -7.762279 &     18.197 $\pm$   0.005 &    18.198 $\pm$   0.004 &    18.432 $\pm$   0.005 &      0.980 \\ 
  1246 & 151.287042 &  -7.762134 &     21.985 $\pm$   0.061 &    21.514 $\pm$   0.045 &    20.935 $\pm$   0.033 &      0.933 \\ 
  1247 & 151.343616 &  -7.762164 &     21.651 $\pm$   0.039 &    21.476 $\pm$   0.038 &    20.902 $\pm$   0.027 &      0.073 \\ 
  1248 & 151.325115 &  -7.762377 &     21.533 $\pm$   0.037 &    21.274 $\pm$   0.034 &    20.561 $\pm$   0.021 &      0.070 \\ 
  1249 & 151.309014 &  -7.762333 &     21.905 $\pm$   0.053 &    21.999 $\pm$   0.066 &    22.572 $\pm$   0.131 &      0.797 \\ 
  1250 & 151.313092 &  -7.762401 &     20.888 $\pm$   0.023 &    20.920 $\pm$   0.026 &    21.108 $\pm$   0.035 &      0.790 \\ 
  1251 & 151.366356 &  -7.762681 &     19.175 $\pm$   0.007 &    19.081 $\pm$   0.006 &    18.671 $\pm$   0.005 &      0.060 \\ 
  1252 & 151.287968 &  -7.762496 &     21.914 $\pm$   0.057 &    22.246 $\pm$   0.085 &    22.187 $\pm$   0.100 &      0.847 \\ 
  1253 & 151.267917 &  -7.762731 &     20.776 $\pm$   0.021 &    20.796 $\pm$   0.023 &    20.889 $\pm$   0.029 &      0.960 \\ 
  1254 & 151.251246 &  -7.762680 &     22.316 $\pm$   0.067 &    22.656 $\pm$   0.106 &    22.495 $\pm$   0.107 &      0.487 \\ 
  1255 & 151.371748 &  -7.763668 &     20.157 $\pm$   0.012 &    20.005 $\pm$   0.012 &    19.485 $\pm$   0.009 &      0.090 \\ 
  1256 & 151.321458 &  -7.763690 &     22.541 $\pm$   0.088 &    22.792 $\pm$   0.129 &    22.460 $\pm$   0.111 &      0.423 \\ 
  1257 & 151.299955 &  -7.763816 &     21.297 $\pm$   0.032 &    21.566 $\pm$   0.046 &    21.177 $\pm$   0.039 &      0.090 \\ 
  1258 & 151.314110 &  -7.763423 &     22.615 $\pm$   0.097 &    22.389 $\pm$   0.092 &    21.744 $\pm$   0.061 &      0.557 \\ 
  1259 & 151.289002 &  -7.763832 &     22.367 $\pm$   0.083 &    22.497 $\pm$   0.106 &    22.516 $\pm$   0.131 &      0.677 \\ 
  1260 & 151.252153 &  -7.763979 &     20.456 $\pm$   0.015 &    20.557 $\pm$   0.018 &    20.803 $\pm$   0.025 &      0.973 \\ 
  1261 & 151.356870 &  -7.764107 &     20.374 $\pm$   0.014 &    20.264 $\pm$   0.014 &    19.781 $\pm$   0.011 &      0.190 \\ 
  1262 & 151.342358 &  -7.764468 &     21.948 $\pm$   0.049 &    22.069 $\pm$   0.063 &    22.305 $\pm$   0.088 &      0.777 \\ 
  1263 & 151.296026 &  -7.764744 &     20.877 $\pm$   0.023 &    20.794 $\pm$   0.024 &    20.903 $\pm$   0.030 &      0.977 \\ 
  1264 & 151.312617 &  -7.764715 &     22.593 $\pm$   0.095 &    22.408 $\pm$   0.094 &    21.715 $\pm$   0.059 &      0.590 \\ 
  1265 & 151.358017 &  -7.764980 &     21.170 $\pm$   0.025 &    21.034 $\pm$   0.026 &    20.407 $\pm$   0.018 &      0.063 \\ 
  1266 & 151.280913 &  -7.765183 &     21.503 $\pm$   0.039 &    21.625 $\pm$   0.048 &    21.535 $\pm$   0.054 &      0.603 \\ 
  1267 & 151.296300 &  -7.765782 &     20.663 $\pm$   0.020 &    20.767 $\pm$   0.023 &    20.104 $\pm$   0.016 &      0.020 \\ 
  1268 & 151.353635 &  -7.765724 &     22.680 $\pm$   0.090 &    22.977 $\pm$   0.138 &    22.891 $\pm$   0.148 &      0.543 \\ 
  1269 & 151.360969 &  -7.765987 &     21.300 $\pm$   0.028 &    21.427 $\pm$   0.036 &    20.743 $\pm$   0.023 &      0.010 \\ 
  1270 & 151.277784 &  -7.766295 &     22.286 $\pm$   0.075 &    22.504 $\pm$   0.104 &    21.797 $\pm$   0.066 &      0.123 \\ 
  1271 & 151.254352 &  -7.766653 &     22.025 $\pm$   0.052 &    21.941 $\pm$   0.056 &    21.401 $\pm$   0.041 &      0.180 \\ 
  1272 & 151.371965 &  -7.766776 &     21.394 $\pm$   0.031 &    21.304 $\pm$   0.033 &    20.705 $\pm$   0.023 &      0.017 \\ 
  1273 & 151.318934 &  -7.766999 &     22.132 $\pm$   0.061 &    21.873 $\pm$   0.057 &    21.266 $\pm$   0.038 &      0.380 \\ 
  1274 & 151.336301 &  -7.767075 &     21.950 $\pm$   0.050 &    21.913 $\pm$   0.056 &    21.618 $\pm$   0.050 &      0.560 \\ 
  1275 & 151.254349 &  -7.767311 &     21.313 $\pm$   0.029 &    21.442 $\pm$   0.037 &    21.090 $\pm$   0.032 &      0.033 \\ 
  1276 & 151.317040 &  -7.767165 &     22.220 $\pm$   0.066 &    22.307 $\pm$   0.084 &    21.609 $\pm$   0.052 &      0.333 \\ 
  1277 & 151.291375 &  -7.767457 &     22.667 $\pm$   0.103 &    22.779 $\pm$   0.133 &    22.460 $\pm$   0.118 &      0.550 \\ 
  1278 & 151.357930 &  -7.767631 &     22.984 $\pm$   0.119 &    22.653 $\pm$   0.103 &    21.906 $\pm$   0.062 &      0.513 \\ 
  1279 & 151.351235 &  -7.768150 &     21.410 $\pm$   0.031 &    21.432 $\pm$   0.036 &    21.587 $\pm$   0.047 &      0.907 \\ 
  1280 & 151.280945 &  -7.768130 &     22.803 $\pm$   0.116 &    22.876 $\pm$   0.144 &    22.447 $\pm$   0.116 &      0.547 \\ 
  1281 & 151.262155 &  -7.768384 &     22.847 $\pm$   0.110 &    22.788 $\pm$   0.121 &    22.708 $\pm$   0.136 &      0.570 \\ 
  1282 & 151.249505 &  -7.768624 &     22.835 $\pm$   0.103 &    23.047 $\pm$   0.146 &    22.711 $\pm$   0.126 &      0.567 \\ 
  1283 & 151.262022 &  -7.768823 &     21.323 $\pm$   0.030 &    21.894 $\pm$   0.055 &    21.336 $\pm$   0.040 &      0.003 \\ 
  1284 & 151.352273 &  -7.769133 &     21.732 $\pm$   0.040 &    21.638 $\pm$   0.043 &    21.188 $\pm$   0.034 &      0.267 \\ 
  1285 & 151.247333 &  -7.769472 &     20.068 $\pm$   0.011 &    20.203 $\pm$   0.014 &    20.763 $\pm$   0.024 &      0.960 \\ 
  1286 & 151.293376 &  -7.769271 &     21.229 $\pm$   0.030 &    21.121 $\pm$   0.030 &    20.564 $\pm$   0.022 &      0.150 \\ 
  1287 & 151.266493 &  -7.769271 &     22.572 $\pm$   0.087 &    22.577 $\pm$   0.101 &    22.536 $\pm$   0.117 &      0.627 \\ 
  1288 & 151.259853 &  -7.769406 &     22.413 $\pm$   0.073 &    22.361 $\pm$   0.081 &    21.943 $\pm$   0.068 &      0.680 \\ 
  1289 & 151.373176 &  -7.769970 &     20.448 $\pm$   0.015 &    20.364 $\pm$   0.015 &    19.718 $\pm$   0.011 &      0.040 \\ 
  1290 & 151.260766 &  -7.770219 &     22.010 $\pm$   0.052 &    22.269 $\pm$   0.075 &    22.709 $\pm$   0.134 &      0.797 \\ 
  1291 & 151.311214 &  -7.769768 &     22.084 $\pm$   0.059 &    22.035 $\pm$   0.066 &    21.974 $\pm$   0.072 &      0.367 \\ 
  1292 & 151.311306 &  -7.770521 &     20.495 $\pm$   0.017 &    20.595 $\pm$   0.020 &    20.037 $\pm$   0.014 &      0.027 \\ 
  1293 & 151.320052 &  -7.770105 &     19.527 $\pm$   0.009 &    19.658 $\pm$   0.010 &    19.411 $\pm$   0.009 &      0.063 \\ 
  1294 & 151.357663 &  -7.769864 &     22.968 $\pm$   0.118 &    23.088 $\pm$   0.152 &    22.868 $\pm$   0.145 &      0.480 \\ 
  1295 & 151.260948 &  -7.769727 &     22.381 $\pm$   0.072 &    22.328 $\pm$   0.079 &    21.757 $\pm$   0.058 &      0.600 \\ 
  1296 & 151.278583 &  -7.770214 &     23.091 $\pm$   0.145 &    22.878 $\pm$   0.140 &    22.572 $\pm$   0.125 &      0.477 \\ 
  1297 & 151.254748 &  -7.770405 &     22.083 $\pm$   0.054 &    22.439 $\pm$   0.086 &    22.022 $\pm$   0.070 &      0.117 \\ 
  1298 & 151.295444 &  -7.770650 &     21.898 $\pm$   0.051 &    21.744 $\pm$   0.052 &    21.170 $\pm$   0.036 &      0.873 \\ 
  1299 & 151.308813 &  -7.770866 &     22.577 $\pm$   0.090 &    22.848 $\pm$   0.135 &    22.450 $\pm$   0.110 &      0.687 \\ 
  1300 & 151.364864 &  -7.770939 &     23.349 $\pm$   0.165 &    23.054 $\pm$   0.148 &    22.188 $\pm$   0.079 &      0.400 \\ 
  1301 & 151.262452 &  -7.771140 &     21.552 $\pm$   0.035 &    21.873 $\pm$   0.053 &    22.222 $\pm$   0.087 &      0.670 \\ 
  1302 & 151.359516 &  -7.771158 &     22.584 $\pm$   0.083 &    22.912 $\pm$   0.130 &    22.561 $\pm$   0.110 &      0.493 \\ 
  1303 & 151.301542 &  -7.772842 &     13.141 $\pm$   0.001 &    12.844 $\pm$   0.000 &    13.530 $\pm$   0.001 &      1.000 \\ 
  1304 & 151.277400 &  -7.771345 &     22.347 $\pm$   0.074 &    22.503 $\pm$   0.099 &    22.686 $\pm$   0.137 &      0.307 \\ 
  1305 & 151.317173 &  -7.771449 &     22.034 $\pm$   0.055 &    22.143 $\pm$   0.071 &    22.450 $\pm$   0.108 &      0.853 \\ 
  1306 & 151.264114 &  -7.771549 &     22.110 $\pm$   0.057 &    22.272 $\pm$   0.076 &    22.510 $\pm$   0.113 &      0.710 \\ 
  1307 & 151.311833 &  -7.771685 &     21.271 $\pm$   0.030 &    21.205 $\pm$   0.032 &    20.588 $\pm$   0.022 &      0.113 \\ 
  1308 & 151.266531 &  -7.771728 &     21.469 $\pm$   0.033 &    21.684 $\pm$   0.046 &    21.771 $\pm$   0.059 &      0.820 \\ 
  1309 & 151.344939 &  -7.771642 &     22.478 $\pm$   0.076 &    22.059 $\pm$   0.061 &    21.643 $\pm$   0.049 &      0.787 \\ 
  1310 & 151.339474 &  -7.772238 &     22.075 $\pm$   0.054 &    22.370 $\pm$   0.082 &    21.945 $\pm$   0.064 &      0.120 \\ 
  1311 & 151.289213 &  -7.772310 &     20.201 $\pm$   0.013 &    20.310 $\pm$   0.015 &    20.564 $\pm$   0.022 &      0.963 \\ 
  1312 & 151.348412 &  -7.772569 &     20.438 $\pm$   0.015 &    20.551 $\pm$   0.018 &    20.981 $\pm$   0.028 &      0.973 \\ 
  1313 & 151.278523 &  -7.772846 &     21.280 $\pm$   0.030 &    23.165 $\pm$   0.177 &    22.231 $\pm$   0.090 &      0.727 \\ 
  1314 & 151.297798 &  -7.772825 &     21.819 $\pm$   0.046 &    22.554 $\pm$   0.104 &    21.710 $\pm$   0.057 &      0.780 \\ 
  1315 & 151.305465 &  -7.772835 &     21.354 $\pm$   0.031 &    22.099 $\pm$   0.069 &    21.632 $\pm$   0.053 &      0.927 \\ 
  1316 & 151.252551 &  -7.772888 &     22.378 $\pm$   0.069 &    22.541 $\pm$   0.093 &    22.491 $\pm$   0.104 &      0.583 \\ 
  1317 & 151.351776 &  -7.773146 &     21.472 $\pm$   0.033 &    21.509 $\pm$   0.039 &    21.038 $\pm$   0.030 &      0.017 \\ 
  1318 & 151.261889 &  -7.771261 &     22.370 $\pm$   0.070 &    22.398 $\pm$   0.084 &    21.972 $\pm$   0.070 &      0.660 \\ 
  1319 & 151.329512 &  -7.773225 &     19.980 $\pm$   0.011 &    20.011 $\pm$   0.012 &    20.082 $\pm$   0.014 &      0.413 \\ 
  1320 & 151.339850 &  -7.773166 &     20.196 $\pm$   0.013 &    20.212 $\pm$   0.014 &    20.442 $\pm$   0.018 &      0.977 \\ 
  1321 & 151.287500 &  -7.773146 &     21.839 $\pm$   0.047 &    22.116 $\pm$   0.071 &    22.242 $\pm$   0.091 &      0.820 \\ 
  1322 & 151.371814 &  -7.773263 &     22.612 $\pm$   0.085 &    22.395 $\pm$   0.082 &    21.615 $\pm$   0.048 &      0.690 \\ 
  1323 & 151.349658 &  -7.773808 &     19.246 $\pm$   0.007 &    19.184 $\pm$   0.007 &    18.778 $\pm$   0.006 &      0.033 \\ 
  1324 & 151.370094 &  -7.773318 &     23.279 $\pm$   0.154 &    22.952 $\pm$   0.134 &    22.101 $\pm$   0.073 &      0.373 \\ 
  1325 & 151.274847 &  -7.773610 &     22.252 $\pm$   0.066 &    22.547 $\pm$   0.099 &    22.275 $\pm$   0.093 &      0.190 \\ 
  1326 & 151.266732 &  -7.773765 &     22.168 $\pm$   0.059 &    22.299 $\pm$   0.077 &    21.819 $\pm$   0.061 &      0.630 \\ 
  1327 & 151.269907 &  -7.773811 &     21.518 $\pm$   0.035 &    21.556 $\pm$   0.041 &    20.619 $\pm$   0.022 &      0.073 \\ 
  1328 & 151.296840 &  -7.774017 &     22.006 $\pm$   0.054 &    22.028 $\pm$   0.065 &    21.446 $\pm$   0.045 &      0.017 \\ 
  1329 & 151.324936 &  -7.773962 &     21.426 $\pm$   0.033 &    21.760 $\pm$   0.049 &    21.107 $\pm$   0.033 &      0.007 \\ 
  1330 & 151.320895 &  -7.774277 &     21.992 $\pm$   0.052 &    22.398 $\pm$   0.087 &    22.115 $\pm$   0.080 &      0.050 \\ 
  1331 & 151.252696 &  -7.774413 &     22.121 $\pm$   0.055 &    21.970 $\pm$   0.057 &    21.764 $\pm$   0.055 &      0.177 \\ 
  1332 & 151.330155 &  -7.774483 &     21.632 $\pm$   0.038 &    21.700 $\pm$   0.046 &    21.257 $\pm$   0.037 &      0.210 \\ 
  1333 & 151.372802 &  -7.774662 &     21.937 $\pm$   0.048 &    22.067 $\pm$   0.062 &    21.740 $\pm$   0.053 &      0.643 \\ 
  1334 & 151.289680 &  -7.774808 &     21.688 $\pm$   0.041 &    21.696 $\pm$   0.048 &    21.042 $\pm$   0.032 &      0.117 \\ 
  1335 & 151.318890 &  -7.774779 &     22.061 $\pm$   0.055 &    22.069 $\pm$   0.065 &    21.686 $\pm$   0.055 &      0.797 \\ 
  1336 & 151.285673 &  -7.774793 &     22.968 $\pm$   0.126 &    22.901 $\pm$   0.139 &    22.707 $\pm$   0.138 &      0.490 \\ 
  1337 & 151.353621 &  -7.771371 &     20.719 $\pm$   0.018 &    20.624 $\pm$   0.019 &    20.286 $\pm$   0.016 &      0.327 \\ 
  1338 & 151.264049 &  -7.775272 &     20.669 $\pm$   0.018 &    20.787 $\pm$   0.022 &    21.045 $\pm$   0.031 &      0.557 \\ 
  1339 & 151.332279 &  -7.775011 &     20.809 $\pm$   0.020 &    20.797 $\pm$   0.022 &    20.891 $\pm$   0.027 &      0.970 \\ 
  1340 & 151.253135 &  -7.775317 &     22.399 $\pm$   0.070 &    22.630 $\pm$   0.101 &    22.536 $\pm$   0.107 &      0.280 \\ 
  1341 & 151.286556 &  -7.775683 &     17.930 $\pm$   0.004 &    17.990 $\pm$   0.003 &    18.354 $\pm$   0.004 &      0.983 \\ 
  1342 & 151.354648 &  -7.775535 &     22.519 $\pm$   0.079 &    22.500 $\pm$   0.090 &    22.833 $\pm$   0.141 &      0.627 \\ 
  1343 & 151.348561 &  -7.775607 &     22.217 $\pm$   0.061 &    22.059 $\pm$   0.061 &    22.185 $\pm$   0.079 &      0.767 \\ 
  1344 & 151.353972 &  -7.775828 &     22.244 $\pm$   0.062 &    22.514 $\pm$   0.092 &    22.379 $\pm$   0.094 &      0.573 \\ 
  1345 & 151.295789 &  -7.776235 &     20.994 $\pm$   0.023 &    21.153 $\pm$   0.030 &    20.602 $\pm$   0.022 &      0.037 \\ 
  1346 & 151.355310 &  -7.776508 &     17.590 $\pm$   0.004 &    17.793 $\pm$   0.003 &    18.260 $\pm$   0.004 &      0.980 \\ 
  1347 & 151.257787 &  -7.776301 &     22.936 $\pm$   0.113 &    22.808 $\pm$   0.119 &    22.183 $\pm$   0.081 &      0.653 \\ 
  1348 & 151.365141 &  -7.776587 &     21.075 $\pm$   0.024 &    20.949 $\pm$   0.024 &    20.555 $\pm$   0.020 &      0.347 \\ 
  1349 & 151.276224 &  -7.776689 &     22.340 $\pm$   0.069 &    22.476 $\pm$   0.091 &    22.596 $\pm$   0.123 &      0.713 \\ 
  1350 & 151.347094 &  -7.776687 &     22.201 $\pm$   0.060 &    22.163 $\pm$   0.067 &    22.283 $\pm$   0.086 &      0.750 \\ 
  1351 & 151.261576 &  -7.776838 &     22.053 $\pm$   0.053 &    22.029 $\pm$   0.060 &    21.341 $\pm$   0.040 &      0.260 \\ 
  1352 & 151.261860 &  -7.776974 &     22.110 $\pm$   0.056 &    21.915 $\pm$   0.055 &    21.341 $\pm$   0.040 &      0.077 \\ 
  1353 & 151.250239 &  -7.777298 &     21.218 $\pm$   0.026 &    21.015 $\pm$   0.026 &    20.905 $\pm$   0.027 &      0.037 \\ 
  1354 & 151.357629 &  -7.777125 &     22.146 $\pm$   0.057 &    21.960 $\pm$   0.057 &    21.185 $\pm$   0.034 &      0.050 \\ 
  1355 & 151.271691 &  -7.777208 &     21.694 $\pm$   0.039 &    21.677 $\pm$   0.045 &    21.062 $\pm$   0.032 &      0.683 \\ 
  1356 & 151.292655 &  -7.777317 &     22.804 $\pm$   0.105 &    22.835 $\pm$   0.129 &    22.694 $\pm$   0.134 &      0.537 \\ 
  1357 & 151.361610 &  -7.777437 &     22.224 $\pm$   0.061 &    22.472 $\pm$   0.088 &    22.242 $\pm$   0.083 &      0.543 \\ 
  1358 & 151.254711 &  -7.777618 &     22.115 $\pm$   0.055 &    22.258 $\pm$   0.073 &    21.837 $\pm$   0.058 &      0.047 \\ 
  1359 & 151.361986 &  -7.656605 &     17.700 $\pm$   0.004 &    17.750 $\pm$   0.003 &    17.762 $\pm$   0.003 &      0.980 \\ 
  1360 & 151.330306 &  -7.777964 &     21.672 $\pm$   0.039 &    21.934 $\pm$   0.056 &    21.354 $\pm$   0.039 &      0.007 \\ 
  1361 & 151.256025 &  -7.778147 &     20.512 $\pm$   0.015 &    20.434 $\pm$   0.016 &    20.240 $\pm$   0.016 &      0.150 \\ 
  1362 & 151.269828 &  -7.778168 &     20.360 $\pm$   0.014 &    20.394 $\pm$   0.016 &    20.545 $\pm$   0.021 &      0.983 \\ 
  1363 & 151.369888 &  -7.778156 &     21.764 $\pm$   0.041 &    21.920 $\pm$   0.054 &    21.098 $\pm$   0.031 &      0.083 \\ 
  1364 & 151.299874 &  -7.778215 &     21.527 $\pm$   0.035 &    21.636 $\pm$   0.045 &    21.233 $\pm$   0.037 &      0.423 \\ 
  1365 & 151.331567 &  -7.778258 &     22.385 $\pm$   0.071 &    22.814 $\pm$   0.121 &    22.302 $\pm$   0.088 &      0.540 \\ 
  1366 & 151.363927 &  -7.778304 &     22.454 $\pm$   0.074 &    22.536 $\pm$   0.093 &    22.311 $\pm$   0.088 &      0.687 \\ 
  1367 & 151.346238 &  -7.777664 &     21.673 $\pm$   0.038 &    21.817 $\pm$   0.050 &    21.655 $\pm$   0.050 &      0.400 \\ 
  1368 & 151.311532 &  -7.778610 &     22.743 $\pm$   0.101 &    22.377 $\pm$   0.085 &    22.417 $\pm$   0.105 &      0.480 \\ 
  1369 & 151.251966 &  -7.778808 &     20.774 $\pm$   0.019 &    20.997 $\pm$   0.025 &    21.902 $\pm$   0.060 &      0.907 \\ 
  1370 & 151.327917 &  -7.778875 &     22.327 $\pm$   0.068 &    22.570 $\pm$   0.098 &    21.954 $\pm$   0.066 &      0.073 \\ 
  1371 & 151.253459 &  -7.779607 &     20.297 $\pm$   0.014 &    20.357 $\pm$   0.015 &    20.502 $\pm$   0.019 &      0.177 \\ 
  1372 & 151.319842 &  -7.779647 &     19.236 $\pm$   0.007 &    19.181 $\pm$   0.007 &    19.466 $\pm$   0.009 &      0.983 \\ 
  1373 & 151.341731 &  -7.779604 &     20.183 $\pm$   0.012 &    20.249 $\pm$   0.014 &    20.560 $\pm$   0.020 &      0.977 \\ 
  1374 & 151.371417 &  -7.779790 &     20.936 $\pm$   0.021 &    20.841 $\pm$   0.022 &    20.389 $\pm$   0.018 &      0.303 \\ 
  1375 & 151.268395 &  -7.779826 &     22.438 $\pm$   0.073 &    22.711 $\pm$   0.110 &    22.344 $\pm$   0.096 &      0.573 \\ 
  1376 & 151.317032 &  -7.779895 &     21.295 $\pm$   0.029 &    21.161 $\pm$   0.030 &    20.548 $\pm$   0.021 &      0.370 \\ 
  1377 & 151.366263 &  -7.779956 &     22.193 $\pm$   0.059 &    22.754 $\pm$   0.113 &    22.982 $\pm$   0.161 &      0.283 \\ 
  1378 & 151.279285 &  -7.779990 &     22.770 $\pm$   0.099 &    22.968 $\pm$   0.140 &    22.154 $\pm$   0.083 &      0.580 \\ 
  1379 & 151.299359 &  -7.780179 &     20.197 $\pm$   0.013 &    20.245 $\pm$   0.014 &    20.625 $\pm$   0.022 &      0.980 \\ 
  1380 & 151.274456 &  -7.780299 &     20.865 $\pm$   0.020 &    20.909 $\pm$   0.024 &    21.172 $\pm$   0.035 &      0.793 \\ 
  1381 & 151.353228 &  -7.656304 &     20.856 $\pm$   0.020 &    22.684 $\pm$   0.094 &    21.100 $\pm$   0.032 &      0.883 \\ 
  1382 & 151.300723 &  -7.780840 &     22.214 $\pm$   0.061 &    22.219 $\pm$   0.073 &    21.639 $\pm$   0.053 &      0.457 \\ 
  1383 & 151.254754 &  -7.781179 &     21.878 $\pm$   0.045 &    21.909 $\pm$   0.054 &    21.896 $\pm$   0.060 &      0.463 \\ 
  1384 & 151.261238 &  -7.781187 &     21.218 $\pm$   0.026 &    21.381 $\pm$   0.035 &    21.882 $\pm$   0.061 &      0.860 \\ 
  1385 & 151.249827 &  -7.781337 &     21.833 $\pm$   0.044 &    21.982 $\pm$   0.058 &    22.451 $\pm$   0.098 &      0.197 \\ 
  1386 & 151.342458 &  -7.781265 &     21.938 $\pm$   0.048 &    22.190 $\pm$   0.069 &    22.760 $\pm$   0.131 &      0.803 \\ 
  1387 & 151.352549 &  -7.781347 &     22.659 $\pm$   0.089 &    22.392 $\pm$   0.082 &    21.578 $\pm$   0.047 &      0.340 \\ 
  1388 & 151.277431 &  -7.781541 &     21.689 $\pm$   0.039 &    21.685 $\pm$   0.045 &    21.916 $\pm$   0.067 &      0.880 \\ 
  1389 & 151.273058 &  -7.781608 &     21.909 $\pm$   0.047 &    21.894 $\pm$   0.054 &    21.569 $\pm$   0.049 &      0.103 \\ 
  1390 & 151.345735 &  -7.781538 &     22.248 $\pm$   0.062 &    22.410 $\pm$   0.084 &    22.274 $\pm$   0.085 &      0.613 \\ 
  1391 & 151.283871 &  -7.657680 &     21.316 $\pm$   0.029 &    21.320 $\pm$   0.035 &    20.111 $\pm$   0.015 &      0.020 \\ 
  1392 & 151.315785 &  -7.657864 &     22.531 $\pm$   0.082 &    22.683 $\pm$   0.117 &    21.764 $\pm$   0.062 &      0.573 \\ 
  1393 & 151.360162 &  -7.657963 &     23.094 $\pm$   0.131 &    22.681 $\pm$   0.106 &    21.686 $\pm$   0.052 &      0.437 \\ 
  1394 & 151.340560 &  -7.658107 &     21.869 $\pm$   0.045 &    21.867 $\pm$   0.054 &    22.068 $\pm$   0.080 &      0.797 \\ 
  1395 & 151.274702 &  -7.658182 &     21.963 $\pm$   0.049 &    22.162 $\pm$   0.070 &    21.295 $\pm$   0.039 &      0.060 \\ 
  1396 & 151.273088 &  -7.780728 &     20.955 $\pm$   0.022 &    20.841 $\pm$   0.022 &    20.382 $\pm$   0.018 &      0.307 \\ 
  1397 & 151.252144 &  -7.658406 &     22.419 $\pm$   0.072 &    22.046 $\pm$   0.061 &    21.150 $\pm$   0.032 &      0.197 \\ 
  1398 & 151.316274 &  -7.658348 &     22.708 $\pm$   0.096 &    22.663 $\pm$   0.115 &    21.737 $\pm$   0.061 &      0.503 \\ 
  1399 & 151.264374 &  -7.658477 &     21.733 $\pm$   0.040 &    21.378 $\pm$   0.035 &    20.619 $\pm$   0.021 &      0.590 \\ 
  1400 & 151.353007 &  -7.658381 &     23.137 $\pm$   0.136 &    23.135 $\pm$   0.160 &    22.616 $\pm$   0.124 &      0.543 \\ 
  1401 & 151.293301 &  -7.658647 &     20.867 $\pm$   0.021 &    20.886 $\pm$   0.024 &    20.821 $\pm$   0.027 &      0.967 \\ 
  1402 & 151.331540 &  -7.658584 &     22.648 $\pm$   0.090 &    22.270 $\pm$   0.080 &    21.202 $\pm$   0.038 &      0.400 \\ 
  1403 & 151.319347 &  -7.659111 &     17.327 $\pm$   0.003 &    17.232 $\pm$   0.002 &    17.331 $\pm$   0.002 &      0.983 \\ 
  1404 & 151.324608 &  -7.658906 &     21.872 $\pm$   0.046 &    21.614 $\pm$   0.045 &    21.068 $\pm$   0.034 &      0.677 \\ 
  1405 & 151.263318 &  -7.659224 &     19.658 $\pm$   0.009 &    19.729 $\pm$   0.010 &    19.842 $\pm$   0.012 &      0.977 \\ 
\end{tabular} \\
\tablefoot{Columns list: (1) ID number; (2) right ascension; (3) declination; (4) $J-$band magnitude; (5) $H-$band magnitude; (6) $K_s-$band magnitude; (7) SExtractor mean $JHKs$ CLASS\_STAR parameter.}
\end{table}

